Fine-Tuning and Prompt Engineering for Large Language Models-based Code Review Automation

Context: The rapid evolution of Large Language Models (LLMs) has sparked significant interest in leveraging their capabilities for automating code review processes. Prior studies often focus on developing LLMs for code review automation, yet require expensive resources, which is infeasible for organizations with limited budgets and resources. Thus, fine-tuning and prompt engineering are the two common approaches to leveraging LLMs for code review automation. Objective: We aim to investigate the performance of LLMs-based code review automation based on two contexts, i.e., when LLMs are leveraged by fine-tuning and prompting. Fine-tuning involves training the model on a specific code review dataset, while prompting involves providing explicit instructions to guide the model's generation process without requiring a specific code review dataset. Method: We leverage model fine-tuning and inference techniques (i.e., zero-shot learning, few-shot learning and persona) on LLMs-based code review automation. In total, we investigate 12 variations of two LLMs-based code review automation (i.e., GPT- 3.5 and Magicoder), and compare them with the Guo et al.'s approach and three existing code review automation approaches. Results: The fine-tuning of GPT 3.5 with zero-shot learning helps GPT-3.5 to achieve 73.17% -74.23% higher EM than the Guo et al.'s approach. In addition, when GPT-3.5 is not fine-tuned, GPT-3.5 with few-shot learning achieves 46.38% - 659.09% higher EM than GPT-3.5 with zero-shot learning. Conclusions: Based on our results, we recommend that (1) LLMs for code review automation should be fine-tuned to achieve the highest performance; and (2) when data is not sufficient for model fine-tuning (e.g., a cold-start problem), few-shot learning without a persona should be used for LLMs for code review automation.

==> section-exp-only/Approach.tex <==
\section{D-ACT: Diff-Aware Code Transformation for Code Review} \label{sec:approach}

%%% Figure sota-vs-ours and Figure motivating-example are in Background.tex
%%% cannot place the above figures here since it will be at the top on the next page (p. 4)


% \begin{figure}[ht]
%     \centering
%     \includegraphics[page=1, width=\linewidth]{figure/overall-approach.pdf}
%     \caption{An overview of our approach.}
%     \label{fig:overview}
% \end{figure}

% \begin{figure*}
%     \centering
%     \includegraphics[page=1, width=\textwidth]{figure/overall-approach-new.pdf}
%     % \caption{An overview of our approach. The bold arrows present the flow of the processes, while the dashed lines present the examples in the process. In the example, the added tokens are in red, while the modified tokens are in blue.}
%     \caption{An overview of our approach. The bold arrows represent the flow of the processes, while the dashed arrows represent the examples in the process. In the example, the changed token is in blue. \kla{pick said step 2 can be combined, but it's not combined yet. 2 separate boxes mean 2 different actions, which is not what we do.}
%     \kla{no one explain arrows in SE papers before (this is the first). Clear figure should be self-explanatory by itself without additional explanations. The figure caption could better sell the key point of the figure, instead of explaining what the arrows are.}
%     }
%     \label{fig:overview}
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[page=1, width=\textwidth]{figure/our-approach.pdf}
    \caption{
    An overview of our approach.
    }
    \label{fig:overview}
\end{figure*}

\pick{
In this section, we present our D-ACT, an NMT-based code transformation approach that leverages  the token-level code difference information and CodeT5 --- the state-of-the-art pre-trained code model~\cite{wang2021codet5}.
}

\pick{Our underlying intuition of using the token-level code difference information is that changed code tokens are more likely to introduce defects than the others~\cite{beller2014modern}; thus, explicitly providing such information may help NMT models better learn the code transformation.
Figure \ref{fig:sota-vs-ours} illustrates an example of the input of our approach. 
Generally speaking, D-ACT uses special tokens (i.e., \texttt{<START\_MOD>} and \texttt{<END\_MOD>}) to explicitly specify which code tokens in the initial version were changed from the codebase version.
We hypothesize that with this information, the NMT model will better capture the relationship between all code tokens and the given special tokens, reducing the probability that code tokens outside of the special tokens will be changed.
We also opt to use the CodeT5 pre-trained model because the model was specifically trained to learn the syntactic and semantic information of code tokens.
This is different from the pre-trained T5 model of Tufano~\ea~\cite{tufano2022using}, which learns source code without focusing syntactic information of code tokens.}



% \textbf{A Motivating Example.} 

%% previously this paragraph is in background
%% will revise later
% However, the aforementioned approaches only learn from the sequence of code tokens without knowing where are newly added code tokens in the initial version
% (as shown in a code diff, i.e., the difference between the codebase and the initial version) like code reviewers \changed{see} in the real practice.
% \oat{example seems weak, or cherry pick}


% For example, Figure~\ref{fig:sota-vs-ours} depicts 
% \kla{demonstrate is not the right word here, as it does not demonstrate anything} 
% the input sequence of code tokens, and the generated output sequences of such approaches and our D-ACT. \kla{make the sentence more specific and insightful, rather than explain This figure presents a book and a cat, but let's say "the cat does poo-poo on a book, making the book dirty". this is more insightful.}
% From this figure, the state-of-the-art code transformation approaches for code review only take a sequence of code tokens of \mInit as the input, without knowing which code tokens are previously changed from the codebase.
% Thus, as mentioned in the limitation of AutoTransform~\cite{AutoTransform}, such approaches may make changes to other code tokens that should remain unchanged.
% In contrast, our approach takes a sequence of code tokens of \mInit, and the code diff (as presented by the special tokens (\texttt{<START\_MOD>} and \texttt{<END\_MOD>}) as the input.
% Thus, our approach only make change to the code token between these special tokens (i.e., \texttt{empty}), while keeping the other code tokens unchanged.

% Thus, such approaches may incorrectly generate the other code tokens that should remain unchanged.
% Thus, such approaches may incorrectly generate \mApproved (when compared to \mApproved in Figure~\ref{fig:motivating-example}) by modifying the other code tokens that should remain unchanged.
% In contrast, our approach uses a sequence of code tokens of \mInit, and special tokens (\texttt{<START\_MOD>} and \texttt{<END\_MOD>}) to represent code diff as the input.
% In contrast, our approach uses a sequence of code tokens of \mInit, and the code diff (as presented by the special tokens (\texttt{<START\_MOD>} and \texttt{<END\_MOD>}) as the input.
% to indicate the changed code tokens in \mInit as input.
% These special tokens are used to indicate that an NMT model should pay more attention to the code tokens between these tokens.
% These special tokens indicates an NMT model that it should pay more attention to the code tokens between these special tokens.
% Thus, our approach only make change to the code token between these special tokens (i.e., \texttt{empty}), while keeping the other code tokens unchanged.
% Thus, our approach can correctly generate $m_{approved}$ (when compared to \mApproved in Figure~\ref{fig:motivating-example}), since our approach only makes change to the code token between these special tokens (i.e., \texttt{empty}).
% , while keeping the other code tokens unchanged.

% In contrast, our approach leverages token-level change information to indicate which code tokens that should be paid more attention.


% From this figure, the state-of-the-art code transformation approaches do not know which code tokens that should be transformed.
% Thus, such approaches may make changes to code tokens that should remain unchanged.
% Thus, such approaches may pay attention to code tokens that should remain unchanged.
% In contrast, our approach leverages the code diff information to let a model knows that the code token \texttt{empty} should be given more attention.


% In this section we explain \kla{wording explain considered as just a report. Do you want to sell your work or just explain this work to someone. Voices, Languages in the paper will have a strong influence on the reviewer's decision.} dataset collection, how we insert code diff information to \mInit, and an NMT architecture of our approach.

% \kla{wording should be consistent. first says data collection (noun), but later says how-question. CONSISTENCY ISSUE!! and realistically, no one will care 'how we insert'. they care about how your approach works. Use the right tones, voices, languages, verbs, etc.}
% \kla{$m_{codebase}$ and others are never defined.}
% However, the existing code transformation approaches for code review~\cite{AutoTransform,tufano2022using} only learn from the sequence of code tokens without knowing where are newly added code tokens \kla{do you consider only newly added or modified as well? I'm confused.} in the initial version
% (as shown in a \textit{code diff}, i.e., the difference between the codebase and the initial version) like code reviewers \changed{see} in the real practice.


% \kla{why start with For example. I don't get much. The flow is not smooth.}
% For example, from Figure~\ref{fig:sota-vs-ours}, the state-of-the-art code transformation approaches for code review only take a sequence of code tokens of \mInit as input, without knowing which code tokens are previously changed from the codebase.
% Thus, as mentioned in the limitation of AutoTransform~\cite{AutoTransform}\kla{a bit weird}, such approaches may make changes to other code tokens that should remain unchanged (highlighted in yellow).
% In contrast, our approach takes a sequence of code tokens of \mInit, and the code diff (as presented by the special tokens (\texttt{<START\_MOD>} and \texttt{<END\_MOD>}) as the input.
% Thus, our approach only make change to the code token between these special tokens (i.e., \texttt{empty}), while keeping the other code tokens unchanged.


% Figure~\ref{fig:sota-vs-ours} presents an example of a code review from the Ovirt project (Change-Id: Iff1f2d), consisting of three versions of the same method, i.e., the \textit{codebase version ($m_{codebase}$)}, the \textit{initial version ($m_{initial}$)}, and the \textit{approved version ($m_{approved}$)}.
% As depicted in this example, reviewers tend to provide comments related to the changed code tokens (i.e., \texttt{empty}) rather than the others. 
% Eventually, the changed code token is later then changed in the approved version (i.e., \texttt{empty} $\rightarrow$ \texttt{EMPTY}), highlighting the importance of the code difference information in the real-world code review practices. 


\subsection{Overview}

Figure~\ref{fig:overview} presents an overview of our D-ACT approach, which consists of three main steps: \pick{(Step 1)} data preparation,  \pick{(Step 2)} training phase, and  \pick{(Step 3)} inference phase.
\pick{In Step 1, we extract three versions of a changed method, i.e., codebase ($m_\mathrm{codebase}$), initial ($m_\mathrm{initial}$), and approved versions ($m_{\mathrm{approved}}$).
Then, we integrate the token-level code difference information into $m_\mathrm{initial}$ (i.e., $m_\mathrm{initial+diff}$).
Once we prepare the dataset, we use pairs of $m_\mathrm{initial+diff}$ and $m_\mathrm{approved}$ to fine-tune the CodeT5 pre-trained model in Step 2.
Finally, in Step 3, for each patch in the testing dataset, we use the fine-tuned CodeT5 model to generate $m_\mathrm{approved}$ based on a given $m_\mathrm{initial+diff}$. }
We describe the details of each step of our D-ACT below.
% In the data preparation step (Step 1), we first obtain three versions of a changed file in a \pick{submitted} patch (i.e., the codebase version, the initial version, and the approved version).
% Then, we identify the changed methods from the three versions of the changed file, resulting $m_{codebase}$, $m_{initial}$ and $m_{approved}$.
% Next, we use \mCodebase and \mInit to analyze the token-level code difference, which is subsequently integrated to $m_{initial}$ resulting $m_{initial+diff}$.
% After that we obtain the dataset which consists of \mInitWithDiff and $m_{approved}$.
% We then split the dataset to the training dataset and the testing dataset.
% In the training phase (Step 2), we first perform subword tokenization on the \mInitWithDiff and $m_{approved}$, using BPE.
% After that we use the tokenized \mInitWithDiff and \mApproved to fine-tune CodeT5.
% In the inference phase (Step 3), we begin with performing subword tokenization on the $m_{initial+diff}$.
% Then, we use the fine-tuned CodeT5 model to generate $m_{approved}$.




\pick{
\subsection{(Step 1) Data Preparation} \label{sec:collect-data}
The key goal of our data preparation step is to integrate the token-level code difference information into the $m_{\mathrm{initial}}$.
To do so, for each changed file in each patch, we first identify changed methods based on its codebase, initial, and approved versions.
Specifically, we employ a source code analysis tool namely Iterative Java Matcher (IJM)~\cite{frick2018generating}\footnote{https://github.com/VeitFrick/IJM} to extract pairs of changed methods between the codebase and initial versions of a changed file, i.e., $\langle m_\mathrm{codebase}, m_\mathrm{initial}\rangle$; and pairs of changed methods between the initial and approved versions $\langle m_\mathrm{initial}, m_\mathrm{approved}\rangle$.
Then, we merge each of $\langle m_\mathrm{codebase}, m_\mathrm{initial}\rangle$ and $\langle m_\mathrm{initial}, m_\mathrm{approved}\rangle$ into a triplet of the changed method $\langle m_\mathrm{codebase}, m_\mathrm{initial}, m_\mathrm{approved} \rangle$ based on the whole content of $m_\mathrm{initial}$.
Note that in our approach, we also consider the newly-added $m_{\mathrm{initial}}$, i.e., $\langle $\O$, m_\mathrm{initial}, m_\mathrm{approved} \rangle$, but we do not consider deleted methods $\langle m_\mathrm{codebase}, m_\mathrm{initial}, $\O$ \rangle$ or $\langle m_\mathrm{codebase}, $\O$, $\O$ \rangle$ since our approach aims to transform the existing \mInit in a patch to the version that is reviewed and approved.
}

% The patch is composed of the difference between the codebase and the initial version, and the difference between the initial version and the approved version. \kla{I don't think so. You said in the intro that the patch is a set of code change, but now you explain something else}
% Then, we reconstruct \kla{why do we need to reconstruct? what is the purpose? what is the problem?} java files from the difference between two versions of a file. which is composed of the added lines, the deleted lines, and the unchanged lines, unlike the code difference obtained from \texttt{git} that contains only the added lines and deleted lines.
% To do so, we reconstruct \kla{same as above? repeat the explanation? why say 'we reconstruct' two times, redundant?} the Java files of the codebase and the Java files of the initial version from the difference between the codebase and the initial version.
% Similarly, we reconstruct the Java files \kla{no one will understand why you need to do this. just clone the repo then you will get the java file. Reviewers will not buy this idea.} of the approved version from the difference between the initial version and the approved version.

% \kla{this does not mean what you did is wrong, but the explanation is not convincing.}
% Then, we reconstruct the Java files of the codebase and the Java files of the initial version from the patch of the codebase $\rightarrow$ the initial version.
% Similarly, we reconstruct the Java files of the approved version from the patch of the initial version $\rightarrow$ the approved version.
% Then, we reconstruct the Java files of the codebase and the Java files of the initial version from the $\varB{Gerrit-Diff_{codebase,initial}}$.
% Similarly, we reconstruct the Java files of the approved version from the $\varB{Gerrit-Diff_{initial,approved}}$.

% To prepare the changed method to analyze and integrate the token-level code difference to $m_{initial}$, we identify the changed method, which is represented as a triplet $\langle m_{codebase}, m_{initial}, m_{approved} \rangle$ from the 3 versions of Java files.
% To obtain the triplet, we first extract pairs of \pairCbInit and $\langle m_{initial}, m_{approved} \rangle$
% %% use \hspace{3cm} to make paragraph looks beautiful
% % After the 3 versions of Java files are obtained from the previous step, we form triplets $\langle m_{codebase}, m_{initial}, m_{approved} \rangle$, by joining \pairCbInit and $\langle m_{initial}, m_{approved} \rangle$.
% % Next, from the 3 versions of Java files in the previous step, we create two types of method pairs (i.e., \pairCbInit where \mCodebase is the method of codebase and \mInit is the method of initial version), and \pairInitApp where \mApproved is the method of approved version)), which will be used to form triplets \triplet. 
% % We choose method-level granularity instead of file-level granularity since Java files are usually composed of a complex structure of classes and methods, which an NMT model may not accurately transform the whole files. 
% by employing a source code analysis tool namely Iterative Java Matcher (IJM)\footnote{https://github.com/VeitFrick/IJM}~\cite{frick2018generating}.
% Given two Java files, IJM establishes method-to-method mapping and then identifies AST operations performed on methods of both Java files, which can be used to identify the pairs of modified methods. 
% In particular, we use IJM to extract \pairCbInit from the Java files of codebase and the Java files of the initial version, and extract the \pairInitApp from the Java files of the initial and the Java files of the approved version. 
% Then, we combine the extracted \pairCbInit and \pairInitApp to form \triplet according to PR-ID, filename and $m_{initial}$, since our work aims to
% % transform the \mInit of the same file in a pull request to the ones of the approved version.
% transform the \mInit of the same file in a patch to the version that is reviewed and approved.

% However, it is possible that the \mInit are newly added to the initial version.
% % However, some \mCodebase of the corresponding \mInit are missing since these \mInit are added in the initial version of a patch (they are newly added to the existing or new Java files).
% % can be added to the existing Java files, or come from newly added Java files). 
% Later, these \mInit are revised until the patch is approved.
% Thus, the method pairs \pairCbInit are missing.
% % Thus, \triplet containing these \mInit mentioned above cannot be formed since there are only $<m_{initial}, m_{approved}>$.
% To ensure that the dataset aligns with the goal of our work, we include \triplet containing such \mInit in our dataset, where the \mCodebase of these triplets are represented as empty.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[page=1,width=\columnwidth]{figure/code-modification-status-identification.pdf}
%     % \caption{How code diff information is inserted to $m_{initial}$. \kla{the caption needs to be rewritten.}}
%     % \caption{How the the representation of the code diff is combined with $m_{initial}$.}
%     \caption{An approach to combine the code diff and $m_{initial}$. The added code tokens are shown in orange, while the modified code tokens are shown in blue.}
%     \label{fig:code-mod-identification}
% \end{figure}

\pick{After we obtain a triplet of a changed method, we analyze the token-level difference information and integrate it into $m_\mathrm{initial}$.
We integrate the token-level code difference information into $m_\mathrm{initial}$ by inserting special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} to specify the code tokens that were changed from $m_\mathrm{codebase}$. 
Figure \ref{fig:sota-vs-ours} shows an example of $m_\mathrm{initial}$ with the token-level code difference information ($m_\mathrm{initial+diff}$).
To do so, we first identify the code tokens in $m_\mathrm{initial}$ that were changed from $m_\mathrm{codebase}$.
Specifically, we tokenize $m_\mathrm{initial}$ and  $m_\mathrm{codebase}$ in sequences of tokens using the Java parser namely  \texttt{javalang}\footnote{https://github.com/c2nes/javalang}.
% Specifically, we use the \texttt{javalang} Java parser\footnote{https://github.com/c2nes/javalang} to tokenize $m_\mathrm{initial}$ and  $m_\mathrm{codebase}$ to sequences of tokens.
Then, we use the approach of Liu~\ea~\cite{liu2021just} to align code tokens between $m_\mathrm{initial}$ and  $m_\mathrm{codebase}$ and identify the changed code tokens (i.e., either replaced or inserted).
Finally, in $m_\mathrm{initial}$, we insert \texttt{<START\_MOD>} and \texttt{<END\_MOD>} at the beginning and the end of each sequence of the changed tokens to produce $m_\mathrm{initial+diff}$.}

% After we obtain the 3 versions of a changed method, we analyze the token-level code difference, using \mCodebase and \mInit.
% We then integrate the obtained token-level code difference to $m_{initial}$, resulting $m_{initial+diff}$.
% To analyze the token-level code difference, we adapt the approach of Liu~\ea~\cite{liu2021just} to identify the edit operation (i.e., \textit{insert}, \textit{delete}, \textit{equal} and \textit{replace}) of the code tokens in $m_{initial}$.
% To begin, \mCodebase and \mInit are tokenized to a sequence of tokens (i.e.,  \tokCodebase and $tm_{initial}$, respectively) by using the Java parser provided by the \texttt{javalang}\footnote{https://github.com/c2nes/javalang} library.
% % Then, we use the approach of Liu~\ea~\cite{liu2021just} to compare the \tokCodebase with the \tokInit to identify the edit operation of $tm_{initial}$.
% Then, we use the token-level alignment approach of Liu~\ea~\cite{liu2021just} to obtain the alignment of the \tokCodebase the $tm_{initial}$.
% The alignment is then used to identify the edit operation of $tm_{initial}$.
% % \kla{you said you use the approach of Liu, but what exactly is this approach -- no one will understand it.  e.g., I use the approach of Oat to walk to the Woodside -- so HOW?}
% % After the edit operation of each \tokInit is obtained, the sequences of \tokInit that have edit operation \textit{insert} or \textit{replace} are identified.
% % Then, the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are added at the beginning and at the end of the sequences, respectively.
% The obtained edit operation is the token-level code difference, which will be integrated to $m_{initial}$.
% To integrate the token-level code difference to $m_{initial}$, we first identify the sequence(s) of code tokens in \tokInit that begin with code tokens having edit operation \textit{insert} or \textit{replace}.
% Then, we insert the special token \texttt{<START\_MOD>} and \texttt{<END\_MOD>} at the beginning and the end of the identified sequence(s), respectively.
% % To integrate the token-level code difference to $m_{initial}$, we insert the special token \texttt{<START\_MOD>} at the beginning and insert the special token \texttt{<END\_MOD>} and at the end of the sequences of the code tokens \kla{what tokens? one method has 100 tokens, where? all?, the language is ambiguous and it is not precisely explained} in \mInit that their corresponding edit operations are \textit{insert} or \textit{replace} \kla{too long, I don't get it (from reading)}, resulting $m_{initial+diff}$.
% % \kla{I know what you do, but the explanation is hard to understand}
% % After that the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are inserted at the beginning and at the end of the sequences of tokens in \mInit that their corresponding edit operations are \textit{insert} or \textit{replace}.
% % surrounded by special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>}.
% % For the edit operation \textit{delete}, since the deleted tokens are not presented in $m_{initial}$, the tokens that have edit operation \textit{delete} are ignored.
% % The example of how to combine the representation of the code diff to \mInit can be seen in Figure~\ref{fig:overview}.
% % For example, in Figure~\ref{fig:overview}, the code token \texttt{Empty} in \mCodebase is modified to \texttt{empty} in $m_{initial}$.
% For example, suppose \tokCodebase is \{ \texttt{…}, ``\texttt{(}'', ``\texttt{this}'', ``\texttt{,}'', ``\texttt{EventArgs}'', ``\texttt{.}'', ``\texttt{Empty}'', ``\texttt{)}'', ``\texttt{;}'' \} and \tokInit is \{ \texttt{…}, ``\texttt{(}'', ``\texttt{this}'', ``\texttt{,}'', ``\texttt{EventArgs}'', ``\texttt{.}'', ``\texttt{empty}'', ``\texttt{)}'', ``\texttt{;}'' \}, the code token \texttt{Empty} in \tokCodebase is modified to \texttt{empty} in $tm_{initial}$.
% Thus, the the edit operation of the code token \texttt{empty} is \texttt{replace}.
% Then, the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are inserted before and after \texttt{empty}, respectively.
% Finally, the \mInitWithDiff is \texttt{… (this, EventArgs.<START\_MOD>empty<END\_MOD>);}.


% For example, in Figure~\ref{fig:overview}, the code diff between \mCodebase and \mInit is \{\texttt{Empty},  \texttt{empty}\}.
% To combine this code diff to \mInit, the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are inserted at the beginning and at the end of the code token \texttt{empty}, respectively.
% % Thus, the edit operation of the code token \texttt{empty} is \textit{replace}.
% % Then, the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are inserted at the beginning and at the end of the code token \texttt{empty}, respectively.
% Note that the code tokens that have the edit operation \textit{delete} are ignored since they are not presented in $m_{initial}$.
% \kla{I think I need Pick to double-check this section again. It's quite plain language.}


% From the example in Figure~\ref{fig:code-mod-identification}, the code tokens \texttt{pattern}, \texttt{.} are added to $m_{initial}$.
% In addition, the code token \texttt{get\_pattern} of \mCodebase is replaced by \texttt{pattern} of $m_{initial}$.
% Thus, their edit operations are \textit{insert}, \textit{insert} and \textit{replace}, respectively.
% Then, the special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are inserted at front of the inserted \textit{insert} and at the back of the modified code token \textit{replace}, respectively.


% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{figure/model-architecture.pdf}
%     \caption{\oat{will remove this fig later.} An overview architecture of the \changed{CodeT5} model of our approach.}
%     % \kla{unusually large :( very awkward. same issue here.}
%     \label{fig:model-architecture}
% \end{figure*}

% From all steps above, we finally obtain the pairs of \mInitWithDiff and $m_{approved}$.


% Finally, we obtain \kla{obtain from where? -- wrong verb?....} \mInitWithDiff and $m_{approved}$, which are split to the training dataset and testing dataset\kla{need a pause.... no one will understand -- you obtain, then split -- hmm? the two verbs are conflicting with each other}.


\subsection{(Step 2) Training Phase}

During the training phase, we leverage the CodeT5 pre-trained code model to learn code transformation in code review through the relationship between the pairs of $m_\mathrm{initial+diff}, m_\mathrm{approved}$ in the training dataset.
Prior to training a model, tokenization plays an important role to break source code into a meaningful sequence of code tokens. 
As suggested by prior work~\cite{AutoTransform, karampatsis2020big,fu2022vulrepair}, 
% \kla{+cite big code != big vocab}, 
we leverage the Byte-Pair Encoding (BPE) approach~\cite{Sennrich2016} to perform subword tokenization, i.e., split tokens into a list of sub-tokens.
With the use of BPE subword tokenization, it will greatly reduce the vocabulary size, while enabling the model to create new tokens that never appear in the training dataset.
We use the BPE tokenizer that is trained on the CodeSearchNet (CSN) corpus~\cite{husain2019codesearchnet}, provided by Wang~\ea~\cite{wang2021codet5}.
Since our approach uses special tokens (i.e., \texttt{<START\_MOD>} and \texttt{<END\_MOD>}) to explicitly specify which code tokens in the \mInit are changed from $m_{\mathrm{codebase}}$, we include the special tokens in the BPE tokenizer to ensure that these tokens will not be split into sub-tokens.
Then, we apply the BPE tokenizer to $m_\mathrm{initial+diff}$ and $m_\mathrm{approved}$ to produce subtoken-level methods (i.e., $sm_\mathrm{initial+diff}$ and $sm_\mathrm{approved}$, respectively), where these subtoken-level methods contain a sequence of subtokens $sm = [\mathrm{st}_1, ..., \mathrm{st}_n]$.
Finally, we feed these sequences into the CodeT5 pre-trained code models in order to learn the relationship between the input sequence of the initial version ($sm_\mathrm{initial+diff}$) and the output sequence of the approved version ($sm_\mathrm{approved}$) for each patch in the training dataset to build an NMT model.
Below, we describe the technical details of the BPE tokenization and the architecture of CodeT5.

% by the 
% To use BPE for D-ACT, we apply the BPE tokenizer obtained from~\cite{wang2021codet5}.
% that is pre-trained on CodeSearchNet (CSN)~\cite{husain2019codesearchnet} and a C/C\# corpus extracted by Wang~\ea~\cite{wang2021codet5}.


% To avoid the BPE tokenizer

% In addition, 



% Before $m_{initial+diff}$ or $m_{approved}$ is split to a sequence of tokens, the special tokens \texttt{<s>} and \texttt{</s>} are added to represent the beginning of a sequence (BOS) and the end of a sequence (EOS), respectively.
% In addition, our special tokens \texttt{<START\_MOD>} and \texttt{<END\_MOD>} are added to the tokenizer to ensure that these tokens are not split to sub-tokens when \mInitWithDiff (or $m_{approved}$) is tokenized.


% In this step, we use \pick{pairs of} \mInitWithDiff and \mApproved to fine-tune the pre-trained CodeT5~\cite{wang2021codet5} model.
% Below we explain the detail of BPE tokenization and the architecture of CodeT5.


\subsubsection{BPE Tokenization}
% We use 
% Using BPE can reduce vocabulary size since rare tokens will be split into multiple sub-tokens.
% To use BPE for D-ACT, we apply the BPE tokenizer obtained from~\cite{wang2021codet5}.
% that is pre-trained on CodeSearchNet (CSN)~\cite{husain2019codesearchnet} and a C/C\# corpus extracted by Wang~\ea~\cite{wang2021codet5}.
% \kla{explain below how BPE works?}
The BPE tokenization process consists of two main steps: generating merge operations which determine how code tokens should be split, and applying merge operations to split code tokens into a list of sub-tokens.
To generate merge operations, BPE first splits all code tokens into a list of characters.
Next, BPE generates a merge operation by identifying the symbol pair (i.e., the pair of two consecutive characters) having the highest frequency in a corpus.
Then, the co-occurrence characters appearing in the identified symbol pair are replaced by the symbol pair, without removing a single character that appears in the symbol pair.
After that, the symbol pair is added to the vocabulary list.
For example, suppose that (`a',`c') has the highest frequency.
The merge operation is (`a',`c') $\rightarrow$ 'ac', which will replace  all of the co-occurrence of (`a', `c') with `ac', without removing `a’ or `c’ that appears alone.
The above steps are then repeated until a given number of merge operations is reached.

After the merge operations are generated, we apply the merge operations to split code tokens into a list of sub-tokens.
To do so, BPE first splits all code tokens into sequences of characters.
Then, the generated merge operations are applied to \mInitWithDiff and \mApproved in the training data, resulting \subTokInitWithDiff and $sm_{\mathrm{approved}}$, respectively.
% Besides, the generated merge operations are applied to \mInitWithDiff in the testing data.

\subsubsection{The Architecture of CodeT5}
The architecture of the CodeT5 is based on the T5 architecture~\cite{raffel2020exploring}, which begins with a word embedding layer, followed by an encoder block and a decoder block.
The architecture then ends with a linear layer and a softmax activation function.

% \kla{please polish the rest}

\smallsection{Word Embedding Layer}
% \kla{too many acronyms, it's better to have all acronyms defined in one place and clearly illustrate what it is and where it is in the code review. It's too hard to understand for non-experts.}
% After \mInit (or \mApproved) is tokenized to a sequence of sub-tokens \subTokInit (or \subTokApprove), each sub-token is converted to an embedding vector that can be obtained from a word embedding matrix.
Given \subTokInitWithDiff (or $sm_{\mathrm{approved}}$) obtained from BPE tokenization, we generate an embedding vector for each sub-token and combine into an embedding matrix.
% After \mInitWithDiff (or $m_{approved}$), is tokenized to \subTokInitWithDiff (or $sm_{approved}$), each sub-token is converted to an embedding vector that can be obtained from a word embedding matrix.
Then, to capture the information related to the position of each token, unlike BERT~\cite{devlin2018bert} that combines embedding vectors with the vectors obtained from absolute position encoding, CodeT5 leverages relative position encoding to encode the position of tokens during self-attention calculation.
The self-attention mechanism is described below.

\smallsection{The Encoder Block}
The generated word embedding matrix of \subTokInitWithDiff is fed to the encoder block, which consists of six identical encoder layers.
Similar to a Vanilla Transformer~\cite{Vaswani2017}, each encoder layer is composed of two sub-components: a multi-head self-attention mechanism and a fully-connected feed-forward network (FFN).
Before the input vector is fed to each sub-component, layer normalization~\cite{ba2016layer} and residual skip connection~\cite{he2016deep} are respectively applied to the input vector.
Different from Vanilla Transformer~\cite{Vaswani2017}, the layer normalization here is a simplified version where additive bias is not applied.
% there is no additive bias being applied.

% to capture the contextual relationship between all tokens in the whole sequence

Multi-head self-attention mechanism~\cite{Vaswani2017} is employed to allow CodeT5 to capture the contextual relationship between all tokens in the whole sequence.
In particular, the multi-head self-attention mechanism calculates the attention score of each token by using the dot product operation.
There are three main components for calculating the attention score: query ($Q$), key ($K$), and value ($V$) matrices.
% The self-attention mechanism performs the following steps to compute the attention score.
% The self-attention mechanism works as follow.
The attention weight is first computed by taking the scaled dot-product between $Q$ and $K$.
The softmax function is then applied to the result of the dot-product.
Finally, the dot-product between the result obtained from the softmax function and $V$ is calculated to update the value in $V$.
However, different from Vanilla Transformer~\cite{Vaswani2017} that encodes the absolute position of each token before computing self-attention score, CodeT5 uses relative positional encoding to efficiently represent the position of tokens.
Thus, an additional matrix $P$, which represents the relative position of tokens, is computed and supplied during self-attention calculation.
% The self-attention calculation can be presented as the equation below:
% $$Attention(Q,K,V,P) = softmax(\frac{Q(K+P)^T}{\sqrt{d_k}})(V+P)$$
Finally, the attention vectors obtained from the last encoder layer will be used to help decoder layers focus on appropriate tokens in the $sm_{\mathrm{initial+diff}}$.

\smallsection{The Decoder Block}
% The attention vectors generated by the encoder block is fed to the decoder block, which consists of six identical decoder layers.
The generated embedding matrix of \subTokApprove is fed to the decoder block, which consists of six identical decoder layers.
Each decoder layer is composed of the sub-components similar to the ones in the encoder layer.
% However, the difference between the encoder layer and the decoder layer is that the decoder layer uses special kind of self-attention mechanisms (i.e., masked multi-head self-attention and multi-head encoder-decoder self-attention) to generate attention vectors.
However, different from the encoder layer, the decoder layer uses special kinds of self-attention mechanism (i.e., masked multi-head self-attention and multi-head encoder-decoder self-attention) to generate attention vectors.
The concept of the masked multi-head self-attention is that during the training phase, the attention of tokens that appear after the current tokens are masked out to ensure that the model does not attend to future (unseen) tokens while generating the next token.
Then, the decoder layer uses the multi-head encoder-decoder self-attention mechanism to compute attention vectors, using the attention vectors generated by the encoder block and the matrix computed by the masked multi-head self-attention mechanism.
After the decoder block computes attention vectors at the last layer, the linear layer will convert the attention vectors to the logits vector, having length equal to the vocabulary size.
Then, the softmax function is applied to the logits vector to generate the vector, which determines the next token to be generated.
% The decoder will keep generating next token until the EOS token (i.e., “</s>”) is generated.
% The generated tokens are then 
Finally, the loss function will compare the generated \subTokApprove with the actual $sm_{approved}$ to estimate an error.

\subsection{(Step 3) Inference Phase}

After we fine-tune the CodeT5 pre-trained model, we aim to generate \mApproved from the given \mInitWithDiff in the testing dataset.
To do so, we first tokenize \mInitWithDiff to \subTokInitWithDiff by using BPE like in the training phase.
Then, we leverage beam search to generate top-$k$ best candidates of $m_{approved}$.
The beam size $k$ is a hyperparameter specifying the number of the best candidates to be generated.
In particular, after a token is generated at each time step, the beam search uses a best-first search strategy to select the top-$k$ candidates that have the highest conditional probability.
The beam search will keep generating the top-$k$ best candidates until the EOS token (i.e., ``\texttt{</s>}") is generated.

% Given the output from the softmax function, in step \circled{3}, we leverage beam search to generate multiple candidates of \mApproved at each time step based on a conditional probability.
% The number of candidates is based on the parameter called beam size $k$.
% In particular, the beam search selects top $k$ \mApproved candidates that have the highest probability using a best-first search strategy at each time step.
% The beam search will terminate when the decoder block generates the EOS token (i.e., ``\texttt{</s>}"). \kla{are you coping from somewhere? looks very familiar.}
% % \kla{last time, you said $</s>$ is the separator tag, but now EOS. So what it should exactly be?}
% % \oat{actually it should be $</s>$}


% % The embedding vector of each sub-token is then combined into a single matrix 
% % Then, our approach compute the relative posi

% % these tokens are converted to numerical vectors by 



% % Figure~\ref{fig:code-mod-identification} demonstrates how edit actions of \tokInit are obtained.
% % If tokens of both \tokCodebase and \tokInit are equal, the edit action of \tokInit is \textit{equal} (denoted by \textit{E}).
% % On the other hand, if tokens of \tokInit do not appear in \tokCodebase, the edit action of \tokInit is \textit{insert} (denoted by \textit{A}).
% % Finally, if tokens of \tokCodebase are modified, the edit action of \tokInit is \textit{modified} (denoted by \textit{M}).
% % The obtained edit action is then used as additional information to be injected to \mInit.



==> section-exp-only/Background-old.tex <==



% \section{Related Work and Research Questions} \label{sec:background}
% \section{Background \& Related Work}  \label{sec:background}
\section{Related Work and Research Questions}  \label{sec:background}

% In this section, we describe the background and related
% work to situate the paper with respect to the literature,


\begin{figure}
    \includegraphics[width=\columnwidth]{figure/LLM-for-code-review-automation-diagram.pdf}
    \caption{An overview of the modelling pipeline of LLMs for code review automation.}
    \label{fig:LLM-modeling-pipeline}
\end{figure}






In this section, we provide the background knowledge of code review automation, discuss the existing large-language model-based code review automation approaches, and formulate the research questions.
% , and LLMs for code review automation

\subsection{Code Review Automation}

% \kla{what is code review automation why do we need it?.}
% \kla{rewrite}
% code review automation tasks <need to define>

%% explain code review process in short + explain problem

Code review is a software quality assurance practice where developers other than an author (aka. reviewers) provide feedback for a code change created by the author to ensure that the code change has sufficient quality to meet quality standards.
While code review can ensure high software quality, code review is still time-consuming and expensive.
Thus, developers still face challenges in receiving timely feedback from reviewers~\cite{macleod2017code, rigby2013convergent}.
Therefore, code review automation approaches~\cite{ tufano2019learning, pornprasit2023d, li2022automating, tufano2022using, tufan2021towards} were proposed to facilitate and expedite the code review process.
% exdevelopers revising their submitted patches.

% \textit{(Oat): will fix}\\

Code review automation is generally formulated as a sequence generation task, where a language model is trained to learn the relationship between the submitted code and the revised code. 
Then, during the inference phase, the model aims to generate a revised version of a code change.
% Code review automation is generating a revised version of a patch submitted by a patch author.
% refers to automatically generating the revised version of the submitted patch.
Recently, neural machine translation (NMT)-based code review automation approaches were proposed~\cite{tufano2019learning, tufano2021towards, AutoTransform}.
Typically, NMT-based code review automation approaches are trained on a specific code review dataset. 
% Such approaches require training models from scratch to learn to translate the submitted 
% the generation of the revised version of submitted patches.
% \textit{(Oat): will fix}\\
However, prior studies~\cite{pornprasit2023d, li2022automating} found that NMT-based code review automation approaches can perform well, but is still not perfect.
This imperfect performance has to do with the limited knowledge of the NMT-based code review automation approaches that are being trained on a small code review dataset.


% such approaches have the limitation that they are only trained from a limited code review dataset.


%% then tell that based on the above problem, code review automation approaches were proposed

%% then tell that code review automation refers to ...

%% at the beginning, NMT-based code review automation approaches were proposed


%% however, the NMT-based approaches still have limitations (come up with the new one, not the existing one)


% In code review automation, a deep learning model is given code submitted for review $C_{submitted}$ (and a reviewer's comment $R_{nl}$ if available) to generate code after a change is made by a developer (i.e., a patch author) $C_{revised}$.
% Recently, neural machine translation (NMT)-based code review automation approaches were proposed~\cite{tufano2019learning, tufano2021towards, AutoTransform}.
% Such approaches require training models from scratch to learn the generation of $C_{revised}$ from given $C_{submitted}$ and $R_{nl}$.
% Thus, such approaches have the limitation that they are trained from limited knowledge of source code (i.e., a limited amount of training data)



% \begin{tabularx}{\columnwidth}{|l|l|l|}
  
% \cline{2-3} 
% \multicolumn{1}{r|}{}  & Guo~\ea~\cite{guo2023exploring} & Our work \\
%     \hline
%     Include fine-tuning LLMs? & No    & \multicolumn{1}{l|}{Yes} \\
%     \hline
%     Prompting technique & Zero-shot learning, Persona & Zero-shot learning, Few-shot learning, Persona \\
%     \hline
%     LLMs model/approach & GPT-3.5, CodeReviewer~\cite{li2022automating} & GPT-3.5, Magicoder~\cite{wei2023magicoder}, CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, D-ACT~\cite{pornprasit2023d} \\
%     \hline
%     Dataset & CodeReviewer~\cite{li2022automating}, their newly collected dataset & CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, D-ACT~\cite{pornprasit2023d} \\
%     \hline
% \end{tabularx}


\subsection{LLMs-based Code Review Automation Approaches}

Large language models (LLMs) for code review automation refer to large language models specifically designed to support code review automation tasks, aiming to understand and generate source code written by developers and natural languages written by reviewers. 
Since source code and comments often have their own semantic and syntactical structures, recent work proposed various LLMs-based code review automation approaches~\cite{li2022automating, tufano2022using, 
 llamareviewer}. 
For example, Li~\ea~\cite{li2022automating} proposed CodeReviewer, a pre-trained LLM that is based on the CodeT5 model~\cite{wang2021codet5}.
Prior studies found that LLMs-based code review automation approaches often outperform NMT-based ones~\cite{pornprasit2023d, li2022automating, tufano2022using}.
For example, Li~\ea~\cite{li2022automating} found that their proposed approach outperforms a transformer-based NMT model by 11.76\%.
% For example, Pornprasit~\ea~\cite{pornprasit2023d} found that their proposed approach outperforms a transformer-based NMT model by at least 1,100\%.
% due to the benefits of pre-training model on the pre-training tasks specific to code review.
Below, we briefly discuss the general modelling pipeline of LLMs for code review automation presented in Figure~\ref{fig:LLM-modeling-pipeline}.

\textbf{Model Pre-Training} refers to the initial phase of training a large language model, where the model is exposed to a large amount of unlabeled data to learn general language representations.
This phase aims to initialize the model's parameters and learn generic features that can be further fine-tuned for specific downstream tasks.
Recently, there have been many large language models for code (i.e., LLMs that are specifically trained on source code and related natural languages).
For example, the open-source community-developed large language models such as Code-LLaMa~\cite{roziere2023codeLLaMa}, StarCoder~\cite{li2023starcoder}, and Magicoder~\cite{wei2023magicoder}; and the commercial large language models such as GPT-3.5.





However, the development of large language models for code requires expensive GPU resources and budget. 
For example, GPT-3.5 requires 10,000 NVIDIA V-100 GPUs for model pre-training.\footnote{https://gaming.lenovo.com/emea/threads/17314-The-hardware-behind-ChatGPT} 
LLaMa2~\cite{touvron2023llama2} requires Meta’s Research Super Cluster (RSC) as well as internal production clusters, which consists of approximately 2,000 NVIDIA A-100 GPUs in total.
Therefore, many software organizations with limited resources and budgets may not be able to develop their large language models.
Thus, fine-tuning and prompt engineering are the two common approaches to leverage the existing LLMs for code review automation when expensive GPU resources are not available for pre-training a large language model from scratch, where these techniques are more desirable for many organizations to quickly adopt new technologies.

% Model pre-training is the first step to build an LLM.
% In this step, an LLM is pre-trained to learn the representation of the next token from the previous tokens~\cite{achiam2023gpt, touvron2023llama, touvron2023llama2, chowdhery2023palm, anil2023palm2, hoffmann2022training}.
% Generally, LLMs are pre-trained on large natural text in different domains and source code corpus.


% \textbf{Model Fine-Tuning} refers to the further phase of training a large language model where a pre-trained language model is further trained on a specific task or dataset to adapt its parameters to perform better on that task. 
% Fine-tuning is a common practice, particularly in transfer learning scenarios, where a model pre-trained on a large dataset (source domain, e.g., source code understanding) is adapted to a related but different task or dataset (target domain, e.g., code review automation).
\textbf{Model Fine-Tuning} is a common practice, particularly in transfer learning scenarios, where a model pre-trained on a large dataset (source domain, e.g., source code understanding) is adapted to a related but different task or dataset (target domain, e.g., code review automation).
Recently, researchers have leveraged model fine-tuning techniques for LLMs to improve the performance of code review automation approaches.
For example, Lu~\ea~\cite{llamareviewer} proposed LLaMa-Reviewer, which is an LLM-based code review automation approach that is being fine-tuned on a base LLaMa model~\cite{touvron2023llama} using three code review automation tasks, i.e., a review necessity prediction task to check if diff hunks need a review, a code review comment generation task to generates pertinent comments for a given code snippet, and a code refinement task to generate minor adjustment to the existing code.
Lu~\ea~\cite{llamareviewer} found that the fine-tuning step on LLMs can greatly improve the performance of the existing code review automation approaches. 


% based on the pre-trained LLaMa model~\cite{touvron2023llama}.
% that is fine-tuned by using a parameter-efficient fine-tuning technique called LoRA~\cite{hu2021lora}.
% They showed that their proposed LLaMa-reviewer spend less time to train when compared to other LLMs for code review automation~\cite{raffel2020exploring, tufano2022using}.

\textbf{Inference} refers to the process of using a pre-trained language model to generate source code based on a given natural language prompt instruction.
Therefore, prompt engineering plays an important role in leveraging LLMs for code review automation to guide LLMs to generate the desired output. 
Different prompting strategies have been proposed.\footnote{https://www.promptingguide.ai/}
For example, zero-shot learning, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger}, chain-of-thought~\cite{kim2023cot, wei2022chain}, tree-of-thought~\cite{kim2023cot, wei2022chain}, self-consistency~\cite{wang2022self}, and persona~\cite{white2023prompt}.
% Recently, several studies 
Nevertheless, not all prompting strategies are relevant to code review automation.
For example, chain-of-thought, self-consistency and tree-of-thought promptings are not applicable to the code review automation task since they are designed for arithmetic and logical reasoning problems.
Thus, we exclude them from our study.

In contrast, zero-shot learning, few-shot learning, and persona prompting are the instruction-based prompting strategies, which are more suitable for software engineering (including code review automation) tasks~\cite{xu2023prompting, dilhara2024unprecedented, misu2024towards, jiang2023llmparser}.
In particular, zero-shot learning involves prompting LLMs to generate an output from a given instruction and an input.
% On the other hand, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} involves prompting LLMs to generate an output from a few or more examples of an input/output pair \kla{this is mentioned everywhere, but no proper definition} and an input.
On the other hand, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} involves prompting LLMs to generate an output from $N$ demonstration examples $\{(x_1, y_1), (x_2, y_2), ..., (x_N, y_N)\}$ and an actual input in a testing set, where $x_i$ and $y_i$ are the inputs and outputs obtained from a training set, respectively.
Persona~\cite{white2023prompt} involves prompting LLMs to act as a specific role or persona to ensure that LLMs will generate output that is similar to the output generated by a specified persona.
% We include a persona in an input prompt to ensure that LLMs will generate output that is similar to the output generated by a specified persona.
% The purpose \kla{whose puprose? your purpose or LLMs's purpose or OpenAI's purpose? I don't get this part.} of including a persona in an input prompt is to ensure that LLMs will generate output that is similar to the output generated by a specified persona.




% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The differences between our work and Guo~\ea's work~\cite{guo2023exploring}.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{0.15\textwidth}|p{0.2\textwidth}|p{0.2\textwidth}|}
\cline{2-3} \multicolumn{1}{r|}{}  & Guo~\ea~\cite{guo2023exploring} & Our work \\
    \hline
    LLMs/approaches & GPT-3.5, CodeReviewer~\cite{li2022automating} & GPT-3.5, Magicoder~\cite{wei2023magicoder}, CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, D-ACT~\cite{pornprasit2023d} \\
    \hline
    % Dataset & CodeReviewer~\cite{li2022automating}, their newly collected dataset & CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, D-ACT~\cite{pornprasit2023d} \\
    % \hline
    Include fine-tuning LLMs? & No    & \multicolumn{1}{l|}{Yes} \\
    \hline
    Prompting techniques & Zero-shot learning, Persona & Zero-shot learning, Few-shot learning, Persona \\
    \hline
    
    \end{tabular}%
    }
  \label{tab:work-comparison}%
\end{table}%


\subsection{GPT-3.5 for Code Review Automation}

% Recently, Guo~\ea~\cite{guo2023exploring} investigated the performance of GPT-3.5 on the code review automation task.
Recently, Guo~\ea~\cite{guo2023exploring} conducted an empirical study to investigate the potential of GPT-3.5 for code review automation.
% In their study, they evaluate the performance of zero-shot ChatGPT with a state-of-the-art code review automation approach (i.e., CodeReviewer~\cite{li2022automating}).
% They showed that zero-shot GPT-3.5 outperforms the existing code review automation approach (i.e., CodeReviewer~\cite{li2022automating}).
% However, there are other approaches to leverage GPT-3.5 (i.e., model fine-tuning and few-shot learning) and code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}) that are not included in their study.
However, the results of their study are still limited to GPT-3.5 when using zero-shot learning, and the CodeReviewer approach~\cite{li2022automating}.
Thus, their study still has the following limitations.
% However, the results of their study are still not conclusive for the following three reasons.
% However, as shown in Table~\ref{tab:work-comparison}, their study is still not conclusive due to the following reasons.

% \textbf{First, Guo~\ea~\cite{guo2023exploring} only conducted experiments with GPT-3.5 and the CodeReviewer approach~\cite{li2022automating} on the CodeReviewer dataset~\cite{li2022automating} and their collected dataset (i.e., the CRN dataset, which is extended from the CodeReviewer dataset~\cite{li2022automating}).}
\textbf{First, Guo~\ea~\cite{guo2023exploring} only conducted experiments with GPT-3.5 and the CodeReviewer approach~\cite{li2022automating}.}
However, there are other code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}) 
% and other code review automation datasets~\cite{pornprasit2023d, tufano2022using}
that are not included in their study (see Table~\ref{tab:work-comparison}). 
% However, Table~\ref{tab:work-comparison} shows that there are other code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}) and other code review automation datasets~\cite{pornprasit2023d, tufano2022using} that are not included in their study. 
% Therefore, practitioners still do not know which LLM for code review automation they should use since
The lack of a systematic evaluation of GPT-3.5 with other code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}) makes it difficult for practitioners to conclude which LLMs for code review automation perform best.
% Therefore practitioners still do not know which LLMs for code review automation perform best.
To address this challenge, we formulate the following research question.

% \RQbox{1, \rqone}

\begin{tcolorbox}[left=2pt, right=2pt, top=2pt,bottom=2pt]
RQ1: \rqone
\end{tcolorbox}


% \textbf{Second, prior studies~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating} found that model fine-tuning can improve the performance of pre-trained LLMs.}
% However, Guo~\ea~\cite{guo2023exploring} did not evaluate the performance of LLMs when being fine-tuned (see Table~\ref{tab:work-comparison}).
\textbf{Second, the performance of LLMs when being fine-tuned is still unknown.}
In particular, Guo~\ea~\cite{guo2023exploring} did not evaluate the performance of LLMs when being fine-tuned.
However, prior studies~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating} found that model fine-tuning can improve the performance of pre-trained LLMs.
The lack of experiments with model fine-tuning makes it difficult for practitioners to conclude whether LLMs for code review automation should be fine-tuned to achieve the most effective results.
% Therefore, practitioners still do not know whether LLMs for code review automation should be fine-tuned to achieve the most effective results.
To address this challenge, we formulate the following research question.

% in Table~\ref{tab:work-comparison} shows that Guo~\ea~\cite{guo2023exploring} did not include model fine-tuning in their experiment.
% Indeed, fine-tuning LLMs requires more resources (e.g., time and budget) than using LLMs without fine-tuning.
% However, due to a lack of experiments with model fine-tuning, practitioners still do not know whether LLMs for code review automation should be fine-tuned to achieve the most effective results.
% it is worth fine-tuning LLMs for code review automation to achieve the highest performance.
% Thus, little is known whether it is worth investing in fine-tuning LLMs for code review automation.
    % Therefore, in this RQ, we evaluate the performance of fine-tuned LLMs and LLMs that are not fine-tuned.


% \RQbox{2, \rqtwo}

\begin{tcolorbox}[left=2pt, right=2pt, top=2pt,bottom=2pt]
RQ2: \rqtwo
\end{tcolorbox}


% \textbf{Third, prior work~\cite{brown2020language, kang2023large, geng2024large} found that using prompts containing demonstration examples and an instruction (aka few-shot learning) could improve the performance of LLMs over using prompts containing only an instruction (aka zero-shot learning).}
% However, Guo~\ea~\cite{guo2023exploring} did not investigate the impact of few-shot learning on LLMs for code review automation (see Table~\ref{tab:work-comparison}).
\textbf{Third, the performance of LLMs for code review automation when using few-shot learning is still unknown.}
% \textbf{Third, the most effective prompting strategy for code review automation is still unknown.}
In particular, Guo~\ea~\cite{guo2023exploring} did not investigate the impact of few-shot learning on LLMs for code review automation.
However, recent work~\cite{brown2020language, kang2023large, geng2024large} found that few-shot learning could improve the performance of LLMs over zero-shot learning.
% using prompts containing demonstration examples and an instruction (aka few-shot learning) could improve the performance of LLMs over using prompts containing only an instruction (aka zero-shot learning).
The lack of experiments with few-shot learning on LLMs for code review automation makes it difficult for practitioners to conclude which prompting strategy (i.e., zero-shot learning, few-shot learning, and persona) is the most effective for code review automation.
% the study of Guo~\ea~\cite{guo2023exploring} still lacks the evaluation with few-shot learning on LLMs for code review automation(see Table~\ref{tab:work-comparison}), making it difficult for practitioners to know which prompting strategy (i.e., zero-shot learning, few-shot learning, and persona) is the most effective for code review automation.
% Thus, practitioners still do not know which prompting strategy (i.e., zero-shot learning, few-shot learning, and persona) is the most effective for code review automation.
To address this challenge, we formulate the following research question.

% \RQbox{3, \rqthree}

\begin{tcolorbox}[left=2pt, right=2pt, top=2pt,bottom=2pt]
RQ3: \rqthree
\end{tcolorbox}

% First, as shown in Table~\ref{tab:work-comparison}, their study did not investigate the other recent code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}).
% In addition, their study is limited to the CodeReviewer dataset~\cite{li2022automating} and their newly collected dataset.


% the impact of model fine-tuning on LLMs.
% In addition, their study lacks evaluation with the other recent code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}) on the other code review automation datasets~\cite{pornprasit2023d, tufano2022using}.

% First, their study lacks evaluation with model fine-tuning and other prompting techniques (e.g., few-shot learning) on LLMs.
% Second, their study lacks evaluation with other recent code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}).
% Third, their study is limited to the CodeReviewer~\cite{li2022automating} and their newly collected dataset.
% Therefore, practitioners still do not know which LLM for code review automation performs best, or which prompting technique is the most effective for code review automation.



% However, their study is still not comprehensive due to the following two reasons.
% First, their study lacks evaluation with other recent code review automation approaches (i.e., D-ACT~\cite{pornprasit2023d} and TufanoT5~\cite{tufano2022using}).
% Second, their study lacks evaluation with other prompting techniques (e.g., few-shot learning) and model fine-tuning on LLMs.

% \textit{Oat: I think I will explain the difference between their work and our work here, then explain problems of their work in the motivation of RQ1}\\
% Different from their work, our work aims to investigate the performance of recently proposed LLMs for code review automation (i.e., CodeReviewer~\cite{li2022automating}, D-ACT~\cite{pornprasit2023d}, and TufanoT5~\cite{tufano2022using}), and the impact of model fine-tuning and prompting techniques (i.e., zero-shot learning, few-shot learning and persona) on GPT-3.5 and Magicoder.

% and compared it with the state-of-the-art code review automation (i.e., CodeReviewer) under two different code review datasets, i.e., the original version of the CodeReviewer dataset and the extended version of the CodeReviewer dataset.







% how well ChatGPT performs in code review tasks. To fill this gap, in this paper, we conduct the first empirical study to understand the capabilities of ChatGPT in code review tasks, specifically focusing on automated code refinement based on given code reviews. To conduct the study, we select the existing benchmark CodeReview and construct a new code review dataset with high quality. We use CodeReviewer, a state-of-the-art code review tool, as a baseline for comparison with ChatGPT. Our results show that ChatGPT outperforms CodeReviewer in code refinement tasks. Specifically, our results show that ChatGPT achieves higher EM and BLEU scores of 22.78 and 76.44 respectively, while the state-of-the-art method achieves only 15.50 and 62.88 on a high-quality code review dataset. We further identify the root causes for ChatGPT’s underperformance and propose several strategies to mitigate these challenges. Our study provides insights into the potential of ChatGPT in automating the code review process, and highlights the potential research directions.




% leveraged the zero-shot prompting technique for code review automation.
% In particular, they show that their proposed prompt, which contains an instruction and scenario description, can outperform CodeReviewer~\cite{li2022automating} on their newly collected dataset.
% \kla{todo}

% - zero-shot not outperform CodeReviewer model based on code reviewer dataset
% - zero-shot outperform CodeReviewer model based on their new dataset (extended dataset, other PL)

% code review automation does not involve following intermediate steps to generate $C_{revised}$ from the given $C_{submitted}$ and $R_{nl}$.\kla{ I don't get it. revise it again. I don't follow your reasoning logic!}

% \kla{what is, why others are not relevant, but we focus on zero,few,persona}


% After LLMs are pre-trained or fine-tuned, they can be used to generate responses by using prompting techniques.
% We explain an overview of the following prompting techniques below.

% \begin{itemize}
%     \item Zero-shot learning involves prompting LLMs to generate an output from a given instruction and an input.
    

%     \item In-context learning (ICL)~\cite{brown2020language, liu2021makes, wei2023larger} involves prompting LLMs to generate an output from example input/output pairs and an input.
    

%     \item Chain-of-thought (CoT)~\cite{kim2023cot, wei2022chain} involves prompting LLMs to follow steps or rationale to generate an output from a given input.
    

%     \item Tree-of-thought (ToT)~\cite{yao2024tree} involves prompting LLMs to explore multiple reasoning paths to select the best path for generating a final output.

%     \item Self-consistency (SC)~\cite{wang2022self} involves prompting LLMs to follow steps or rationale to generate multiple outputs from a given input.
%     The final generated output is then selected from majority voting.

%     \item Persona~\cite{white2023prompt} involves prompting LLMs to act as a specific role or persona.
%     The purpose of including persona in an input prompt is to ensure that LLMs will generate output that is similar to the output generated by a specified persona.
% \end{itemize}



%% just my outline
% consists of 3 main steps
% - pre-train
%     - train model to ...
%     - how to train: use ... tasks and train on large datasets
% - fine-tune
%     - fine-tune pre-trained model for downstream tasks
% - inference
%     - use LLM to generate text
%     - there are different ways to do inference
%         - 0-shot, in-context, ... (explain meaning of each one)

% \kla{have you talked about what is LLM before talking about the pipeline?}


% Large language models (LLMs)~\cite{ touvron2023llama2, achiam2023gpt, workshop2022bloom} are large deep learning models that are based on the transformer architecture~\cite{Vaswani2017} and pre-trained on massive datasets.\kla{is this sentence about LLM modelling? T-T Just a basic writing Oat! you just read your section title}
% Recently, researchers proposed LLMs for code~\cite{roziere2023codeLLaMa, li2023starcoder, wei2023magicoder}.

% Generally, an LLM modeling pipeline consists of the following steps


% Model pre-training are classified in the following categories:

% \begin{itemize}
%     \item Pre-training encoder-only LLMs~\cite{devlin2018bert}:
%     Generally, encoder-only LLMs are pre-trained with the masked language modeling (MLM) task (i.e., predicting the masked tokens).
%     The goal of this task is to train an LLM to learn the representation of masked tokens from their surrounding tokens. 


%     \item Pre-training decoder-only LLMs~\cite{achiam2023gpt, touvron2023llama, touvron2023llama2, chowdhery2023palm, anil2023palm2, hoffmann2022training}:
%     Decoder-only LLMs are pre-trained with the next-token prediction task (i.e., predicting the next token from the previous tokens).
%     The goal of this task is to train an LLM to learn the representation of next token from the previous tokens.
    
    
%     \item Pre-training encoder-decoder LLMs~\cite{raffel2020exploring, xue2020mt5, lewis2020bart}:
%     The LLMs in this category are pre-trained on both encoder and decoder parts.
%     Recent work propose different approaches for pre-training such LLMs.
%     For example, Raffel~\ea~\cite{raffel2020exploring} pre-trained the text-to-text transformer ... .
    
% \end{itemize}





% \subsection{LLMs for Code Review Automation}

%% just my outline
% - recent work proposed different pre-trained LLM (TufanoT5, CodeReviewer)
% - there is 1 work that fine-tune open-source LLM for this task
% - there is 1 work that explores prompting method in GPT-3.5


% Recently, pre-trained LLMs for code review automation were proposed.
% In particular, Li~\ea~\cite{li2022automating} proposed CodeReviewer, a pre-trained LLM that is based on the CodeT5~\cite{wang2021codet5} model.
% CodeReviewer is pre-trained with the training tasks specific to code review.
% In addition, Tufano~\cite{tufano2022using} presented a pre-trained LLM that is based on the T5~\cite{raffel2020exploring} architecture.
% Their LLM is pre-trained with natural languages and source code.

% Prior work~\cite{llamareviewer} proposed LLaMa-reviewer, a pre-trained LLaMa model~\cite{touvron2023llama} that is fine-tuned by using a parameter-efficient fine-tuning technique called LoRA~\cite{hu2021lora}.
% Lu~\ea~\cite{llamareviewer} showed that their proposed LLaMa-reviewer spend less time to train when compared to other LLMs for code review automation~\cite{raffel2020exploring, tufano2022using}.


% Previously, Guo~\ea~\cite{guo2023exploring} conducted experiments with GPT-3.5 to find the best combination of a prompt and a hyper-parameter (i.e., temperature) for code review automation task.
% \kla{if you say this, then why do we need your work :( it is exactly the same as this sentence. }
% However, their study only explores zero-shot prompting.

==> section-exp-only/Experiment.tex <==

% \begin{table*}[h]
%   \centering
%   \caption{(RQ1) The evaluation results of GPT-3.5 when zero-shot learning and few-shot learning is performed.}
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
% \cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
%     \hline
%     \ChatGPTZeroShot & 17.72\% & 44.17\% & 13.52\% & 78.36\% & 2.62\% & 74.92\% & 0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\
%     \hline
%     \ChatGPTFewShot  & \textbf{26.55\%} & \textbf{47.50\%} & 19.79\% & \textbf{81.47\%} & 8.96\% & \textbf{79.21\%} & \textbf{2.34\%} & \textbf{75.33\%} & \textbf{2.89\%} & \textbf{81.40\%} & 1.64\% & \textbf{73.83\%} \\
%     \hline
%     \end{tabular}%
%   }
%   \label{tab:rq1-result}%
% \end{table*}%





% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ1.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ1-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ1.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\tufanoData~dataset (with comment)}
%          \label{fig:RQ1-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ1.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ1-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ1.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ1-EM-intersection-D-ACT}
%      \end{subfigure}
     
%     \caption{(RQ1) Venn diagrams showing EM achieved by \ChatGPTZeroShot~and \ChatGPTFewShot.}
%     \label{fig:RQ1-EM-intersection}
% \end{figure*}



\section{Experiment Setup} \label{sec:exp_design}

\begin{table*}
  \centering
  % \caption{An overview statistic of the studied datasets (the Android, Google and Ovirt projects are obtained from~\cite{pornprasit2023d}).}
  \caption{A statistic of the studied datasets (the dataset of Android, Google and Ovirt are from \DACTData~\cite{pornprasit2023d}).}
%   \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
\hline   Dataset  & \# Train & \# Validation & \# Test & \# Language & Granularity & Has Comment\\
    \hline
    % \CodeReviewerDataNew~\cite{guo2023exploring} & - & - & 14,945\footnote{The number is from the dataset provided in replication package} \\
    \CodeReviewerData~\cite{li2022automating} & 150,405 & 13,102 & 13,104 & 9 & Diff Hunk & Yes\\
    \tufanoData~\cite{tufano2022using} & 134,238 & 16,779 & 16,779 & 1 & Function & Yes/No\\
    Android~\cite{pornprasit2023d} & 14,690 & 1,836 & 1,835 & 1 & Function & No\\
    Google~\cite{pornprasit2023d} & 9,899 & 1,237 & 1,235 & 1 & Function & No\\
    Ovirt~\cite{pornprasit2023d}  & 21,509 & 2,686 & 2,688 & 1 & Function & No\\
    % Gerrit & 3,144 & 544 & 370 \\
    \hline
    \end{tabular}%
    % }
  \label{tab:dataset}%
\end{table*}%



In this section, we explain the detail of the datasets, hyper-parameter setting of GPT-3.5, and evaluation measures in our experiment.

% \subsection{Dataset}


%     In this study, we use the following datasets which are summarized in Table~\ref{tab:dataset}: \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and Code\-Reviewer\textsubscript{data}~\cite{li2022automating}.
%     % \CodeReviewerData~\cite{li2022automating}.
%     We describe the details of these datasets below.

%     %  \textbf{\CodeReviewerDataNew}: Guo~\ea~\cite{guo2023exploring} collected the dataset from GitHub pull requests that appear after January 1, 2022.
%     % The pull requests are obtained from the repositories in \CodeReviewerData~dataset and new repositories that have different programming languages (e.g., SQL and Perl) with the repositories in  \CodeReviewerData~dataset

%     \begin{itemize}
%         \item \textbf{\CodeReviewerData}: Li~\ea~\cite{li2022automating} collected this dataset from the GitHub projects across nine programming languages (i.e., C, C++, C\#, Java, Python, Ruby, php, Go, and Javascript).
%     % that contain at least 1,500 pull requests.
%     % The dataset contains the following information.
%         The dataset contains triplets of the current version of code (diff hunk granularity), the reviewers' comment, and the revised version of code (diff hunk granularity).
        
%         \item \textbf{\tufanoData}: Tufano~\ea~\cite{tufano2022using} collected this dataset from Java projects in GitHub containing at least 50 pull requests, and 6,388 Java projects hosted in Gerrit.
%         Each record in the dataset contains a triplet of code submitted for review (function granularity), a reviewer's comment, and code after being revised (function granularity).
%         Tufano~\ea~\cite{tufano2022using} created two types of this dataset (i.e., Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment)).
        
%         \item  \textbf{\DACTData}: Pornprasit~\ea~\cite{pornprasit2023d} collected this dataset from the three Java projects hosted on Gerrit (i.e., Android, Google and Ovirt).
%         Each record in the dataset contains a triplet of codebase (function granularity), code of the first version of a patch (function granularity), and code of the approved version of a patch (function granularity).
%     \end{itemize}






\subsection{Hyper-Parameter Setting}

    In this study, we use the following hyper-parameter settings when using GPT-3.5 to generate improved code: temperature of 0.0 (as suggested by Guo~\ea~\cite{guo2023exploring}), top\_p of 1.0 (default value), and max length of 512.
    For model fine-tuning, we use hyper-parameters  (e.g., number of epochs and learning rate) that are automatically provided by OpenAI API.
    % we rely on the OpenAI API to select suitable hyper-parameters (e.g., number of epochs and learning rate).



    
\subsection{Evaluation Measure}
    
    % We evaluate the generated refined code in the code refinement tasks by using the following measures:
    % We use the following evaluation measures in our experiment:

    % \begin{enumerate}
    %     % \item \textbf{Exact Match (EM)}~\cite{tufano2019learning, pornprasit2023d} is the number of generated code that is exactly the same as the actual code (i.e., the code in ground-truth).
    %     \item \textbf{Exact Match (EM)}~\cite{li2022automating, pornprasit2023d, tufano2019learning} is the number of the generated improved code that is the same as the actual improved code in the testing dataset.
    %     We use this measure since it is widely used for evaluating code review automation approaches~\cite{tufano2022using, pornprasit2023d,tufano2019learning}.
    %     To compare the generated improved code with the actual improved code, we first tokenize both improved code to sequences of tokens.
    %     Then, we compared the sequence of tokens of the generated improved code with the sequence of tokens of the actual improved code.
    %     % The higher EM, the better a model to generate code that is exactly the same as the actual code
    %     A high value of EM indicates that a model can generate improved code that is the same as the actual improved code in the testing dataset.
        
    %     % \item \textbf{Edit Progress (EP)}~\cite{zhou2023EditProgress} measures the progress that is made to generate code that is exactly the same as the actual code in historical review records.
    %     % Given the input code $\tilde{C}$, the actual code $\bar{C}$ and the generated code $\hat{C}$, the Edit Progress metric can be calculated by the following equation:
    
    %     % $$\text{Edit Progress} = \frac{\left| D_{\tilde{C} \longrightarrow \bar{C}}\right| - \left| D_{\hat{C} \longrightarrow \bar{C}}\right|}{\left| D_{\tilde{C} \longrightarrow \bar{C}}\right|}$$
        
    %     % where $D$ is the Levenshtein distance~\cite{levenshtein1966binary}
    %     % % The higher EP, the better a model to make progress towards generating code that looks exactly the same as the actual code.
    %     % \bigskip
        
    %     % A positive value of EP indicates that a model is making progress towards generating code that looks exactly the same as the actual code in historical review records.
    %     % In contrast, a negative value of EP indicates that a model makes more mistakes than making progress.

    %     \item \textbf{CodeBLEU}~\cite{ren2020codebleu} is the extended version of BLEU (i.e., an n-gram overlap between the translation generated by a deep learning model and the translation in ground tr\-uth)~\cite{bleu} for automatic evaluation of the generated code.
    %     We do not measure BLEU like in prior work~\cite{tufano2022using, li2022automating} since Ren~\ea~\cite{ren2020codebleu} found that this measure ignores syntactic and semantic correctness of the generated code.
    %     In addition to BLEU, CodeBLEU considers the weighted n-gram match, matched syntactic information (i.e., abstract syntax tree: AST) and matched semantic information (i.e., data flow: DF) when computing the similarity between the generated improved code and the actual improved code.
    %     % CodeBLEU can be calculated by the following equation:
    %     % % \begin{multline}
    %     %     % \nonumber
    %     % \footnotesize
    %     % $$\text{CodeBLEU} = \alpha \cdot \text{BLEU} + \beta \cdot \text{BLEU\textsubscript{weight}} + 
    %     % \gamma \cdot \text{Match\textsubscript{AST}} + \delta \cdot \text{Match\textsubscript{DF}}$$
    %     % % \end{multline}      
    %     % \normalsize
    %     % The higher CodeBLEU, the better a model to generate code that is syntactically and semantically similar to the actual code.
    %     A high value of CodeBLEU indicates that a model can generate improved code that is syntactically and semantically similar to the actual improved code in the testing dataset.

    % \end{enumerate}


% \subsection{Experimental Environment}

%     We conduct the experiment in the server equipped with the following hardware: an AMD Ryzen 9 5950X @3.4 GHz 16-Core CPU, an SSD of 1 Terabyte, a RAM of 64 Gigabyte, and an NVIDIA GeForce RTX 3090 GPU with 24 GB memory.





% \subsection{Research Questions}

%     In this study, we formulate the following two research questions.
    
%     % RQ1: Li et. al เป็นคนแรกที่เสนอ task นี้ และแสดงให้เห็นว่า pre-trained model ทำ task นี้ได้ แต่ว่ายังไม่มีงานไหนที่เอา LLM ทำกับ task นี้ ดังนั้นเราเลยทำ
    
%     \textbf{RQ1: \rqI}
    
%     \textbf{Motivation.}
%     Recently, Guo~\ea~\cite{guo2023exploring} conducted an empirical study to explore the potential of using \chatGPT~for code refinement task, which is limited by only the approach and dataset presented in~\cite{li2022automating}.
%     However, there exist other code refinement approaches and datasets that are not explored in their study.
%     Thus, there is still doubt about how \chatGPT~perform when compared to other existing code refinement approaches in other datasets.
%     To address this issue, we formulate this RQ to investigate the performance of \chatGPT~and the existing code refinement approaches on other code refinement datasets.


    
%     % - งานก่อนหน้าวัด performance ของ model โดยใช้ exact match กับ BLEU ซึ่ง measure พวกนี้ไม่ได้เหมาะสำหรับการทำ evaluation กับ code transformation เท่าไหร่
%     % - ... et. al~\cite{winter2022developers} บอกว่าจริงๆแล้วมันยังต้องใช้คนในการประเมินผลที่ได้จาก deep learning-based tool อยู่ดี ดังนั้นเราควรดู measure อื่นที่บ่งบอก improvement ของ result ที่ได้จาก tool/approach ด้วย
%     % - ... et. al~\cite{ren2020codebleu} บอกว่าไม่ควรใช้ BLEU เพราะว่ามัน ignore the
%     % syntactic and semantic of generated source code. ดังนั้นก็เลยไม่เหมาะกับการทำ evaluation สำหรับ code synthesis
%     % - ดังนั้นเราเลยทำ evaluation กับ ChatGPT และ code transformation approach โดยใช้ measure อื่นๆเพิ่มเติมนอกจาก exact match

%     % old one 2 (not directly relate to RQ)
%     % Previous work~\cite{tufano2022using, tufan2021towards, li2022automating} evaluate the performance of code refinement approaches by using exact match and BLEU~\cite{bleu} as measurements.
%     % % However, Winter~\ea~\cite{winter2022developers} found that human decisions are still needed when applying the recommendations generated by automated tools.
%     % % Thus, we should not rely on the exact match measure when evaluating code transformation approaches~\cite{zhou2023generation}.
%     % However, we should not rely on the exact match measure when evaluating code refinement approaches~\cite{zhou2023generation} since Winter~\ea~\cite{winter2022developers} found that human decisions are still needed when applying the recommendations generated by automated tools.
%     % In addition, Ren~\ea~\cite{ren2020codebleu} argued that BLEU~\cite{bleu} should not be used to evaluate code synthesis approaches since this measure ignores the syntactic and semantics of generated code, which do not present in natural language.
%     % Therefore, we formulate this RQ to investigate the performance of ChatGPT compared to the performance of the existing code refinement approaches by using additional measurements that are suitable for code refinement task.

%     %% old one (still not exciting)
%     % Previous work shows that using few-shot learning with LLMs, which are more complex than pre-trained code models (e.g., CodeT5~\cite{wang2021codet5}), can outperform the existing approaches that are built on pre-trained code models in various SE tasks~\cite{xia2023automated, geng2024large, ahmed2022few}.
%     % For example, Xia~\ea~\cite{xia2023automated} show that using few-shot learning with Codex~\cite{chen2021evaluating} can outperform the existing state-of-the-art automated program repair approaches.
%     % However, little is known whether using few-shot learning with LLMs (e.g., ChatGPT) can outperform the existing approaches~\cite{tufano2022using, pornprasit2023d, li2022automating} for transforming the first version of a patch to the version that reviewers are likely approved.
%     % Thus, we formulate this RQ to investigate the performance of LLMs compared to the performance of such approaches.

    
%     %%% old one (not exciting)
%     % LLMs are more complex that the pre-trained code models (e.g., CodeBERT~\cite{codebert} or CodeT5~\cite{ wang2021codet5}) due to having more parameters.
%     % Previous studies show that LLMs (e.g., ChatGPT) can be used for software engineering tasks such as automated program repair~\cite{fan2023automated, xia2023automated}.
%     % However, little is known about how well LLMs perform when transforming the first version of a patch to the version that reviewers are likely to approve.
%     % Thus, we formulate this RQ to evaluate the performance of LLMs with the existing code transformation approaches~\cite{tufano2022using, pornprasit2023d, li2022automating}
    
%     % RQ2: งานก่อนหน้าแสดงให้เห็นว่า LLM ใช้กับ code -> text task อย่างเช่น code summarization task [Automatic Code Summarization via ChatGPT: How Far Are We?] แต่ว่ายังไม่มีงานไหนที่ทำ empirical study เกี่ยวกับการสร้าง review comment
    
%     \textbf{RQ2: \rqII}

% %     		○ การทำ evaluation ใน RQ1 นี่ทำกับ test set ที่เอามาจาก historical review record
% % 		○ แต่ว่า code ใน historical review record อาจจะยังมีคุณภาพไม่ดีสุดด้วยเหตุผลหลายอย่าง (อย่างเช่น reviewer ดูแค่ error ที่เห็นได้ชัดเจน) ดังนั้น recommendation อันที่ LLM สร้างมาไม่ตรงกับ ground truth ใน test set อาจจะมีประโยชน์กับ developer ก็ได้
% % ดังนั้นเราเลยทำ survey study เพื่อดูว่า recommendation ที่ได้จาก LLM พวกนี้มันจะมีประโยชน์กับ developer มากน้อยแค่ไหนและ developer มี willingness to adapt recommendation มากน้อยแค่ไหน

%     % sridhara2023chatgpt
%     \textbf{Motivation.}
%     The evaluation of previous work~\cite{tufano2022using, pornprasit2023d, li2022automating, guo2023exploring}  only relies on the patches in the historical review records.
%     However, alternative recommendations should also be considered when evaluating code refinement approaches since Bacchelli~\ea~\cite{bacchelli2013expectations} find that developers do code review to find alternative solutions (e.g., better implementation).
%     % In RQ1, we use the approved patches in the historical review records to conduct the experiment.
%     % In RQ1, we evaluate how well the existing code refinement approaches~\cite{tufano2022using, pornprasit2023d, li2022automating} perform when learning from the training dataset of the historical review records.
%     % Previous work~\cite{tufano2022using, pornprasit2023d, li2022automating} evaluate how well code refinement approaches perform when learning from the training dataset of the historical review records.
%     % However, in real practice, Bacchelli~\ea~\cite{bacchelli2013expectations} find that developers do code review to find alternative solutions (e.g., better implementation).
%     % The closest work related to generating alternative recommendation is from Sridhara~\ea~\cite{sridhara2023chatgpt}, showing that ChatGPT could potentially be used to provide recommendations to developers in code review.
%     % Recently, Sridhara~\ea~\cite{sridhara2023chatgpt} showed that LLM (i.e., ChatGPT) could potentially be used to provide recommendations to developers in code review.
%     % However, little is known about how developers perceive the recommendations generated by \chatGPT.
%     Thus, we formulate this RQ to investigate the perception of developers on the alternative recommendations generated by \chatGPT.

%     %%% old one (not ok because lack of supporting evidence + blame developers
%     % In RQ1, we use the approved patches in the historical review records for evaluation.
%     % evaluate the performance by using  with the test set collected from the historical review records.
%     % However, such patches may not have the highest quality since reviewers provide comments that are irrelevant to code improvement~\cite{bosu2015characteristics}.
%     % Thus, alternative recommendations might be considered since they might be useful for practitioners. 
%     % Therefore, we formulate this RQ to evaluate the degree of usefulness and willingness to adapt the alternative recommendations that are generated by LLMs.



% % \subsection{Hyper-parameter Setting}
% % We use the same hyper-parameter as reported in~\cite{pornprasit2023D-ACT, li2022codereviewer} to train and evaluate D-ACT and CodeReviewer models.
% % For ChatGPT, we use default parameter to generate refined methods.


% \begin{table}[t]
%   \centering
%   % \caption{An overview statistic of the studied datasets (the Android, Google and Ovirt projects are obtained from~\cite{pornprasit2023d}).}
%   \caption{An overview statistic of the studied datasets.}
% %   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|}
% \hline   Dataset  & \# train & \# validation & \# test \\
%     \hline
%     CodeReviewer~\cite{li2022automating} & 150,405 & 13,102 & 13,103 \\
%     Tufano~\cite{tufano2022using} & 134,238 & 16,779 & 16,779 \\
%     Android~\cite{pornprasit2023d} & 14,690 & 1,836 & 1,835 \\
%     Google~\cite{pornprasit2023d} & 9,899 & 1,237 & 1,235 \\
%     Ovirt~\cite{pornprasit2023d}  & 21,509 & 2,686 & 2,688 \\
%     % Gerrit & 3,144 & 544 & 370 \\
%     \hline
%     \end{tabular}%
%     % }
%   \label{tab:data-stat}%
% \end{table}%

% \subsection{Dataset}

%     % - collect from where?
%     % - what are input, output (or component)?
%     % - for what task?

%     In this study, we use the following datasets which are summarized in Table~\ref{tab:data-stat}: \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and \CodeReviewerData~\cite{li2022automating}.
%     We describe the details of these datasets below.

%     \begin{itemize}

%         \item \textbf{\tufanoData}: Tufano~\ea~\cite{tufano2022using} collected this dataset from GitHub projects containing at least 50 pull requests, and 6,388 Gerrit projects.
%         Each record in the dataset contains a triplet of code submitted for review (method-level), a reviewer's comment, and code after being revised (method-level) based on a reviewer's comment.
%         The dataset is used to train models for \CodeCommentToCode~and \CodeToCode~tasks.
    
%         \item \textbf{\CodeReviewerData}: Li~\ea~\cite{li2022automating} collected this dataset from GitHub projects that contain at least 1,500 pull requests.
%         % The dataset contains the following information.
%         % The dataset is divided into two categories.
%         % The data in the first category are the pairs of code differences and labels indicating whether the code differences need reviewers' comment.
%         % These data pairs are used to train models for the review necessity prediction task.
%         % The data in the second category contains triplets of the current version of code, the reviewers' comment, and the revised version of code.
%         The dataset contains triplets of the current version of code, the reviewers' comment, and the revised version of code.
%         These data triplets are used to train models for \CodeDiffToComment~task.
    
%         \item \textbf{\DACTData}: Pornprasit~\ea~\cite{pornprasit2023d} collected this dataset from the three software projects hosted on Gerrit (i.e., Android, Google and Ovirt).
%         Each record in the dataset contains a triplet of codebase, code of the first version of a patch, and code of the approved version of a patch.
%         The dataset is used to train models for code $\longrightarrow$ code task.

%     \end{itemize}
    

% % \subsection{Data Filtering}
% % % To do data filtering for Openstack and Qt datasets, we first sort the datasets by commit date since code changes are submitted in temporal order.
% % To do data filtering, we first sort the datasets by commit date since code changes are submitted in the temporal order.
% % Then, we follow data filtering steps in~\cite{pornprasit2023d} to ensure the validity of datasets.

% % \subsection{Implementation Detail}

% % % - for LLMs
% % %     - use gpt-3.5 and gpt-4 from API provided by OpenAI
% % %     - use LLaMa-code model provided by HuggingFace
% % % - for state-of-the-art
% % %     - use implementations provided in replication packages~\cite{paper here}
% % % - for pre-trained models
% % %     - use the following models: CodeBERT, GraphCodeBERT, ... //also cite them

% %     We describe the implementation details of large language models and the existing code refinement approaches~\cite{li2022automating, pornprasit2023d, tufano2022using} below. 
% %     % and pre-trained code models~\cite{codebert, guo2020graphcodebert,ahmad2021plbart,wang2021codet5,guo2022unixcoder} below.

% %     % First, for large language models, we use GPT-3.5 from the API provided by OpenAI\footnote{https://openai.com/}, and use Code LLaMa model~\cite{roziere2023code} provided by HuggingFace.
% %     % First, for large language models, we use a commercial LLM (i.e., GPT-3.5)  from the API provided by OpenAI\footnote{https://openai.com/}, and use an open-source LLM (i.e., Code LLaMal~\cite{roziere2023code}) provided by HuggingFace.
% %     First, for large language models, we use \chatGPT~from the API provided by OpenAI\footnote{https://openai.com/}. 
% %     % and use Google Bard from the implementation in GitHub\footnote{https://github.com/dsdanielpark/Bard-API}.
% %     We use default hyper-parameter settings and use the maximum length of the generated result of 512.
    
% %     Second, we use the implementations of the existing code refinement approaches that are provided in the replication packages~\cite{li2022automating, pornprasit2023d, tufano2022using}.
% %     % Lastly, we fine-tune the following pre-trained code models: CodeBERT~\cite{codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, PLBART~\cite{ahmad2021plbart}, CodeT5~\cite{wang2021codet5} and UniXCoder~\cite{guo2022unixcoder}.
% %     To fine-tune the existing code refinement approaches, we use a training batch size of 6 and a learning rate of 5e-5.
% %     % We select the final models that achieve the lowest loss value or the highest BLEU score calculated from the validation set to generate results from the testing set.
% %     We also use an early-stopping strategy~\cite{prechelt2002early} by using a patience value of 7 and delta value of 0.001, to prevent the models from being overfitted to the training sets.


% \subsection{Experimental Environment}

%     We conduct the experiment in the server equipped with the following hardware: an AMD Ryzen 9 5950X @3.4 GHz 16-Core CPU, an SSD of 1 Terabyte, a RAM of 64 Gigabyte, and an NVIDIA GeForce RTX 3090 GPU with 24 GB memory.




==> section-exp-only/Introduction-old-2.tex <==
\section{Introduction}

Modern code review is the practice where reviewers (i.e., developers other than the patch author) review a \emph{patch (i.e., a set of code changes)} that is created by a developer (i.e., a patch author) to ensure that the patch has sufficient quality.
Generally, the main goals of code review are finding defects~\cite{bacchelli2013expectations, macleod2017code} and improving the quality of code (e.g., readability)~\cite{han2022code, alomar2022code, beller2014modern,ThongtanunamMSR2015, Sadowski2018, morales2015code}.
Although code review can ensure high software quality, such practice also introduces challenges to developers.
In particular, code review can be time-consuming~\cite{bosu2013impact}.
For example, developers in Microsoft Bing have to undergo around 3,000 reviews per month~\cite{rigby2013convergent}.

To address the above challenge, prior work~\cite{tufano2019learning, AutoTransform, tufano2021towards, pornprasit2023d, li2022automating, tufano2022using} proposed neural machine translation (NMT)-based code review automation approaches to facilitate developers revising their patches.
For example, Pornprasit~\ea~\cite{pornprasit2023d} proposed \DACTmodel~to generate the patch that reviewers are likely to approve from the first version of a patch.
Similarly, Li~\ea~\cite{li2022automating} and Tufano~\ea~\cite{tufano2022using} built pre-trained models for various code review automation tasks (e.g., generating reviewers' comments from a given code difference, generating improved code from the code submitted for review).

% - ก่อนหน้านี้มีคนทำ LLM มากมายหลายอย่างเลย
%     - อย่างเช่น PaLM จาก Google, GPT-3.5 turbo (ChatGPT) จาก Microsoft, Code LLaMa จาก Meta

Recently, several groups of researchers proposed large language models (LLMs) that are based on the transformer~\cite{Vaswani2017} architecture.
For example, the researchers from OpenAI team are the first to present a commercial LLM namely  GPT-3.5, a large generative model pre-trained on natural language and source code.
Similarly, Rozière~\ea~\cite{roziere2023codeLLaMa} from Meta introduced Code LLaMa, the open-source LLM that is based on LLaMa-2 model~\cite{touvron2023llama2} further trained with source code.


% - มีงานก่อนหน้าหลายอย่างที่แสดงให้เห็นว่า LLM มันเอามาใช้ใน SE task ได้หลายอย่าง และมันก็ outperform งานก่อนหน้าด้วยนะ
%     - อย่างเช่น automated program repair, code summarization, comment generation
%     - ยกตัวอย่างงานของแต่ละกลุ่มมาอย่างละ 1-2 อันไรงี้ขำๆ

Prior studies show that LLM could be used for various software engineering tasks (e.g., automated program repair~\cite{wei2023copiloting, jin2023inferfix, xia2023conversational} and code summarization~\cite{ahmed2022few, gao2023makes, sun2023automatic}) and even outperform the existing deep learning-based approaches.
For instance, Xia~\ea~\cite{xia2023conversational} proposed a conversational-based approach for automated program repair.
Ahmed~\ea~\cite{ahmed2022few} proposed using few-shot learning for code summarization.


% - อย่างไรก็ตาม ยังไม่มีงานไหนที่ศึกษาการใช้ LLM ในหลายแง่มุม (นั่นคือการใช้ few-shot learning, การใช้ persona และการ fine-tune LLM) สำหรับทำ code review automation
%     - ดังนั้นจนถึงตอนนี้ก็เลยยังไม่รู้ว่าควรจะเอา LLM มาใช้ยังไงเพื่อให้มันสร้าง improved code ได้ถูกต้องมากที่สุด
%     - เราเลยมาทำ study นี้ขึ้นมาเพื่อปิด knowledge gap ตรงนี้
%     - ซึ่งการทำแบบนี้จะช่วยให้แนวทางการใช้ LLM เพื่อทำ code review automation สำหรับ practitioner

However, to the best of our knowledge, none of the existing work conducts a study of using LLMs in different aspects (i.e., using few-shot learning, using persona prompts, and model fine-tuning) for code review automation tasks.
% Thus, little is known about how LLMs should be used so that they can correctly generate the improved code as much as possible.
Thus, little is known about how LLMs should be used for code review automation tasks.
Therefore, we conduct this study to fill this knowledge gap.
By doing so, practitioners would have guidelines for using LLMs for code review automation.


% - ในงานนี้เราทำ empirical study เพื่อศึกษาดูว่าจะเอา LLM มาช้ยังไงเพื่อให้มันสร้าง improved code ได้ถูกต้องมากที่สุด
%     - เราใช้ 0-shot และ few-shot learning 
%     - เราใช้ persona ใน prompt
%     - เราลองเอา ChatGPT มา fine-tune ดู
%     - เราทำการทดลองเพื่อตอบ RQ ต่อไปนี้
%         - RQ1 + results
%         - RQ2 + results
%         - RQ3 + results
%         - RQ4 + results


In this work, we conduct an empirical study to investigate how LLMs should be used for code review automation tasks.
In particular, we conduct the study with GPT-3.5 by using 0-shot and few-shot learning~\cite{brown2020language} approaches.
We also investigate the impact of using persona in a prompt and fine-tuning GPT-3.5.
Through a case study of the three code review automation datasets (i.e., \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and Code\-Reviewer\textsubscript{data}~\cite{li2022automating}), we answer the following research questions:

\textbf{(RQ1) \rqone}

\smallsection{Result}
Including examples in input prompts could increase Exact Match and CodeBLEU by at least 46.38\% and 3.97\%, respectively.

\textbf{(RQ2) \rqtwo}

\smallsection{Result}
In overall, GPT-3.5 that does not use persona achieves higher Exact Match and CodeBLEU than GPT-3.5 that uses persona.

\textbf{(RQ3) \rqthree}

\smallsection{Result}
In overall, fine-tuned GPT-3.5 achieves higher Exact Match and CodeBLEU than GPT-3.5 that is not fine-tuned.

\textbf{(RQ4) \rqfour}

\smallsection{Result}
The existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d} always outperform GPT-3.5 that uses 0-shot learning while fine-tuned GPT-3.5 outperforms the existing code review automation approaches in \tufanoData~and \DACTData.

\textbf{Implications.}
Our results imply that (1) practitioners should use few-shot learning rather than 0-shot learning, (2) practitioners could construct prompts without using persona in the prompts, and (3) practitioners could fine-tune GPT-3.5 by using a small training dataset.

\textbf{Contributions.}
In summary, the main contributions of our work are as follows

\begin{itemize}
    \item We are the first to conduct an empirical study of using GPT-3.5 in different aspects (i.e., using few-shot learning, using persona prompts, and model fine-tuning) for code review automation tasks.
    \item We discuss the implication of our findings for practitioners for adapting GPT-3.5 for code review automation.
\end{itemize}

\textbf{Paper Organization.}
Section~\ref{sec:background} describes the background with respect to the literature.
% Section~\ref{sec:task-prompt} describes the details of code review automation tasks and prompt design.
Section~\ref{sec:study-design} describes the study design of our study.
% Section~\ref{sec:exp_design} describes the experimental design.
Section~\ref{sec:results} presents the experiment results.
Section~\ref{sec:discussion} discusses our experiment results.
Section~\ref{sec:threat} describes possible threats to the validity.
% Section~\ref{sec:RelatedWork} describes the literature related to our work.
Section~\ref{sec:conclusion} draws the conclusions of our work.


==> section-exp-only/Introduction-old-3.tex <==
\section{Introduction}

\kla{need to update, as the last thing?}


%%LLM คืออะไร + มีคนทำออกมามากมายหลายเจ้า
Recently, large language models (LLMs)--large deep learning models that are based on the transformer architecture~\cite{Vaswani2017} and pre-trained on massive datasets--were proposed~\cite{roziere2023codeLLaMa, touvron2023llama2, achiam2023gpt, workshop2022bloom}.
For example, the researchers from OpenAI were the first to present a commercial LLM namely  GPT-3.5, a large generative model pre-trained on natural language and source code.
Similarly, Rozière~\ea~\cite{roziere2023codeLLaMa} from Meta introduced Code LLaMa, the open-source LLM that is based on LLaMa-2 model~\cite{touvron2023llama2} further trained with source code.

%%งานก่อนหน้าใน ML field ได้มีการศึกษาเรื่องการเอา LLM มาใช้งานในหลายแง่มุมด้วยกัน ซึ่งโดยหลักๆก็เกี่ยวกับ prompt design, few-shot learning และ model-finetuning
% Prior studies conducted experiments focusing on different aspects (i.e., prompt engineering~\cite{lu2023bounding, arora2022ask, sivarajkumar2023empirical}, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} and model fine-tuning~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating}) of leveraging LLMs for downstream tasks.
Prior studies conducted experiments focusing on different approaches to leverage LLMs (e.g., prompt engineering~\cite{lu2023bounding, arora2022ask, sivarajkumar2023empirical}, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} and model fine-tuning~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating}) for downstream tasks.
For instance, Arora~\ea~\cite{arora2022ask} proposed the prompt design based on the question-answering prompts, which helps an open-source LLM to outperform GPT-3 that few-shot learning is performed.
% and showed that their proposed prompt design helps open.
Another example is Bro\-wn \textit{et al.}~\cite{brown2020language} that conducted an empirical study of few-shot learning on LLMs for a variety of natural language processing (NLP) tasks.
Lastly, Chen~\ea~\cite{chen2021evaluating} conducted an experimental study of an LLM (i.e., GPT-3) fine-tuned on source code.


% Another example is the study of ... conducted studies for few-shot learning.
% Lastly, 

% conducted studies for model fine-tuning.

%%% old version

%% และที่งานใน ML field มันเอา LLM มาใช้แล้วได้ผลดี พวกคนใน SE field ก็เลยเอา LLM มาใช้กันหลายงานเลย
% By seeing the promising capabilities of LLMs in NLP tasks, LLMs-based approaches for software engineering tasks~\cite{deligiannis2023fixing, eliseeva2023commit, yu2023wavecoder, chakraborty2023ranking, chen2024large, misu2024towards, jiang2023llmparser} were proposed.
% For example, Deligiannis~\ea~\cite{deligiannis2023fixing} proposed \chatGPT-based approach for fixing compilation errors in Rust.
% % Deligiannis~\ea~\cite{eliseeva2023commit} presented \chatGPT-based approach for commit message generation.
% Prior work~\cite{xia2023automated, chen2023effectiveness, schafer2023empirical, gao2023constructing, yuan2023evaluating} also conducted empirical studies of LLMs on different software engineering tasks.
% For instance, Sch{\"a}fer~\ea~\cite{schafer2023empirical} investigated the performance of GPT-3.5 for automated unit test generation in Javascript.
% % Chen~\ea~\cite{chen2023effectiveness} conducted an empirical study of LLMs in domain-specific code generation.
% However, the existing literature still lacks the study of different approaches to leveraging GPT-3.5 (e.g., prompt engineering~\cite{lu2023bounding, arora2022ask, sivarajkumar2023empirical}, few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} and model fine-tuning~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating}) for code review automation (i.e., automatically generating improved code from submitted code)~\cite{tufano2022using, li2022automating, pornprasit2023d}.

%%% end old version

\revised{R1-7}
{
By seeing the promising capabilities of LLMs in NLP tasks, recent research focused on proposing LLM-based approaches for software engineering~\cite{chen2024large, misu2024towards, jiang2023llmparser, zhang2024automated, llamareviewer}, or empirical studies of LLM for software engineering~\cite{xia2023automated, gao2023constructing, zhang2024automated}.
However, recent work did not show whether few-shot learning outperforms zero-shot learning~\cite{xia2023automated, gao2023constructing}, or showed that one-shot learning does not always outperform zero-shot learning~\cite{zhang2024automated}.
In addition, the current literature still lacks the study of the impact of persona patterns in the proposed approaches~\cite{chen2024large, misu2024towards, jiang2023llmparser, zhang2024automated}.
Thus, it is still unclear whether persona patterns should be included in input prompts.
Lastly, Lu~\ea~\cite{llamareviewer} showed that the fine-tuned LLaMa~\cite{touvron2023llama} model still does not outperform the existing code review automation approaches~\cite{li2022automating, tufano2022using}.
}


% In this work, we conduct an experimental study to investigate the impact of few-shot learning, prompt design, and model fine-tuning on GPT-3.5 for the code review automation task.
\revised{R1-1}{
In this work, we conduct an experimental study to investigate the performance of GPT-3.5 on code review automation tasks under different settings (i.e., performing few-shot learning, including persona in input prompts, and fine-tuning GPT-3.5).
}
In particular, to perform few-shot learning, we obtain examples from BM25~\cite{robertson2009probabilistic}, and investigate the impact of the persona prompt pattern~\cite{white2023prompt}.
% To do few-shot learning, we select example pairs of input and output from the training set by using BM25~\cite{robertson2009probabilistic}.
% For the impact of prompt design, we investigate the impact of the persona prompt pattern~\cite{white2023prompt}.
% To fine-tune GPT-3.5, we randomly select a subset of training samples from training sets, then fine-tune GPT-3.5 by using the API provided by OpenAI\footnote{https://platform.openai.com/docs/guides/fine-tuning/create-a-fine-tuned-model}.
We also compare the performance of GPT-3.5 with the existing deep learning-based code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d} with respect to the following evaluation measures: Exact Match (EM)~\cite{pornprasit2023d, tufano2019learning} and CodeBLEU~\cite{ren2020codebleu}.
% In particular, we conduct the study with GPT-3.5 by using zero-shot and few-shot learning~\cite{brown2020language} approaches.
% We also investigate the impact of using persona in a prompt and fine-tuning GPT-3.5.
Through the experimental study of the three code review automation datasets (i.e., \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and Code\-Reviewer\textsubscript{data}~\cite{li2022automating}), we answer the following four research questions:

\textbf{(RQ1) \rqone}

\smallsection{Result}
When few-shot learning is performed, GPT-3.5 achieves at least 46.38\% higher EM and at least 3.97\% higher CodeBLEU than GPT-3.5 that zero-shot learning is performed.
% GPT-3.5 can achieve higher Exact Match and CodeBLEU by providing example input/output pairs in input prompts to help GPT-3.5 adapt to the code refinement task that it never learned during model pre-training phase.
% Few-shot learning could increase Exact Match and CodeBLEU by at least 46.38\% and 3.97\%, respectively.
The increase in Exact Match and CodeBLEU is due to providing example input/output pairs in input prompts to GPT-3.5 to learn how to generate improved code.


\textbf{(RQ2) \rqtwo}

\smallsection{Result}
% In overall, GPT-3.5 that does not use persona achieves higher Exact Match and CodeBLEU than GPT-3.5 that uses persona.
% GPT-3.5 that persona is not included in input prompts achieves at least 1.03\% and 1.21\% higher EM and CodeBLEU than GPT-3.5 that persona is included in input prompts, respectively.
When persona is included in input prompts to generate improved code, GPT-3.5 achieves at least 1.02\% lower EM and 0.15\% lower CodeBLEU than when persona is not included in the input prompts.
The decrease in Exact Match and CodeBLEU is due to persona decreasing the likelihood of GPT-3.5 generating more correct and similar improved code to actual improved code.


\textbf{(RQ3) \rqthree}

\smallsection{Result}
% In overall, fine-tuned GPT-3.5 achieves higher Exact Match and CodeBLEU than GPT-3.5 that is not fine-tuned.
Fine-tuned GPT-3.5 achieves at least 9.74\% higher EM and 0.12\% higher CodeBLEU than GPT-3.5 that zero-shot and few-shot learning is performed.
The increase in Exact Match and CodeBLEU is due to GPT-3.5 being fine-tuned with thousands of samples in a training dataset to learn how to generate improved code.

\textbf{(RQ4) \rqfour}

\smallsection{Result}
% In overall, fine-tuned GPT-3.5 outperforms the existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d} in terms of Exact Match.
The existing code review automation approaches achieve at least 5.47\% higher EM than GPT-3.5 that zero-shot learning is performed while fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.

%% อื่นๆที่เหลือก็เอามาจากอันเก่าเนี่ยแหละ


% \textbf{Implications.}
% Our results imply that practitioners should (1) perform few-shot learning rather than zero-shot learning, (2) construct prompts without including persona in the prompts, and (3) fine-tune GPT-3.5 by using a small training set.

\textbf{Recommendation.}
Based on our experiment results, we recommend that when using GPT-3.5 for code review automation
(1) few-shot learning should be performed rather than zero-shot learning,
(2) persona should not be included when constructing prompts, 
and (3) GPT-3.5 should be fine-tuned by using a small training dataset.



\textbf{Contributions.}
In summary, the main contributions of our work are as follows:

\begin{itemize}
    % \item We are the first to conduct experiments to investigate the impact of few-shot learning, prompt design, and model fine-tuning on GPT-3.5 for the code review automation tasks.
    \item We are the first to conduct an experimental study to investigate the performance of GPT-3.5 on code review automation tasks under different settings (i.e., performing few-shot learning, including persona in input prompts, and fine-tuning GPT-3.5)
    \item We provide recommendations for adapting GPT-3.5 for code review automation.
\end{itemize}


\revised{R1-7}
{
\textbf{Novelty.}
Our experimental study presents the following findings:

\begin{itemize}
    \item Different from prior work~\cite{xia2023automated, gao2023constructing, zhang2024automated}, few-shot learning outperforms zero-shot learning on code review automation tasks. 
    % when few-shot learning is performed, GPT-3.5 achieves higher performance than GPT-3.5 that zero-shot learning is performed.
    % unlike prior work that did not show superior performance of few-shot learnring over zero-shot learning~\cite{xia2023automated, gao2023constructing}, or showed that one-shot learning does not always outperform zero-shot learning~\cite{yuan2023evaluating}.
    \item Including persona has a negative impact on the performance of GPT-3.5 on code review automation tasks, which is not shown in previous studies~\cite{chen2024large, misu2024towards, jiang2023llmparser, zhang2024automated}.
    % , unlike previous work ~\cite{chen2024large, misu2024towards, jiang2023llmparser, zhang2024automated} that did not show whether including persona in input prompts could increase the performance of their approaches.
    \item Model fine-tuning could help GPT-3.5 outperforms the existing code review automation approaches~\cite{li2022automating, tufano2022using, pornprasit2023d}, which contradicts to Lu's~\ea~findings~\cite{llamareviewer}.
    % which contradicts to  Lu~\ea's findings that fine-tuned LLaMa~\cite{touvron2023llama} does not outperform the existing code review automation approaches~\cite{llamareviewer}. 
\end{itemize}
}

\textbf{Open Science.}
% To facilitate future work, we make the script, the dataset, and the output generated by GPT-3.5 available online\footnote{https://shorturl.at/fpR28}.
Our supplementary material will be made available upon acceptance.

\textbf{Paper Organization.}
Section~\ref{sec:background} describes the background with respect to the literature.
% Section~\ref{sec:task-prompt} describes the details of code review automation tasks and prompt design.
Section~\ref{sec:study-design} describes the study design of our study.
Section~\ref{sec:exp_design} describes the experiment setup.
Section~\ref{sec:results} presents the experiment results.
Section~\ref{sec:discussion} discusses our experiment results.
Section~\ref{sec:threat} describes possible threats to the validity.
% Section~\ref{sec:RelatedWork} describes the literature related to our work.
Section~\ref{sec:conclusion} draws the conclusions of our work.



==> section-exp-only/Introduction-old.tex <==
% \begin{table*}[ht]
%     \centering
%     \caption{The summary of the recent literature related to code review automation. (the Year column shows the year that a study was published)}
%     \label{tab:recent-work}
%     \begin{tabular}{|c|c|c|c|c|c|} 
    
%         \hline 
%          Study  & Year & Approach  &  Baseline   &Input/Output Representation&  Has ChatGPT?\\ \hline 
%          Guo~\ea~\cite{guo2023exploring} & 2023 & ChatGPT & CodeReviewer~\cite{li2022automating}  & code at diff hunk level& Yes \\ 
%          \hline
%          Pornprasit~\ea~\cite{pornprasit2023d} & 2023 & D-ACT & Tufano~\ea~\cite{tufano2022using}  &code at method level& No \\ 
%          \hline
%          Li~\ea~\cite{li2022automating}  & 2022 & CodeReviewer & Transformer~\cite{Vaswani2017}, T5~\cite{raffel2020exploring}, CodeT5~\cite{wang2021codet5}  &code at diff hunk level& No \\ 
%          \hline
%          Tufano~\ea~\cite{tufano2022using} & 2022 & Pre-trained T5 & None  &code at method level& No \\ 
%          \hline
%          % Tufano~\ea~\cite{tufano2021towards} & Transformer + code abstraction & None & Newly collected Java code from GitHub & No \\ 
%          % \hline 
%          % Thongtanunam~\ea~\cite{AutoTransform} & Transformer + BPE & Tufano~\ea~\cite{tufano2019learning} & Tufano~\ea~\cite{tufano2019learning} & No \\ 
%          % \hline 
%          % Tufano~\ea~\cite{tufano2019learning} & RNN & None & Newly collected code in Java (Android, Google, Ovirt) & No \\ 
%          % \hline 

%     \end{tabular}
    
% \end{table*}

\section{Introduction}\label{sec:intro}

Modern code review is the practice where reviewers (i.e., developers other than the patch author) review a \emph{patch (i.e., a set of code changes)} that is created by a developer (i.e., a patch author) to ensure that the patch has sufficient quality.
Generally, the main goals of code review are finding defects~\cite{bacchelli2013expectations, macleod2017code} and improving the quality of code (e.g., readability)~\cite{han2022code, alomar2022code, beller2014modern,ThongtanunamMSR2015, Sadowski2018, morales2015code}.
Although code review can ensure high software quality, such practice also introduces challenges to developers.
In particular, code review can be time-consuming~\cite{bosu2013impact}.
For example, developers in Microsoft Bing have to undergo around 3,000 reviews per month~\cite{rigby2013convergent}.

To address the above challenge, prior work~\cite{tufano2019learning, AutoTransform, tufano2021towards, pornprasit2023d, li2022automating, tufano2022using} proposed neural machine translation (NMT)-based code review automation approaches to facilitate developers revising their patches.
For example, Pornprasit~\ea~\cite{pornprasit2023d} proposed \DACTmodel~to generate the patch that reviewers are likely to approve from the first version of a patch.
Similarly, Li~\ea~\cite{li2022automating} and Tufano~\ea~\cite{tufano2022using} built pre-trained models for various code review automation tasks (e.g., generating reviewers' comments from a given code difference, generating improved code from the code submitted for review).

Recently, Guo~\ea~\cite{guo2023exploring} observed that code review automation aligns well with the strength of a large language model-based AI assistant (i.e., \chatGPT).
Thus, they conducted experiments with \chatGPT~to find the best prompt and temperature value for code review automation tasks.
While the study of Guo~\ea~\cite{guo2023exploring} shows the potential of using ChatGPT for code review automation, we find the following two limitations in their work.
% They found that \chatGPT~can outperform the existing code review automation approach (i.e., CodeReviewer~\cite{li2022automating}).
% While their study shows the potential of using \chatGPT~to automate code review, 
% However, their study is only limited to 0-shot learning (i.e., providing a prompt with input to a model).
% Indeed, apart from 0-shot learning, few-shot learning~\cite{brown2020language} is another approach to leverage \chatGPT~for downstream tasks.
% Recent work showed that few-shot learning can be applied for various software engineering tasks~\cite{geng2024large, ahmed2022few, deligiannis2023fixing, xia2023automated}.
% However, few-shot learning is not well-studied in the field of code review automation.
% Thus, little is known about the performance of few-shot learning for code review automation. 
% % Therefore, we conduct this study to fill this gap in the literature.
% Therefore, we conduct this study to pave the way forward using few-shot learning for code review automation.
% Therefore, we conduct experiments to understand the capabilities of few-shot learning for code review automation.

First, the study of Guo~\ea~\cite{guo2023exploring} overlooked the existing code review automation benchmarks. In particular, Guo~\ea~\cite{guo2023exploring} conducted their study with their newly collected dataset and showed that ChatGPT outperforms CodeReviewer. However, their study lacks an empirical evaluation of the existing code review automation approaches in the other benchmarks. Thus, it is still unclear about how ChatGPT performs when compared to the existing code review automation approaches in the other benchmarks. Thus, we conduct a replication study to fill this knowledge gap, which could potentially be useful for practitioners to consider using ChatGPT for code review automation.

Second, the study of Guo~\ea~\cite{guo2023exploring} does not consider few-shot learning. In particular, Guo ~\ea~\cite{guo2023exploring} designed their prompt for 0-shot learning (i.e., the prompt only contains an instruction and an input sample). However, there is another learning technique for LLMs called few-shot learning, which is providing some input/output examples and the actual input sample to LLM. Indeed, prior work showed that few-shot learning is effective for a variety of software engineering tasks~\cite{geng2024large, ahmed2022few, deligiannis2023fixing, xia2023automated}. However, using few-shot learning for code review automation is still largely unexplored. Thus, we conduct a study to investigate the capability of few-shot learning for code review automation. We expect that the findings from the study could help researchers see the potential of using few-shot learning for code review automation.



In this paper, we investigate the capabilities of few-shot learning for code review automation.
In our experiment, we use \chatGPT~to do 0-shot learning and few-shot learning.
To do 0-shot learning, we use the best prompt created by Guo~\ea~\cite{guo2023exploring} (we will call 0-shot learning with this prompt as \emph{\ChatGPTGuo} henceforth).
For few-shot learning (we will call this as \emph{\ChatGPTFewShot}~henceforth), we use BM25~\cite{robertson2009probabilistic} to select examples from the training set for test samples, which is more effective than random sampling~\cite{gao2023constructing, yuan2023evaluating}.
Through a case study of the existing code review automation benchmarks (i.e., \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and \CodeReviewerData~\cite{li2022automating}), we address the following research questions:


\textbf{(RQ1) \rqI}

\textbf{Result.}
\willdo

% \textbf{Result.}
% When using few-shot learning, ChatGPT\textsubscript{few-shot} achieves 1.56\% and 26.49\% lower EM and CodeBLEU than \ChatGPTGuo, respectively on \CodeReviewerData~dataset.

% Guo~\ea's approach~\cite{guo2023exploring} achieves 1.67\% and 36.04\% higher EM and CodeBLEU than \ChatGPTFewShot, respectively on \CodeReviewerData~dataset.


\textbf{(RQ2) \rqII}

\textbf{Result.}
\willdo

% \textbf{Result.}
% In terms of EM, \ChatGPTFewShot~achieves at least 30.74\% higher than \ChatGPTGuo.
% In terms of CodeBLEU, \ChatGPTFewShot~achieves at least 3.2\% higher than \ChatGPTGuo.
% \ChatGPTFewShot~achieves at least 30.74\% and 3.2\% higher EM and CodeBLEU than Guo~\ea's approach~\cite{guo2023exploring}, respectively on \tufanoData~and \DACTData~dataset.

% \textbf{(RQ3) \rqIII}

% \textbf{Result.}
% In terms of EM, \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d} achieve at least 6.72\% higher than \ChatGPTFewShot~while \ChatGPTFewShot~achieves at least 13.81\% higher than \Tufanomodel~\cite{tufano2022using}.
% In terms of CodeBLEU, \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d} achieve at least 92.31\% higher
% \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d} achieves 6.72\% and at least 92.31\% higher EM than \ChatGPTFewShot, respectively while \ChatGPTFewShot~achieves at least 13.81\% higher EM than \Tufanomodel~\cite{tufano2022using}.
% In terms of CodeBLEU, \Tufanomodel~(in case input does not contain a reviewer's comment), \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d} achieve at least 8.04\% higher \ChatGPTFewShot~while \ChatGPTFewShot achieves 1.13\% higher CodeBLEU than \Tufanomodel~(in case input contains a reviewer's comment).
% On the other hand, \Tufanomodel~(\CodeToCode~task), \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d} achieves at least 8.04\% higher CodeBLEU than \ChatGPTFewShot while \ChatGPTFewShot achieves 1.13\% higher CodeBLEU than \Tufanomodel~(\CodeCommentToCode~task).

% The experiment results suggest that \ChatGPTFewShot~outperforms Guo~\ea's approach~\cite{guo2023exploring} but does not always outperform the existing code review automation approaches.
% Thus, future work should explore how to do few-shot learning that can outperform all existing code review automation approaches.


\textbf{Paper Organization.}
Section~\ref{sec:background} describes the background with respect to the literature.
% Section~\ref{sec:task-prompt} describes the details of code review automation tasks and prompt design.
Section~\ref{sec:study-design} describes the study design of the survey study.
% Section~\ref{sec:exp_design} describes the experimental design.
Section~\ref{sec:results} presents the experiment results.
Section~\ref{sec:discussion} discusses our experiment results.
Section~\ref{sec:threat} describes possible threats to the validity.
Section~\ref{sec:RelatedWork} describes the literature related to our work.
Section~\ref{sec:conclusion} draws the conclusions of our work.



==> section-exp-only/Motivation.tex <==
\section{Motivation}

\begin{table*}[ht]
    \centering
    \caption{The summary of the recent literature related to code review automation.}
    \label{tab:recent-work}
    \begin{tabular}{|c|c|c|c|c|} 
    
        \hline 
         Study  & Year published& Approach  &  Baseline(s)   &  Has ChatGPT?\\ \hline 
         Guo~\ea~\cite{guo2023exploring} & 2023 & ChatGPT & CodeReviewer~\cite{li2022automating}  & Yes \\ 
         \hline
         Pornprasit~\ea~\cite{pornprasit2023d} & 2023 & D-ACT & Tufano~\ea~\cite{tufano2022using}  & No \\ 
         \hline
         Li~\ea~\cite{li2022automating}  & 2022 & CodeReviewer & \thead{Transformer~\cite{Vaswani2017}, \\ T5~\cite{raffel2020exploring}, CodeT5~\cite{wang2021codet5}}  & No \\ 
         \hline
         Tufano~\ea~\cite{tufano2022using} & 2022 & Pre-trained T5 & Tufano~\ea~\cite{tufano2021towards}  & No \\ 
         \hline
         % Tufano~\ea~\cite{tufano2021towards} & Transformer + code abstraction & None & Newly collected Java code from GitHub & No \\ 
         % \hline 
         % Thongtanunam~\ea~\cite{AutoTransform} & Transformer + BPE & Tufano~\ea~\cite{tufano2019learning} & Tufano~\ea~\cite{tufano2019learning} & No \\ 
         % \hline 
         % Tufano~\ea~\cite{tufano2019learning} & RNN & None & Newly collected code in Java (Android, Google, Ovirt) & No \\ 
         % \hline 

    \end{tabular}
    
\end{table*}


Recently, researchers conducted studies relating to code review automation, which can be summarized in Table~\ref{tab:recent-work}.
The table shows that while prior work~\cite{pornprasit2023d, li2022automating, tufano2022using} compared the proposed approaches with the existing code review automation approaches or pre-trained models, only the study of Guo~\ea~\cite{guo2023exploring} compared \chatGPT~with the existing code review automation approach (i.e., CodeReviewer~\cite{li2022automating}).
% From the table, we can see that 
% The table shows that each study has its own dataset with input/output representations specific to the approach in that study.
% The table shows that each study use the dataset with input/output representations specific to the approach in that study.
% different datasets have different input/output representations for their approaches.
% From the table, we can see that the authors collected the datasets that are specific to their studies.
% For example, Tufano~\ea~\cite{tufano2022using} collected reviewers' comments, and pairs of code submitted for review and code after being revised at the method level, to fine-tune their pre-trained T5 model.
% For example, Tufano~\ea~\cite{tufano2022using} used the dataset consisting of reviewers' comments, and pairs of code submitted for review and code after being revised at the method level, to fine-tune their pre-trained T5 model.
% In contrast, Li~\ea~\cite{li2022automating} used the dataset consisting of reviewers' comments, and pairs of code submitted for review and code after being revised at diff hunk level, to fine-tune their CodeReviewer model.
% However, we can see that 
% The table also shows that only Guo~\ea~\cite{guo2023exploring} conducted their study with \chatGPT~by comparing \chatGPT~with the existing code review automation approach (i.e., CodeReviewer~\cite{li2022automating}) on the dataset collected by Li~\ea~\cite{li2022automating}.
% The table shows that only Guo~\ea~\cite{guo2023exploring} conducted their study with \chatGPT~on the dataset collected by Li~\ea~\cite{li2022automating}.
% While the aforementioned studies~\cite{tufano2022using, li2022automating, guo2023exploring} use datasets with different input/output representations,
% On the other hand, the aforementioned studies~\cite{tufano2022using, li2022automating, guo2023exploring}
% Even though these studies are conducted with datasets having different input/output representations, these studies share a similarity in that they only evaluate their proposed approaches and baselines with the patches obtained from the historical review records.
However, these studies share a similarity in that they only evaluate their proposed approaches and baselines with the patches obtained from the historical review records.
Based on the current literature explained above, we find that prior work~\cite{tufano2022using, li2022automating, guo2023exploring, pornprasit2023d} has the following two limitations relating how evaluation is conducted in the studies.

% - finding ที่บอกว่า ChatGPT มัน generalize ดีกว่า existing approach (CodeReviewer) นี่มันอาจจะเป็นเรื่องที่ optimistic เกินไปหน่อย
%   - เพราะว่าทำการทดลองกับ dataset ที่เก็บมาเองแค่อันเดียว
%   - แต่เอาจริงก็มี dataset อื่นอีกที่ยังไม่ได้ explore
%   - ดังนั้นก็เลยยังไม่รู้ว่าจริงๆแล้ว ChatGPT มันจะ generalize กับ dataset อื่นเมื่อเทียบกับ existing approach อันอื่นมั้ย
%   - ดังนั้นถ้าได้รู้เรื่องพวกนี้แล้วก็น่าจะเป็นแนวทางให้ developer ตัดสินใจได้ว่าจะใช้ ChatGPT หรือ existing approach ดีหว่าไรงี้??

\textbf{The performance of \chatGPT~in the study of Guo~\ea~\cite{guo2023exploring} may be overly optimistic.}
Guo~\ea~\cite{guo2023exploring} found that \chatGPT~has better generalization capabilities than \CodeReviewerModel~\cite{li2022automating}.
However, their findings may be overly optimistic for the following two reasons.
% However, the evaluation of Guo~\ea~\cite{guo2023exploring} overlooks the other benchmarks that are used in recent work~\cite{tufano2022using, pornprasit2023d, zhou2023EditProgress}.
First, the evaluation of Guo~\ea~\cite{guo2023exploring} overlooks the other benchmarks that are used in recent work~\cite{tufano2022using, pornprasit2023d, zhou2023EditProgress} since they only conducted the experiment on Li~\ea's~\cite{li2022automating} dataset and their collected dataset.
Second, the experiment of Guo~\ea~\cite{guo2023exploring} lacks the comparison between \chatGPT~and the other existing code review automation approaches~\cite{tufano2022using, pornprasit2023d}.
% , since Guo~\ea~\cite{guo2023exploring} only conducted the experiment with \CodeReviewerModel~\cite{li2022automating} and \chatGPT.
Thus, little is known about the generalizability of \chatGPT~on the other benchmarks, and the performance of \chatGPT~when compared to the existing code review automation approaches.
% By filling these gaps, practitioners would have more information to help them decide what tools or approaches they should adapt to automate code review tasks.
By filling these gaps, we could ensure the generalizability of \chatGPT~for code review automation, which could help practitioners decide what tools or approaches they should adapt to automate code review tasks.
% practitioners would have more information to help them decide what tools or approaches they should adapt to automate code review tasks.

% the performance of \chatGPT~on their newly collected dataset is better than that of \CodeReviewerModel~\cite{li2022automating}.

% generalization capabilities than CodeReviewer when applied to unseen datase


% Second, the
\textbf{The evaluation in previous studies~\cite{tufano2022using, pornprasit2023d, li2022automating, guo2023exploring} only relies on the patches in the historical review records.}
In particular, these studies evaluate code review automation approaches to find to what extent the generated code is similar to or the same as the ones in the historical review records.
However, prior work~\cite{winter2022developers, kochhar2016practitioners} found that developers do not blindly trust the recommendations generated by automated approaches.
For example, Winter~\ea~\cite{winter2022developers} conducted a survey study with developers to understand their perceptions on automatic program repair approaches.
The survey results showed that developers would make decisions before applying the recommendations that are generated by automated approaches.
Thus, based on this finding, human evaluation for alternative recommendations (i.e., the recommendations that are not exactly the same as ground truth) should be considered.
% generated by code review automation approaches should be considered when evaluating such approaches.
By doing so, researchers could understand the perception of practitioners on the alternative recommendations, which could be useful for developing code review automation approaches that can satisfy practitioners' expectations.

% are similar to ACR tools. 47.0% 
% expect that the generated refined code is similar to or the same as the ones in the historical review records.
% However, these studies do not include the human evaluation of alternative recommendations (i.e., the recommendations that are not exactly the same as ground truth), which should also be considered since Bacchelli~\ea~\cite{bacchelli2013expectations} find that developers do code review to find alternative solutions (e.g., better implementation).
% The evaluation of alternative recommendations should also be considered since Bacchelli~\ea~\cite{bacchelli2013expectations} find that developers do code review to find alternative solutions (e.g., better implementation).
% Thus, little is known about the perception of practitioners on the alternative recommendations.


The limitations explained above motivate us to address the following two research questions:

\textbf{(RQ1) \rqI}

\textbf{(RQ2) \rqII}


==> section-exp-only/RelatedWork.tex <==
\section{Related Work} \label{sec:RelatedWork}

In this section, we describe the literature that is related to our study.

% \subsection{ChatGPT in Software Engineering}

% Recently, \chatGPT~has been applied to various software engineering tasks.
% For example, Plein~\ea~\cite{plein2023automatic} conducted a feasibility study on using~\chatGPT~for automatic test case generation based on bug reports.
% Xiong~\ea~\cite{xiong2023program} explore the ability of \chatGPT~for program testing task.
% Sch{\"a}fer~\ea~\cite{xiong2023program} conducted an empirical evaluation of \chatGPT~for automated unit test generation.
% Deligiannis~\ea~\cite{deligiannis2023fixing} proposed \chatGPT~based approach for fixing compilation errors in Rust.
% Lastly, Deligiannis~\ea~\cite{eliseeva2023commit} presented \chatGPT~based approach for commit message generation task.
% Different from the above studies, our study focuses on the evaluation of \chatGPT~for code review automation task.

\subsection{LLM in software engineering}

Recently, a number of LLMs for code were proposed~\cite{fried2022incoder, li2023starcoder, luo2023wizardcoder, chen2021evaluating, roziere2023codeLLaMa, anil2023palm2, achiam2023gpt}.
For example, Roziere~\ea~\cite{roziere2023codeLLaMa} proposed Code LLaMa, a pre-trained decoder model for code which is based on LLaMa 2 model~\cite{touvron2023llama2}.
Li~\ea~\cite{li2023starcoder} proposed, a decoder-only transformer model~\cite{Vaswani2017} that is pre-trained with the source code from GitHub and addition python code. 
Besides, LLMs-based approaches were developed to support various software engineering tasks~\cite{chen2024large, xu2023prompting, dilhara2024unprecedented, misu2024towards, jiang2023llmparser, zhang2024automated, yang2023apidocbooster}.
For instance, Yang~\ea~\cite{yang2023apidocbooster} developed an LLM-based approach for augmenting API documentation.
Chen~\ea~\cite{chen2024large} presented RLCE, an LLM-based approach for repository-level automated program repair.



% \subsection{Recommendation System in Code Review}

\subsection{AI--based Approaches to Support Developers in Code Review}

Prior work presented various AI--based approaches to support developers in code review.
For example, researchers proposed machine learning--based approaches for reviewer recommendation~\cite{thongtanunam2014improving,thongtanunam2015should,balachandran2013reducing,rahman2016correct,ouni2016search, ruangwan2018emse}, review comment generation~\cite{hong2022commentfinder, siow2020core, tufano2022using}, and review task prioritization based on code change characteristics~\cite{fan2018early, thongtanunam2017review, maddila2019predicting}.
While these approaches could help developers reduce their effort, patch authors still have to revise their submitted patch until it is approved by reviewers.
Thus, code review automation approaches~\cite{tufano2019learning, tufan2021towards, li2022automating, pornprasit2023d, AutoTransform} were proposed to help developers revise their submitted patches.


==> section-exp-only/Result-old-2.tex <==

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Prompt template for each dataset}
%   \label{tab:prompt-template}
%     \begin{tabular}{|p{0.25\columnwidth}|p{0.65\columnwidth}|}
%     \hline
%     Task  & \multicolumn{1}{l|}{Prompt} \\
%     \hline
%     \emph{\CodeCommentToCode} (for \tufanoData~and \CodeReviewerData) & // Example current version of code (1)\newline    \textless input code\textgreater\newline\newline// Example reviewer comment (1)\newline    \textless input comment\textgreater\newline\newline// Example next version of code (1)\newline    \textless output code\textgreater\newline\newline...\newline\newline Improve the given current version of code below based on the given reviewer's comment (the improved code should follow the format of the provided examples)\newline\newline\newline// Current version of code:\newline    \textless input code\textgreater\newline\newline// Reviewer comment:\newline    \textless input comment\textgreater \\
%     \hline
%    \emph{\CodeToCode} (for \tufanoData) & // Example current version of code (1) \newline    \textless input code\textgreater\newline\newline// Example next version of code (1)\newline    \textless output code\textgreater\newline\newline...\newline\newline Improve the given current version of code below (the improved code should follow the format of the provided examples)\newline\newline// Current version of code:\newline    \textless input code\textgreater \\
%     \hline
%     \emph{\CodeToCode} (for \DACTData) & // Example first version of code (1):\newline     \textless input code\textgreater\newline\newline // Example of the code that reviewers approve (1) \newline    \textless output code\textgreater \newline\newline …\newline\newline\newline Improve the code below so that reviewers will approve (the improved code should follow the format of the provided examples)\newline\newline    \textless input code\textgreater \\
%     \hline
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%


\begin{figure}[t]
     \centering
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page=1, trim = {0 11cm 3cm 0}, clip]{figure/prompt-templates-new.pdf}
         % \caption{Prompt template (few-shot learning) for \emph{\CodeCommentToCode~task} (\tufanoData~datasets)}
         \caption{Prompt template for \emph{\CodeCommentToCode~task}}
         \label{fig:few-shot-with-comment}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page=2, trim = {0 12cm 3cm 0}, clip]{figure/prompt-templates-new.pdf}
         % \caption{Prompt template (few-shot learning) for \emph{\CodeToCode~task} (\tufanoData~and \DACTData~datasets)}
         \caption{Prompt template for \emph{\CodeToCode~task}}
         \label{fig:few-shot-no-comment}
     \end{subfigure}
    \par\bigskip 
     % \begin{subfigure}[]{\columnwidth}
     %     \centering
     %     \includegraphics[width=\columnwidth, page=3, trim = {0 9cm 0 0}, clip]{figure/prompt-templates.pdf}
     %     \caption{Prompt template (0-shot learning) for \emph{\CodeCommentToCode~task} (\tufanoData~datasets)}
     %     \label{fig:zero-shot-with-comment}
     % \end{subfigure}
     % \par\bigskip 
     % \begin{subfigure}[]{\columnwidth}
     %     \centering
     %     \includegraphics[width=\columnwidth, page=4, trim = {0 12cm 0 0}, clip]{figure/prompt-templates.pdf}
     %     % \caption{Prompt template (0-shot learning) for \emph{\CodeToCode~task} (\tufanoData~and \DACTData~datasets)}
     %     \caption{Prompt template (without examples) for \emph{\CodeToCode~task}}
     %     \label{fig:zero-shot-no-comment}
     % \end{subfigure}
        \caption{Prompt template for RQ1}
        \label{fig:prompt-template-0-shot}
\end{figure}


\begin{figure}[htbp]
     \centering
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page=3, trim = {0 1cm 2cm 0}, clip]{figure/prompt-templates-new.pdf}
         % \caption{Prompt template (few-shot learning) for \emph{\CodeCommentToCode~task} (\tufanoData~datasets)}
         \caption{Prompt template for \emph{\CodeCommentToCode~task} (\tufanoData~dataset)}
         \label{fig:few-shot-with-comment}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page=4, trim = {0 1cm 0 0}, clip]{figure/prompt-templates-new.pdf}
         % \caption{Prompt template (few-shot learning) for \emph{\CodeToCode~task} (\tufanoData~and \DACTData~datasets)}
         \caption{Prompt template for \emph{\CodeCommentToCode~task} (\CodeReviewerData~dataset)}
         \label{fig:few-shot-no-comment}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page=5, trim = {0 3cm 2cm 0}, clip]{figure/prompt-templates-new.pdf}
         % \caption{Prompt template (0-shot learning) for \emph{\CodeToCode~task} (\tufanoData~and \DACTData~datasets)}
         \caption{Prompt template for \emph{\CodeToCode~task} (\tufanoData~and \DACTData~dataset)}
         \label{fig:zero-shot-no-comment}
     \end{subfigure}
        \caption{Prompt template for each task (few-shot).}
        \label{fig:prompt-templates-few-shot}
\end{figure}


\begin{figure}[ht]
     \centering
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, page=1]{figure/exact_match_intersection.pdf}
         \caption{\CodeReviewerData~dataset}
         \label{fig:em-codereviewer}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, page=2]{figure/exact_match_intersection.pdf}
         \caption{\DACTData~dataset}
         \label{fig:em-dact}
     \end{subfigure}
    \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, page=3]{figure/exact_match_intersection.pdf}
         \caption{\tufanoData~dataset (\CodeCommentToCode~task)}
         \label{fig:em-tufano-code-comment}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, page=4]{figure/exact_match_intersection.pdf}
         \caption{\tufanoData~dataset (\CodeToCode~task)}
         \label{fig:em-tufano-code}
     \end{subfigure}
     
    \caption{Exact match for each dataset. (will make changes later)}
    \label{fig:EM}
\end{figure}



% Table generated by Excel2LaTeX from sheet 'for-RENE-submission'
\begin{table}[ht]
  \centering
  \caption{Experiment results of \tufanoData~dataset.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
\cline{2-5}    \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\CodeCommentToCode~task} & \multicolumn{2}{c|}{\CodeToCode~task} \\
\cline{2-5}    \multicolumn{1}{c|}{} & EM  & CodeBLEU & EM  & CodeBLEU \\
    \hline
    TufanoT5 & 2,418 & 79.48 & 932  & 77.26 \\
    \hline
    Guo~\ea~\cite{guo2023exploring} & 1,882  & 73.76 & 286  & 74.4 \\
    \hline
    \ChatGPTFewShot & 3,460  & 82.22 &   &  \\
    \hline
    \end{tabular}%
  }
  \label{tab:Tufano-Data-result}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'for-RENE-submission'
\begin{table}[ht]
  \centering
  \caption{Experiment results of \DACTData~dataset.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
\cline{2-7}    \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{exact match} & \multicolumn{3}{c|}{CodeBLEU} \\
\cline{2-7}    \multicolumn{1}{c|}{} & google & ovirt & android & google & ovirt & android \\
    \hline
    D-ACT & 74    & 48    & 12    & 81.85 & 79.77 & 75.99 \\
    \hline
    Guo's approach & 6     & 18    & 5     & 76.21 & 67.57 & 68.49 \\
    \hline
    ChatGPT (few-shot) & 61    & \textbf{56} & \textbf{23} & \textbf{82.53} & 75.8  & \textbf{77.15} \\
    \hline
    \end{tabular}%
  }
  \label{tab:D-ACT-Data-result}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'for-RENE-submission'
\begin{table}[ht]
  \centering
  \caption{Experiment results of \CodeReviewerData~dataset.}
    \begin{tabular}{|c|c|c|}
\cline{2-3}    \multicolumn{1}{c|}{} & EM  & CodeBLEU \\
    \hline
    % Guo~\ea~\cite{guo2023exploring} & 3,524  & -0.35 & 59.72 \\
    % \hline
    CodeReviewer & 4,354  &  55.43 \\
    \hline
    \ChatGPTFewShot & 3,453  & 48.14 \\
    \hline
    \end{tabular}%
  \label{tab:CodeReviewer-data-result}%
\end{table}%


\section{Results} \label{sec:results}


In this section, we present the results of the following three research questions.


\textbf{RQ1: \rqI}

\textbf{Approach.}
To address this RQ, we analyze the revised code generated by \ChatGPTGuo~and the existing code review automation approaches (i.e., \Tufanomodel~and \DACTmodel).
To do so, we first apply \ChatGPTGuo~on the testing dataset of \tufanoData~and \DACTData~datasets, by adapting the best prompt (as shown in Figure~\ref{fig:prompt-template-0-shot}) and temperature value presented by Guo~\ea~\cite{guo2023exploring}.
Then, we compare the results of \ChatGPTGuo~with \Tufanomodel~and \DACTmodel~which are obtained from the replication package.


% To address this RQ, we analyze the revised code generated by \ChatGPTFewShot~ and Guo~\ea's approach~\cite{guo2023exploring} on \CodeReviewerData~dataset.
% To do few-shot learning, we create a prompt for each test sample in the testing dataset collected by Li~\ea~\cite{li2022automating}.
% To do so, we use BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to select three pairs of input and output from the training set for each testing sample.
% We use BM25~\cite{robertson2009probabilistic} since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that it can outperform a random sample selection approach.
% % We then add the selected examples of each test set to the prompt created by Guo~\ea~\cite{guo2023exploring}.
% % We then use the selected examples of each test sample and a test sample to create a prompt based on the template in Figure~\ref{fig:few-shot-with-comment}.
% Then, for each test sample, we use the selected examples to create a prompt based on the template in Figure~\ref{fig:few-shot-with-comment}.
% After that, we use the created prompts to generate results from \chatGPT.
% Finally, we compare the performance of the obtained results with the results of Guo~\ea~\cite{guo2023exploring} which are obtained from the replication package.

\textbf{Result. \Tufanomodel~and \DACTmodel~achieve at least 28.48\% and 140\% higher EM than \ChatGPTGuo, respectively.}
Table~\ref{tab:Tufano-Data-result} shows the performance measure of \Tufanomodel~and \ChatGPTGuo~with respect to EM and CodeBLEU.
The table shows that for \CodeCommentToCode~task, \Tufanomodel~achieves 28.48\% ($\frac{2,418-1,882}{1,882}$) higher EM and 7.75\% ($\frac{79.48-73.76}{73.76}$) higher CodeBLEU than \ChatGPTGuo.
Figure~\ref{} also shows that there are ... test samples that only \Tufanomodel~can correctly generate, ... test samples that \Tufanomodel~and \ChatGPTGuo~can correctly generate, and ... test samples that only \ChatGPTGuo~can correctly generate.
For \CodeToCode~task, \Tufanomodel~achieves 216.78\% ($\frac{906-286}{286}$) higher EM and 3.84\% ($\frac{77.26-74.4}{74.4}$) higher CodeBLEU than \ChatGPTGuo.
Figure~\ref{} also shows that there are ... test samples that only \Tufanomodel~can correctly generate, ... test samples that \Tufanomodel~and \ChatGPTGuo~can correctly generate, and ... test samples that only \ChatGPTGuo~can correctly generate.
The results indicate that \Tufanomodel~is more accurate and can generate revised code that is more similar to the actual revised code than \ChatGPTGuo.

Table~\ref{tab:D-ACT-Data-result} shows the performance measure of \ChatGPTGuo~and \DACTmodel~with respect to EM and CodeBLEU.
The table shows that \DACTmodel~achieves at least 140\% ($\frac{12-5}{5}$) higher EM and 7.4\% ($\frac{81.85-76.21}{76.21}$) higher CodeBLEU than \ChatGPTGuo.
Figure~\ref{} also shows that there are ... test samples that only \DACTmodel can correctly generate, ... test samples that \DACTmodel~and \ChatGPTGuo~can correctly generate, and ... test samples that only \ChatGPTGuo~can correctly generate.
The results indicate that \DACTmodel~is more accurate and can generate revised code that is more similar to the actual revised code than \ChatGPTGuo.


\resultBox{\textbf{Summary of RQ1:} \Tufanomodel~and \DACTmodel~outperform \ChatGPTGuo~in terms of EM and CodeBLEU.}

% \textbf{Result. Guo~\ea~\cite{guo2023exploring}'s approach achieves 1.67\%  higher EM than \ChatGPTFewShot.}
% Table~\ref{tab:CodeReviewer-data-result} shows the performance measure of Guo~\ea's approach~\cite{guo2023exploring}, and \ChatGPTFewShot~with respect to EM, EP and CodeBLEU on \CodeReviewerData~dataset.
% The table shows that Guo~\ea~\cite{guo2023exploring}'s approach achieves 1.67\% ($\frac{3,524-3,466}{3,466}$) and 36.04\% ($\frac{59.72-43.9}{43.9}$) higher EM and CodeBLEU than \ChatGPTFewShot, respectively.
% Figure~\ref{fig:em-codereviewer} also shows that there are 933 test samples that only Guo's approach~\cite{guo2023exploring} can correctly generate, 2,591 test samples that Guo's approach~\cite{guo2023exploring} and \ChatGPTFewShot~can correctly generate, and 875 test samples that only \ChatGPTFewShot~can correctly generate.
% These results indicate that Guo~\ea's approach~\cite{guo2023exploring} is more accurate and can generate revised code that is more similar to the actual revised code than \ChatGPTFewShot.
% On the other hand, we find that Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~achieve negative EP (-0.35 and -0.43, respectively).
% These results indicate that both Guo~\ea~\cite{guo2023exploring}'s approach and \ChatGPTFewShot~still make more mistake when generating revised code.

% \resultBox{\textbf{Summary of RQ1:} Using few-shot learning does not help Guo~\ea's approach to generate more correct revised code on \CodeReviewerData~dataset.}

\textbf{RQ2: \rqII}

\textbf{Approach.}
To address this RQ, we analyze the revised code generated by \ChatGPTFewShot~and the existing code review automation approaches (i.e., \Tufanomodel, \DACTmodel~and \CodeReviewerModel).
To do so, we first use \ChatGPTFewShot~to generate the revised code from a given set of examples (i.e., a pair of given code and revised code) and the given code in test sets.
In particular, we use BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to select three pairs of input and output from the training set for each testing sample since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that it can outperform a random sample selection approach.
% To do so, we first use BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to select three pairs of input and output from the training set for each testing sample.
% We use BM25~\cite{robertson2009probabilistic} since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that it can outperform a random sample selection approach.
Then, for each test sample, we use the selected examples to create a prompt based on the template in Figure~\ref{fig:prompt-templates-few-shot}.
Finally, we compare the results from \ChatGPTFewShot~with the results of the existing code review automation approaches (i.e., \CodeReviewerModel, \Tufanomodel~and \DACTmodel) which are obtained from the replication package.


\textbf{Result. \willdo}
Table~\ref{tab:Tufano-Data-result} shows the performance measure of \ChatGPTFewShot~and \Tufanomodel~with respect to EM and CodeBLEU.
The table shows that for \CodeCommentToCode~task, \ChatGPTFewShot~achieves 43.09\% ($\frac{3,460-2,418}{2,418}$) higher EM and 7.75\% ($\frac{82.22-79.48}{79.48}$) higher CodeBLEU than \ChatGPTGuo.
Figure~\ref{} also shows that there are ... test samples that only \ChatGPTFewShot~can correctly generate, ... test samples that \ChatGPTFewShot~and \Tufanomodel~can correctly generate, and ... test samples that only \Tufanomodel~can correctly generate.
For \CodeToCode~task, \ChatGPTFewShot~achieves ...\% ($\frac{...-906}{906}$) higher EM and ...\% ($\frac{...-77.26}{77.26}$) higher CodeBLEU than \Tufanomodel.
Figure~\ref{} also shows that there are ... test samples that only \ChatGPTFewShot~can correctly generate, ... test samples that \ChatGPTFewShot~and \Tufanomodel~can correctly generate, and ... test samples that only \Tufanomodel~can correctly generate.
The results indicate that \ChatGPTFewShot~is more accurate and can generate revised code that is more similar to the actual revised code than \Tufanomodel.

Table~\ref{tab:D-ACT-Data-result} shows  that \ChatGPTFewShot~achieves 16.67\% ($\frac{56-48}{48}$) and 91.67\% ($\frac{23-12}{12}$) higher EM than \DACTmodel~for Ovirt and Android, respectively while achieving 17.57\% ($\frac{61-74}{74}$) lower EM than \DACTmodel~for Google.
Figure~\ref{} also shows that there are ... test samples that only \ChatGPTFewShot~can correctly generate, ... test samples that \ChatGPTFewShot~and \DACTmodel~can correctly generate, and ... test samples that only \DACTmodel~can correctly generate.
In addition, \ChatGPTFewShot~achieves 0.83\% ($\frac{82.53-81.85}{81.85}$) and 1.53\% ($\frac{77.15-75.99}{75.99}$) higher CodeBLEU than \DACTmodel~for Google and Android, respectively while achieving 4.98\% ($\frac{75.8-79.77}{79.77}$) lower CodeBLEU than \DACTmodel~for Ovirt.
The results indicate that \ChatGPTFewShot~partially outperforms \DACTmodel.

Table~\ref{tab:CodeReviewer-data-result} shows the performance measure of \ChatGPTFewShot~and \CodeReviewerModel~with respect to EM and CodeBLEU.
The table shows that \CodeReviewerModel~achieves 26.09\% ($\frac{4,354-3,453}{3,453}$) higher EM and 15.14\% ($\frac{55.43-48.14}{48.14}$) higher CodeBLEU than \ChatGPTFewShot.
Figure~\ref{} also shows that there are ... test samples that only \CodeReviewerModel~can correctly generate, ... test samples that \CodeReviewerModel~and \ChatGPTFewShot~can correctly generate, and ... test samples that only \ChatGPTFewShot~can correctly generate.
The results indicate that \ChatGPTFewShot~does not outperform \CodeReviewerModel.

\resultBox{\textbf{Summary of RQ2:} \ChatGPTFewShot~outperforms \Tufanomodel~and \DACTmodel, but underperform \CodeReviewerModel.}


% Table~\ref{tab:Tufano-Data-result} shows the performance measures of Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~with respect to EM, EP and CodeBLEU for \tufanoData~dataset.
% For the \CodeCommentToCode~task, we find that \ChatGPTFewShot~achieves 30.74\% ($\frac{2,752-2,105}{2,105}$) and 3.2\% ($\frac{78.59-76.15}{76.15}$) higher EM and CodeBLEU than Guo~\ea's approach~\cite{guo2023exploring}, respectively.
% Figure~\ref{fig:em-tufano-code-comment} also shows that there are 456 test samples that only Guo's approach~\cite{guo2023exploring} can correctly generate, 1,649 test samples that Guo's approach~\cite{guo2023exploring} and \ChatGPTFewShot~can correctly generate, and 1,103 test samples that only \ChatGPTFewShot~can correctly generate.
% The results indicate that \ChatGPTFewShot~is more accurate and can generate revised code that is more similar to the actual revised code than Guo~\ea's approach~\cite{guo2023exploring}.
% However, we find that \ChatGPTFewShot~and Guo~\ea's approach~\cite{guo2023exploring} achieves negative EP (-0.13 and -0.04, respectively), indicating that \ChatGPTFewShot~and Guo~\ea's approach~\cite{guo2023exploring} make more mistake towards generating revised code.

% On the other hand, for the \CodeToCode~task, we find that \ChatGPTFewShot~achieves 235.65\% ($\frac{1,111-331}{331}$) higher EM than Guo~\ea's approach~\cite{guo2023exploring}.
% Besides, Figure~\ref{fig:em-codereviewer} shows that there are 130 test samples that only Guo's approach~\cite{guo2023exploring} can correctly generate, 201 test samples that Guo's approach~\cite{guo2023exploring} and \ChatGPTFewShot~can correctly generate, and 910 test samples that only \ChatGPTFewShot~can correctly generate.
% The results indicate that \ChatGPTFewShot~is more accurate than Guo~\ea's approach~\cite{guo2023exploring}.
% However, \ChatGPTFewShot~achieves 0.92\% ($\frac{75.42-76.12}{75.42}$) lower CodeBLEU than Guo~\ea's approach~\cite{guo2023exploring}.
% We also find that both \ChatGPTFewShot and Guo~\ea's approach~\cite{guo2023exploring} achieve negative EP (-0.14 and -0.18, respectively).
% The results indicate that both approaches make more mistakes when generating revised code.


% Table~\ref{tab:D-ACT-Data-result} shows the performance measures of Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~with respect to EM, EP and CodeBLEU on \DACTData~dataset.
% The table shows that \ChatGPTFewShot~achieves 69.23\% ($\frac{22-13}{13}$) higher EM than Guo~\ea's approach~\cite{guo2023exploring} for the Google project while achieving similar EM to Guo~\ea's approach~\cite{guo2023exploring} for the Android and Ovirt projects.
% In addition, Figure~\ref{fig:em-dact} shows that for all software projects, there are 31 test samples that only Guo's approach~\cite{guo2023exploring} can correctly generate, 14 test samples that Guo's approach~\cite{guo2023exploring} and \ChatGPTFewShot~can correctly generate, and 40 test samples that only \ChatGPTFewShot~can correctly generate.
% The results indicate that \ChatGPTFewShot~is more accurate than Guo~\ea's approach~\cite{guo2023exploring} for the Google project.
% In contrast, we observe that Guo~\ea's approach~\cite{guo2023exploring} achieves 1\% ($\frac{68.49-67.83}{67.83}$) - 5\% ($\frac{76.21-72.55}{72.55}$) higher CodeBLEU than \ChatGPTFewShot, indicating that Guo~\ea's approach~\cite{guo2023exploring} generates revised code that is more similar to the actual revised code than \ChatGPTFewShot.
% On the other hand, both Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~achieve negative EP for all projects, indicating that  Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~still make more mistake when generating revised code.

% \resultBox{\textbf{Summary of RQ2:} Using few-shot learning could help Guo~\ea's approach to correctly generate more revised code for \tufanoData~and \DACTData~dataset. However, in overall, Guo~\ea's approach still generates revised code more similar to the actual revised code than \ChatGPTFewShot.}


% Table~\ref{tab:D-ACT-Data-result} shows that \DACTmodel~achieves 85.19\% ($\frac{50-27}{27}$) - 469.23\% ($\frac{74-13}{13}$) higher EM than \chatGPT.
% % We also find that for all software projects in the \DACTData~dataset, there are 127 test samples that only \DACTmodel~can correctly generate, and 7 test samples that \DACTmodel~and \chatGPT~can correctly generate.
% % Similarly, there are 2,662 test samples that only \CodeReviewerModel~can correctly generate, and 1,171 test samples that \CodeReviewerModel~and \chatGPT~can correctly generate.
% % \CodeReviewerModel~and \DACTmodel~achieve 430.89\% ($\frac{3,833-722}{722}$) and at least 50\% ($\frac{12-8}{8}$) higher EM than \chatGPT, respectively.
% % We also find that there are 3,349 test samples that only \CodeReviewerModel~can correctly generate, and 238 test samples that \CodeReviewerModel~and \chatGPT~can correctly generate.
% % Similarly, for the whole test set in the \DACTData~dataset, there are 132 test samples that only \DACTmodel~can correctly generate, and 2 test samples that \DACTmodel~and \chatGPT~can correctly generate.
% In addition, \DACTmodel~achieves 7.4\% ($\frac{81.85-73.63}{76.21}$) - 18.06\% ($\frac{79.77-67.57}{67.57}$) higher CodeBLEU than \chatGPT.
% We also observe that while \DACTmodel~achieves positive EP on Android, \chatGPT~achieves negative EP for all software projects in this dataset.




% \textbf{RQ3: \rqIII}

% \textbf{Approach.}
%     To address this RQ, we analyze the revised code generated by \ChatGPTFewShot~in RQ2 and the existing code review automation approaches~\cite{tufano2022using, pornprasit2023d, li2022automating}.
%     The revised code generated by such approaches~\cite{tufano2022using, pornprasit2023d, li2022automating} is obtained from the replication packagess~\cite{tufano2022using, pornprasit2023d, guo2023exploring}.
%     % similar to RQ2, we obtain the results of the existing code review automation approaches~\cite{tufano2022using, pornprasit2023d, li2022automating}.
%     After that, we evaluate the performance of \ChatGPTFewShot~and the existing code review automation approaches using the same evaluation measures as RQ1 and RQ2.
%     % To address this RQ, we conduct the experiment to evaluate the performance of \chatGPT~against the existing code review automation approaches (i.e., TufanoT5~\cite{tufano2022using} and D-ACT~\cite{pornprasit2023d}).
%     % % To do so, we first collect the Gerrit dataset and obtain the dataset from prior work~\cite{pornprasit2023d}.
%     % To do so, we first obtain the dataset from prior work~\cite{pornprasit2023d, tufano2022using}.
%     % Then, we obtain the results from \chatGPT~by using the prompt and temperature value as reported in RQ2 of Guo~\ea's work~\cite{guo2023exploring}.
%     % After that, we obtain the results of \DACTmodel~and \Tufanomodel~from the replication packages.
%     % Finally, we evaluate the performance of \chatGPT~and the existing code review automation approaches using the evaluation measures described in Section~\ref{sec:study-design}.
%     % Note that we remove code comments during the evaluation since we only focus on generating improved code.



% \textbf{Result. \CodeReviewerModel~and \DACTmodel~achieves 6.72\% and at least 92.31\% higher EM than \ChatGPTFewShot, respectively while \ChatGPTFewShot~achieves at least 13.81\% higher EM than \Tufanomodel.}
% Table~\ref{tab:CodeReviewer-data-result} shows that \CodeReviewerModel~achieves 6.72\% ($\frac{3,699-3,466}{3,466}$) and 8.04\% ($\frac{47.43-43.9}{43.9}$) higher EM and CodeBLEU than \ChatGPTFewShot, respectively.
% Figure~\ref{fig:em-codereviewer} also shows that there are 1,624 test samples that only \ChatGPTFewShot~can correctly generate, 1,842 test samples that \ChatGPTFewShot~and \CodeReviewerModel~can correctly generate, and 1,857 test samples that only \CodeReviewerModel~can correctly generate.
% These results indicate that \CodeReviewerModel~is more accurate and can generate revised code that is more similar to the actual revised code than \ChatGPTFewShot.
% On the other hand, we find that \CodeReviewerModel~achieves positive EP (0.37) while \ChatGPTFewShot~achieve negative EP (-0.43).
% These results indicate that \CodeReviewerModel~makes better progress towards generating revised code than \ChatGPTFewShot.

% Table~\ref{tab:Tufano-Data-result} shows that for the \CodeCommentToCode~task, \ChatGPTFewShot~achieves 13.81\% ($\frac{2,752-2,418}{2,418}$) and 1.13\% ($\frac{79.48-78.59}{78.59}$) higher EM and CodeBLEU than \Tufanomodel, respectively.
% In addition, Figure~\ref{fig:em-tufano-code-comment} shows that there are 2,349 test samples that only \ChatGPTFewShot~can correctly generate, 403 test samples that \ChatGPTFewShot~and \Tufanomodel~can correctly generate, and 2,015 test samples that only \Tufanomodel~can correctly generate.
% The results indicate that \ChatGPTFewShot~is more accurate and can generate revised code that is more similar to the actual revised code than \Tufanomodel.
% However, we find that \Tufanomodel~achieves positive EP (0.25) while \ChatGPTFewShot~achieves negative EP (-0.04), indicating that \Tufanomodel~makes better progress towards generating revised code than \ChatGPTFewShot.

% % In addition, we find that \Tufanomodel~and \ChatGPTFewShot~achieve higher EP.


% On the other hand, for the \CodeToCode~task, we find that \ChatGPTFewShot~achieves 19.21\% ($\frac{1,111-932}{932}$) higher EM than \Tufanomodel.
% Besides, Figure~\ref{fig:em-tufano-code} shows that there are 1,044 test samples that only \ChatGPTFewShot~can correctly generate, 67 test samples that \ChatGPTFewShot~and \Tufanomodel~can correctly generate, and 865 test samples that only \Tufanomodel~can correctly generate.
% The results indicate that \ChatGPTFewShot~is more accurate than \Tufanomodel.
% However, \Tufanomodel~achieves 2.43\% ($\frac{77.26-75.42}{75.42}$) higher CodeBLEU than \ChatGPTFewShot.
% We also find that \ChatGPTFewShot~achieves negative EP (-0.14) while \Tufanomodel~achieves positive EP (0.02), indicating that \Tufanomodel~makes better progress towards generating revised code than \ChatGPTFewShot.

% % \ChatGPTFewShot and Guo~\ea's approach~\cite{guo2023exploring} achieve negative EP (-0.14 and -0.18, respectively).
% % The results indicate that both approaches make more mistakes when generating revised code.


% Table~\ref{tab:D-ACT-Data-result} shows that \DACTmodel~achieves 92.31\% ($\frac{50-26}{26}$) - 236.36\% ($\frac{74-22}{22}$) and 12.03\% ($\frac{75.99-67.83}{67.83}$) - 20.41\% ($\frac{79.77-66.25}{66.25}$) higher EM and CodeBLEU than \ChatGPTFewShot, respectively.
% Figure~\ref{fig:em-tufano-code} also shows that there are 47 test samples that only \ChatGPTFewShot~can correctly generate, 7 test samples that \ChatGPTFewShot~and \DACTmodel~can correctly generate, and 129 test samples that only \DACTmodel~can correctly generate.
% The results indicate that \DACTmodel~is more accurate and can generate revised code that is more similar to the actual revised code than \ChatGPTFewShot.
% We also find that while \ChatGPTFewShot~achieves negative EP for all projects, \DACTmodel~achieves positive EP for Android project.

% \resultBox{\textbf{Summary of RQ3:} Using few-shot learning could help Guo~\ea's approach to correctly generate more revised code than \Tufanomodel. However, this is not the case for \CodeReviewerModel~and \DACTmodel.}


% % indicating that \DACTmodel~is more accurate than \ChatGPTFewShot.
% % In addition, we find that \DACTmodel~achieves 12.03\% - 20.41\% higher CodeBLEU than \ChatGPTFewShot

% % \ChatGPTFewShot~achieves 69.23\% higher EM than Guo~\ea's approach~\cite{guo2023exploring} for the Google project while achieving similar EM similar to Guo~\ea's approach~\cite{guo2023exploring}.
% % The results indicate that \ChatGPTFewShot~is more accurate than Guo~\ea's approach~\cite{guo2023exploring} for the Google project.
% % In contrast, we observe that Guo~\ea's approach~\cite{guo2023exploring} achieves 1\% - 5\% higher CodeBLEU than \ChatGPTFewShot, indicating that Guo~\ea's approach~\cite{guo2023exploring} generates revised code that is more similar to the actual revised code than \ChatGPTFewShot.
% % On the other hand, both Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~achieve negative EP for all projects, indicating that  Guo~\ea's approach~\cite{guo2023exploring} and \ChatGPTFewShot~still make more mistake when generating revised code.


%     % Table~\ref{tab:Tufano-Data-result} shows the performance measures of \Tufanomodel~and \chatGPT~with respect to EM, EP and CodeBLEU for \CodeCommentToCode~and \CodeToCode~tasks.
%     % The table shows that for the 0-shot setting, \Tufanomodel~achieves 14.87\% ($\frac{2,418-2,105}{2,105}$) and 181.57\% ($\frac{932-331}{331}$) higher EM than \chatGPT~for \CodeCommentToCode~and \CodeToCode~tasks, respectively.
%     % % and 122.06\% ($\frac{755-340}{340}$) higher EM than \chatGPT~for \CodeCommentToCode~task and \CodeToCode task, respectively.
%     % % In addition, \Tufanomodel~achieve 5.71\% (for \CodeCommentToCode~task) and 5.46\% (for \CodeToCode~task) higher CodeBLEU than \chatGPT.
%     % % We also find that there are 2,096 test samples that only \Tufanomodel~can correctly generate, and 293 test samples that \Tufanomodel~and \chatGPT~can correctly generate for \CodeCommentToCode~task.
%     % % Similarly, there are 716 test samples that only \Tufanomodel~can correctly generate, and 39 test samples that \Tufanomodel~and \chatGPT~can correctly generate for \CodeToCode~task.
%     % On the other hand, \Tufanomodel~achieves 4.37\% ($\frac{79.48-76.15}{76.15}$) and 1.50\% ($\frac{77.26-76.12}{76.12}$) higher CodeBLEU than \chatGPT~for \CodeCommentToCode~task and \CodeToCode~task, respectively.
%     % We can also see that \Tufanomodel~achieves positive EP for both \CodeCommentToCode~and \CodeToCode~tasks (0.32 and 0.02, respectively), while \chatGPT~achieves negative EP for both tasks (-0.016 and -0.18, respectively).

%     % Table~\ref{tab:D-ACT-Data-result} shows that \DACTmodel~achieves 85.19\% ($\frac{50-27}{27}$) - 469.23\% ($\frac{74-13}{13}$) higher EM than \chatGPT.
%     % % We also find that for all software projects in the \DACTData~dataset, there are 127 test samples that only \DACTmodel~can correctly generate, and 7 test samples that \DACTmodel~and \chatGPT~can correctly generate.
%     % % Similarly, there are 2,662 test samples that only \CodeReviewerModel~can correctly generate, and 1,171 test samples that \CodeReviewerModel~and \chatGPT~can correctly generate.
%     % % \CodeReviewerModel~and \DACTmodel~achieve 430.89\% ($\frac{3,833-722}{722}$) and at least 50\% ($\frac{12-8}{8}$) higher EM than \chatGPT, respectively.
%     % % We also find that there are 3,349 test samples that only \CodeReviewerModel~can correctly generate, and 238 test samples that \CodeReviewerModel~and \chatGPT~can correctly generate.
%     % % Similarly, for the whole test set in the \DACTData~dataset, there are 132 test samples that only \DACTmodel~can correctly generate, and 2 test samples that \DACTmodel~and \chatGPT~can correctly generate.
%     % In addition, \DACTmodel~achieves 7.4\% ($\frac{81.85-73.63}{76.21}$) - 18.06\% ($\frac{79.77-67.57}{67.57}$) higher CodeBLEU than \chatGPT.
%     % We also observe that while \DACTmodel~achieves positive EP on Android, \chatGPT~achieves negative EP for all software projects in this dataset.

==> section-exp-only/Result-old-3.tex <==

% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
% \begin{table*}[htbp]
%   \centering
%   \caption{(RQ3) The evaluation results of fine-tuned ChatGPT.}
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
% \cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
%     \hline
%     ChatGPT (with persona) & 37.70\% & \textbf{49.20\%} & \textbf{21.98\%} & \textbf{83.04\%} & \textbf{6.04\%} & 79.76\% & 2.29\% & \textbf{74.74\%} & 6.14\% & 81.02\% & 2.64\% & \textbf{74.95\%} \\
%     \hline
%     ChatGPT (without persona) & \textbf{37.93\%} & 49.00\% & 22.16\% & 82.99\% & 6.02\% & \textbf{79.81\%} & \textbf{2.34\%} & 74.15\% & \textbf{6.71\%} & \textbf{81.08\%} & \textbf{3.05\%} & 74.67\% \\
%     \hline
%     \end{tabular}%
%   }
%   \label{tab:rq3-result}%
% \end{table*}%


\section{Result} \label{sec:results}


In this section, we present the experiment results of the follwing four research questions.

\noindent \textbf{(RQ1) \rqone}

\noindent \smallsection{Approach}
To address this RQ, we use the prompts in Figure~\ref{fig:prompt-templates} without persona to enable GPT-3.5 to perform 0-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
Then, we measure EM and CodeBLEU of the results obtained from GPT-3.5.
% The results of 0-shot and few-shot learning are denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
GPT-3.5 that we perform 0-shot and few-shot learning are denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  % \makegapedcells
  \centering
  \caption{(RQ2) The evaluation results \ChatGPTZeroShot.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShotWithPersona & 17.07\% & 43.11\% & 12.49\% & 77.32\% & 2.29\% & 73.21\% & \textbf{0.57\%} & 55.88\% & 0.00\% & 50.65\% & 0.22\% & 45.73\% \\
    \hline
    \ChatGPTZeroShotWithoutPersona & \textbf{17.72\%} & \textbf{44.17\%} & \textbf{13.52\%} & \textbf{78.36\%} & \textbf{2.62\%} & \textbf{74.92\%} & 0.49\% & \textbf{61.85\%} & \textbf{0.16\%} & \textbf{61.04\%} & \textbf{0.48\%} & \textbf{56.55\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq2-result-0-shot}%
\end{table*}%



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ2) The evaluation results of \ChatGPTFewShot.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTFewShotWithPersona & 26.28\% & 47.43\% & \textbf{20.03\%} & 81.61\% & \textbf{9.18\%} & 78.98\% & 1.62\% & 74.65\% & 2.45\% & 81.07\% & \textbf{1.67\%} & 73.29\% \\
    \hline
    \ChatGPTFewShotWithoutPersona & \textbf{26.55\%} & \textbf{47.50\%} & 19.79\% & \textbf{81.47\%} & 8.96\% & \textbf{79.21\%} & \textbf{2.34\%} & \textbf{75.33\%} & \textbf{2.89\%} & \textbf{81.40\%} & 1.64\% & \textbf{73.83\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq2-result-few-shot}%
\end{table*}%

\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ2.pdf}
         \caption{\CodeReviewerData~dataset}
         \label{fig:RQ2-1-EM-intersection-CodeRec}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ2.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (with comment)}
         \label{fig:RQ2-1-EM-intersection-tufano-code-comment}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (without comment)}
         \label{fig:RQ2-1-EM-intersection-tufano-code}
     \end{subfigure}
    \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
         \caption{\DACTData~dataset}
         \label{fig:RQ2-1-EM-intersection-D-ACT}
     \end{subfigure}
     
     \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTZeroShot~(with and without persona).}
    \label{fig:changed-token-count}
\end{figure*}



\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=5]{figure/EM-RQ2.pdf}
         \caption{\CodeReviewerData~dataset}
         \label{fig:RQ2-2-EM-intersection-CodeRec}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=6]{figure/EM-RQ2.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
      \caption{\tufanoData~dataset (without comment)}
     \label{fig:RQ2-2-EM-intersection-tufano-code}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=7]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (without comment)}
         \label{fig:RQ2-2-EM-intersection-tufano-code}
     \end{subfigure}
    \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=8]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
         \caption{\DACTData~dataset}
         \label{fig:RQ2-2-EM-intersection-D-ACT}
     \end{subfigure}
     
     \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTFewShot~(with and without persona).}
    \label{fig:changed-token-count}
\end{figure*}


% To address this RQ, we do 0-shot and few-shot learning by first creating the input prompts from the prompt templates in Figure~\ref{fig:0-shot prompt} and~\ref{fig:few-shot prompt}, respectively without using persona.
% To do few-shot learning,  we use BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to select three pairs of input and output from the training set for each testing sample.
% We do so since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform a random sample selection approach.
% Then, we obtain the improved code from GPT-3.5 by using the created input prompts.

% After that, we compare the results of \ChatGPTZeroShot~and \ChatGPTFewShot~in terms of EM and CodeBLEU.

\noindent \smallsection{Result}
\textbf{Few-shot learning helps increase EM and CodeBLEU by at least 46.38\% and 3.97\%, respectively.}
Table~\ref{tab:rq1-result} shows the evaluation results of \ChatGPTZeroShot~and GPT-3.5\textsubscript{few-shot} in terms of EM and CodeBLEU.
The table shows that GPT-3.5\textsubscript{few-shot} achieves EM of 1.64\% - 26.55\%, which is at least 46.38\% ($\frac{19.79-13.52}{13.52}$) higher than \ChatGPTZeroShot.
% 49.38\% ($\frac{26.47-17.72}{17.72}$), 46.38\% ($\frac{19.79-13.52}{13.52}$) and 241.98\% ($\frac{8.96-2.62}{2.62}$) higher EM than \ChatGPTZeroShot~on the \CodeReviewerData, Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment) datasets, respectively.
% The table also shows that \ChatGPTFewShot~achieves at least 241.67\% ($\frac{1.64-0.48}{0.48}$) higher EM than \ChatGPTZeroShot~on the \DACTData~dataset.
The table also shows that GPT-3.5\textsubscript{few-shot} achieves CodeBLEU of 47.55\% - 81.47\%, which is 3.97\% ($\frac{81.47-78.36}{78.36}$) - 33.36\% ($\frac{81.4-61.04}{61.04}$) higher than \ChatGPTZeroShot.
Figure~\ref{fig:RQ1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ1-EM-intersection-D-ACT} show the Venn diagram of the improved code that GPT-3.5\textsubscript{0-shot} and GPT-3.5\textsubscript{few-shot} correctly generate.
The figures show that the improved code that only \ChatGPTFewShot~correctly generates accounts for 38.64\% - 84.29\% of the total improved code correctly generated by \ChatGPTZeroShot~and \ChatGPTFewShot, which is at least 280.8\% higher than \ChatGPTZeroShot. 
% 7.65\% ($\frac{47.55-44.17}{44.17}$), 3.97\% ($\frac{81.47-78.36}{78.36}$) and 5.73\% ($\frac{79.21-74.92}{74.92}$) higher CodeBLEU than \ChatGPTZeroShot~on the \CodeReviewerData, Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, the table shows that GPT-3.5\textsubscript{few-shot} achieves at least 21.79\% ($\frac{75.33-61.85}{61.85}$) higher CodeBLEU than \ChatGPTZeroShot~on the \DACTData~dataset.
The results indicate that few-shot learning could help GPT-3.5 to generate more correct and unique improved code, and generate more similar improved code to actual improved code than 0-shot learning.



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[ht]
  \centering
  \caption{(RQ3) The evaluation results of \ChatGPTFineTune~(with persona).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShot & 17.07\% & 43.11\% & 12.49\% & 77.32\% & 2.29\% & 73.21\% & 0.57\% & 55.88\% & 0.00\% & 50.65\% & 0.22\% & 45.73\% \\
    \hline
    \ChatGPTFewShot & 26.28\% & 47.43\% & 20.03\% & 81.61\% & \textbf{9.18\%} & 78.98\% & 1.62\% & 74.65\% & 2.45\% & \textbf{81.07\%} & 1.67\% & 73.29\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.70\%} & \textbf{49.20\%} & \textbf{21.98\%} & \textbf{83.04\%} & 6.04\% & \textbf{79.76\%} & \textbf{2.29\%} & \textbf{74.74\%} & \textbf{6.14\%} & 81.02\% & \textbf{2.64\%} & \textbf{74.95\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq3-with-persona}%
\end{table*}%



\noindent \textbf{(RQ2) \rqtwo}

\noindent \smallsection{Approach}
% To address this RQ, similar to RQ1, we create the input prompts for GPT-3.5 by using the prompt templates in Figure~\ref{fig:prompt-templates} with persona.
% Then, we obtain the improved code from GPT-3.5 by using the created input prompts.
To address this RQ, we use the prompts in Figure~\ref{fig:prompt-templates} with persona to enable GPT-3.5 to perform 0-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
% we do 0-shot and few-shot learning with GPT-3.5 as explained in Section~\ref{sec:study-design} by using persona in the input prompts. 
Then, similar to RQ1, we measure EM and CodeBLEU of the results obtained from GPT-3.5 that persona is included in the input prompts and GPT-3.5 that persona is not included in the input prompts.
% The results obtained from \ChatGPTZeroShot~and \ChatGPTFewShot~that we include persona in the input prompts are denoted as \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
% Similarly, the results obtained from \ChatGPTZeroShot~and \ChatGPTFewShot~that we do not include persona in the input prompts are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.
\ChatGPTZeroShot~and \ChatGPTFewShot~that persona is included in the input prompts are denoted as \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
Similarly, \hspace{1.5pt} \ChatGPTZeroShot~and GPT-3.5\textsubscript{few-shot} that persona is not included in the input prompts are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.

\noindent \smallsection{Result}
% \textbf{In overall, \ChatGPTZeroShot~and \ChatGPTFewShot~that we use input prompts with persona achieve higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot~that we use input prompts without persona.}
% \textbf{In overall, \ChatGPTZeroShotWithoutPersona~and GPT-3.5-NP\textsubscript{few-shot} achieve higher EM and CodeBLEU than GPT-3.5-WP\textsubscript{few-shot} and \ChatGPTFewShotWithPersona}
\textbf{\ChatGPTZeroShotWithoutPersona~achieves at least 3.81\% and 1.35\% higher EM and CodeBLEU than GPT-3.5-WP\textsubscript{0-shot}, respectively. 
Similarly, \ChatGPTFewShotWithoutPersona~achieves at least 1.03\% and 1.21\% higher EM and \hspace{6pt} CodeBLEU than GPT-3.5-WP\textsubscript{few-shot}, respectively.}
Table~\ref{tab:rq2-result-0-shot} shows the evaluation results of GPT-3.5\textsubscript{0-shot} that persona is included and not included in input prompts.
The table shows that \ChatGPTZeroShotWithoutPersona~achieves EM of 0.16\% - 17.72\%, which is 3.81\% ($\frac{17.72-17.07}{17.07}$) - 118.18\% ($\frac{0.48-0.22}{0.22}$) higher than \ChatGPTZeroShotWithPersona.
% 49.38\% ($\frac{26.47-17.72}{17.72}$), 46.38\% ($\frac{19.79-13.52}{13.52}$) and 241.98\% ($\frac{8.96-2.62}{2.62}$) higher EM than \ChatGPTZeroShot~on the \CodeReviewerData, Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment) datasets, respectively.
% The table also shows that \ChatGPTFewShot~achieves at least 241.67\% ($\frac{1.64-0.48}{0.48}$) higher EM than \ChatGPTZeroShot~on the \DACTData~dataset.
The table also shows that \ChatGPTZeroShotWithoutPersona~achieves CodeBLEU of 44.17\% - 78.36\%, which is 1.35\% ($\frac{78.36-77.32}{77.32}$) - 23.66\% ($\frac{56.55-45.73}{45.73}$) higher than \ChatGPTZeroShotWithPersona.
Figure~\ref{fig:RQ2-1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-1-EM-intersection-D-ACT} show the Venn diagram of the improved code that \ChatGPTZeroShotWithPersona~and GPT-3.5-NP\textsubscript{0-shot} correctly generate.
The figures show that the improved code that only \ChatGPTZeroShotWithoutPersona~correctly generates accounts for 13.82\% - 50\% of the total improved code correctly generated by \ChatGPTZeroShotWithoutPersona~and \ChatGPTZeroShotWithPersona, which is 28.24\% - 225\% higher than \ChatGPTZeroShotWithPersona. 
% The results indicate that using few-shot learning could help GPT-3.5 to generate more correct and unique improved code, and generate more similar improved code to actual improved code than using 0-shot learning.

% The table shows that in terms of EM, \ChatGPTZeroShot~that does not use persona achieves 3.81\% ($\frac{17.72-17.07}{17.07}$), 8.25\% \newline ($\frac{13.52-12.49}{12.49}$), and 14.41\% ($\frac{2.62-2.29}{2.29}$) higher EM than GPT-3.5\textsubscript{0-shot} that uses persona on the \CodeReviewerData, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% On the other hand, for the \DACTData~dataset, \ChatGPTZeroShot~that does not use persona achieves at least 118.18\% ($\frac{0.48-0.22}{0.22}$) higher EM on the Ovirt project while achieving 14.04\% ($\frac{0.49-0.57}{0.57}$) lower EM than \ChatGPTZeroShot~that uses persona on the Android project.
% In terms of CodeBLEU, \ChatGPTZeroShot~that does not use persona achieves 2.46\% ($\frac{44.17-43.11}{43.11}$), 1.35\% ($\frac{78.36-77.32}{77.32}$), and 2.34\% \newline ($\frac{74.92-73.21}{73.21}$) higher CodeBLEU than \ChatGPTZeroShot~that uses persona on the the \CodeReviewerData, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, \ChatGPTZeroShot~that does not use persona achieves at least 10.68\% ($\frac{61.85-55.88}{55.88}$) higher CodeBLEU than \ChatGPTZeroShot~that uses persona on the \DACTData~dataset.

Table~\ref{tab:rq2-result-few-shot} shows the evaluation results of \ChatGPTFewShot~that persona is included and not included in input prompts.
The table shows that \ChatGPTFewShotWithoutPersona~achieves EM of 2.34\% - 26.55\%, which is 1.03\% ($\frac{26.55-26.28}{26.28}$) - 44.44\% ($\frac{2.34-1.62}{1.62}$) higher than GPT-3.5-WP\textsubscript{few-shot}.
On the contrary, for the Tufano\textsubscript{data} dataset, GPT-3.5-WP\textsubscript{few-shot} achieves EM of 9.18\% - 20.03\%, which is 1.21\% ($\frac{20.03-19.79}{19.79}$) - 2.46\% ($\frac{9.18-8.96}{8.96}$) higher than \ChatGPTFewShotWithoutPersona.
The table also shows that GPT-3.5-NP\textsubscript{few-shot} achieves CodeBLEU of 47.55\% - 81.40\%, which is 0.19\% \\($\frac{47.55-47.46}{47.46}$) - 0.91\% ($\frac{75.33-74.65}{74.65}$) higher than \ChatGPTFewShotWithPersona.
Figure~\ref{fig:RQ2-2-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-2-EM-intersection-D-ACT} show the Venn diagram of the improved code that \ChatGPTFewShotWithPersona~and \ChatGPTFewShotWithoutPersona~correctly generate.
The figures show that the improved code that only GPT-3.5-NP\textsubscript{few-shot} correctly generates accounts for \hspace{2pt} 5.03\% - 24.14\% of the total improved code correctly generated by GPT-3.5-NP\textsubscript{few-shot} and \ChatGPTFewShotWithPersona, which is 19.74\% - 84.21\% higher than \ChatGPTFewShotWithPersona.
In contrast, for the Tufano\textsubscript{data} dataset, the improved code that only \ChatGPTFewShotWithPersona~correctly generates accounts for 6.71\% - 10.64\% of the total improved code correctly generated by \ChatGPTFewShotWithoutPersona~and \ChatGPTFewShotWithPersona, which is 20.1\% - 26.06\% higher than \ChatGPTFewShotWithoutPersona.


% The table shows that in terms of EM, \ChatGPTFewShot~that does not use persona achieves 0.88\% \newline ($\frac{26.46-26
% 32}{26.32}$) higher EM than \ChatGPTFewShot~that uses persona on the CodeReviewer\textsubscript{data} dataset, while achieving 1.2\% ($\frac{19.79-20.03}{20.03}$) and 2.4\% ($\frac{8.96-9.18}{9.18}$) lower EM than \ChatGPTFewShot~that uses persona on the \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% On the other hand, \ChatGPTFewShot~that does not use persona achieves at least 17.96\% ($\frac{2.89-2.45}{2.45}$) higher EM than \ChatGPTFewShot~that uses persona on the Android and Google projects while achieving 1.8\% ($\frac{1.64-1.67}{1.67}$) lower EM than \ChatGPTFewShot~that uses persona on the Ovirt project.
% In terms of CodeBLEU, \ChatGPTFewShot~that does not use persona achieves 0.19\% ($\frac{47.55-47.46}{47.46}$) and 0.29\% ($\frac{79.21-78.98}{78.98}$) higher CodeBLEU than \ChatGPTFewShot~that uses persona on the CodeReviewer\textsubscript{data} and \tufanoData~(without comment) datasets, respectively, while achieving 0.17\% ($\frac{47.55-47.47}{47.47}$) lower CodeBLEU than \ChatGPTFewShot~that uses persona on the Tufano\textsubscript{data} (with comment) dataset.
% On the other hand, \ChatGPTFewShot~that does not use persona achieves at least 0.41\% ($\frac{81.4-81.07}{81.07}$) higher than \ChatGPTFewShot~that uses persona on the \DACTData~dataset.
% The above results indicate that using persona does not always help GPT-3.5 to correctly generate more improved code.

The results indicate that in overall, \ChatGPTZeroShot~and \ChatGPTFewShot~that persona is not included in the input prompts can generate more correct and unique improved code and generate more similar improved code to actual improved code than GPT-3.5\textsubscript{0-shot} and \ChatGPTFewShot~that persona is included in the input prompts.



\noindent \textbf{(RQ3) \rqthree}

\noindent \smallsection{Approach}
To address this RQ, we fine-tune GPT-3.5 as explained in Section~\ref{sec:study-design}.
% We do so by using prompts that contain persona and do not contain persona similar to RQ2.
Then, similar to RQ1 and RQ2, we measure EM and CodeBLEU of the results obtained from the fine-tuned GPT-3.5 (the fine-tuned GPT-3.5 models are denoted as \ChatGPTFineTune).
In addition, we analyze the improved code that \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~correctly generate to understand the characteristics of code changes of such improved code.
To do so, we randomly select the improved code that is only correctly generated by a particular model (e.g., we randomly obtain the improved code that only \ChatGPTZeroShot~correctly generates while the others do not.) by using the confidence level of 95\% and the confidence interval of 5\%.
Then, we classify the code change of the selected improved code into three categories (i.e., \textit{fixing bug}, \textit{refactoring} and \textit{other}) by following the taxonomy of code change created by Tufano~\ea~\cite{tufano2019learning}.



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ3) The evaluation results of \ChatGPTFineTune~(without persona).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShot & 17.72\% & 44.17\% & 13.52\% & 78.36\% & 2.62\% & 74.92\% & 0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\
    \hline
    \ChatGPTFewShot & 26.55\% & 47.50\% & 19.79\% & 81.47\% & \textbf{8.96\%} & 79.21\% & 2.34\% & \textbf{75.33\%} & 2.89\% & \textbf{81.40\%} & 1.64\% & 73.83\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.93\%} & \textbf{49.00\%} & \textbf{22.16\%} & \textbf{82.99\%} & 6.02\% & \textbf{79.81\%} & 2.34\% & 74.15\% & \textbf{6.71\%} & 81.08\% & \textbf{3.05\%} & \textbf{74.67\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq3-without-persona}%
\end{table*}%


\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0.5cm 0.7cm 0 0}, clip]{figure/fine-tuned-vs-0-shot-and-few-shot-with-persona-analysis.pdf}
         \caption{The results of GPT-3.5 (with persona)}
         \label{fig:RQ3-analysis-with-persona}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0.5cm 0.7cm 0 0}, clip]{figure/fine-tuned-vs-0-shot-and-few-shot-without-persona-analysis.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
      \caption{The results of GPT-3.5 (without persona)}
     \label{fig:RQ3-analysis-without-persona}
     \end{subfigure}
     % \par\bigskip 

     \caption{(RQ3) The EM achieved by \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~categorized by types of code change.}
    \label{fig:RQ3-analysis}
\end{figure*}



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ4) The evaluation results of GPT-3.5 compared to the existing code review autmation approaches.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-13}    \multicolumn{1}{r|}{} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} & \multicolumn{1}{l|}{exact match} & \multicolumn{1}{l|}{CodeBLEU} \\
    \hline
    \ChatGPTZeroShot & 17.72\% & 44.17\% & 13.52\% & 78.36\% & 2.62\% & 74.92\% & 0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\
    \hline
    \ChatGPTFewShot & 26.55\% & 47.50\% & 19.79\% & 81.47\% & \textbf{8.96\%} & 79.21\% & \textbf{2.34\%} & 75.33\% & 2.89\% & 81.40\% & 1.64\% & 73.83\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.93\%} & 49\% & \textbf{22.16\%} & \textbf{82.99\%} & 6.02\% & \textbf{79.81\%} & \textbf{2.34\%} & 74.15\% & \textbf{6.71\%} & 81.08\% & \textbf{3.05\%} & 74.67\% \\
    \hline
    \CodeReviewerModel & 33.23\% & \textbf{55.43\%} & - & - & - & - & - & - & - & - & - & - \\
    \hline
    \Tufanomodel & - & - & 14.26\% & 79.48 & 5.40\% & 77.26\% & - & - & - & - & - & - \\
    \hline
    \DACTmodel & - & - & - & - & - & - & 0.65\% & \textbf{75.99\%} & 5.98\% & \textbf{81.85\%} & 1.79\% & \textbf{79.77\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq4-result}%
\end{table*}%


\noindent \smallsection{Result}
% \textbf{In overall, \ChatGPTFineTune~achieve higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot.}
% \textbf{\ChatGPTFineTune~always achieves higher EM and CodeBLEU than \ChatGPTZeroShot, but does not always achieve higher EM and CodeBLEU than \ChatGPTFewShot.}
\textbf{\ChatGPTFineTune~achieves at least 9.74\% and 0.12\% higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot.}
Table~\ref{tab:rq3-with-persona} shows the evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~that persona is included when fine-tuning GPT-3.5.
The table shows that for the \tufanoData~(with comment), CodeRe\-viewer\textsubscript{data} and \DACTData~datasets, \hspace{2pt} GPT-3.5\textsubscript{fine-tuned} achieves EM of 2.29\% - 37.70\%, which is at least 75.98\% ($\frac{21.98-12.49}{12.49}$) and 9.74\% ($\frac{21.98-20.03}{20.03}$) higher than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
However, for the Tufa\-no\textsubscript{data} (without comment) dataset, we observe that GPT-3.5\textsubscript{few-shot} achieves EM of 9.18\%, which is 51.99\% higher than \hspace{1pt}GPT-3.5\textsubscript{fine-tuned}.
% However, we find that \ChatGPTFineTune~achieves 34.2\% lower EM than \ChatGPTFewShot~on the \tufanoData~(without comment) dataset.
% The table shows that in terms of EM, \ChatGPTFineTune~achieves 120.86\% ($\frac{37.70-17.07}{17.07}$), 75.98\% ($\frac{21.98-12.49}{12.49}$) and 163.76\% ($\frac{6.04-2.29}{2.29}$) higher EM than \ChatGPTZeroShot~on the \CodeReviewerData, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, \ChatGPTFineTune~achieves at least 301.75\% ($\frac{2.29-0.57}{0.57}$) higher EM than \ChatGPTZeroShot~on the \DACTData~dataset.
% The table also shows that \ChatGPTFineTune~achieves 43.24\% ($\frac{37.70-26.32}{26.32}$) and 9.74\% ($\frac{21.98-20.03}{20.03}$) higher EM than \ChatGPTFewShot~on the \CodeReviewerData~and \tufanoData~(with comment) datasets, respectively.
% Likewise,  \ChatGPTFineTune~achieves at least 41.36\% ($\frac{2.29-1.62}{1.62}$) higher EM than \ChatGPTFewShot~on the \hspace{0.01cm} D-ACT\textsubscript{data} dataset.
% On the other hand,  \ChatGPTFineTune~achieves 34.2\% ($\frac{6.04-9.18}{9.18}$) lower EM than \ChatGPTFewShot~on the \tufanoData~(with comment) dataset.
% The table also shows that \ChatGPTFineTune~achieves CodeBLEU of 49.20\% - 83.04\%, which is 7.4\% ($\frac{83.04-77.32}{77.32}$) - 63.9\% ($\frac{74.95-45.73}{45.73}$) and 0.12\% ($\frac{74.74-74.65}{74.65}$) - 3.73\% ($\frac{49.20-47.43}{47.43}$) higher than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
The table also shows that \ChatGPTFineTune~achieves CodeBLEU of 49.20\% - 83.04\%, which is at least 7.4\% \\($\frac{83.04-77.32}{77.32}$) and 0.12\% ($\frac{74.74-74.65}{74.65}$) higher than \ChatGPTZeroShot~and \hspace{1.5pt} GPT-3.5\textsubscript{few-shot}, respectively.
% In terms of CodeBLEU, GPT-3.5\textsubscript{fine-tuned} achieves 14.13\% ($\frac{49.20-34.11}{43.11}$), 7.4\% ($\frac{83.04-77.32}{77.32}$) and 8.95\% \newline ($\frac{79.76-73.21}{73.21}$) higher CodeBLEU than \ChatGPTZeroShot~on the Code\-Reviewer\textsubscript{data}, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, GPT-3.5\textsubscript{fine-tuned} achieves at least 33.75\% ($\frac{74.74-55.88}{55.88}$) higher CodeBLEU than \ChatGPTZeroShot~on the \DACTData~dataset.
% The table also shows that GPT-3.5\textsubscript{fine-tune} achieves 3.64\% ($\frac{49.20-47.47}{47.47}$), 1.75\% ($\frac{83.04-81.61}{81.61}$) and 0.99\% \newline ($\frac{79.76-78.98}{78.98}$) higher CodeBLEU than \ChatGPTFewShot~on the Code\-Reviewer\textsubscript{data}, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% On the other hand, \ChatGPTFineTune~achieves at least 0.12\% ($\frac{74.74-74.65}{74.65}$) higher CodeBLEU than \ChatGPTFewShot~on the Android and Ovirt projects while achieving 0.06\% ($\frac{81.02-81.07}{81.07}$) lower CodeBLEU on the Google project of the \DACTData~dataset.

Table~\ref{tab:rq3-without-persona} shows the evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~that persona is not included when fine-tuning GPT-3.5.
The table shows that for the Tufano\textsubscript{data} (with comment), CodeRev\-iewer\textsubscript{Data} and \DACTData~datasets, GPT-3.5\textsubscript{fine-tuned} achieves EM of 2.34\% - 37.93\%, which is at least 63.91\% ($\frac{22.16-13.52}{13.52}$) and 11.98\% ($\frac{22.16-19.79}{19.79}$) higher than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
However, \hspace{1pt} for the Tufano\textsubscript{data} (without comment), we observe that GPT-3.5\textsubscript{few-shot} achieves EM of 8.96\%, which is 48.84\% higher \hspace{1pt} than GPT-3.5\textsubscript{fine-tuned}.
% The table also shows that \ChatGPTFineTune~achieves CodeBLEU of 49.00\% - 82.99\%, which is 5.91\% ($\frac{82.99-78.36}{78.36}$) - 32.83\% ($\frac{81.08-61.04}{61.04}$) and 1.14\% ($\frac{74.67-56.55}{56.55}$) - 3.05\% ($\frac{49.00-47.55}{47.55}$) higher than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
The table also shows that \hspace{0.5pt} GPT-3.5\textsubscript{fine-tuned} achieves CodeBLEU of 49.00\% - 82.99\%, which is at least 5.91\% \\ ($\frac{82.99-78.36}{78.36}$) and 1.14\% ($\frac{74.67-56.55}{56.55}$) higher than \hspace{2pt} GPT-3.5\textsubscript{0-shot} and \ChatGPTFewShot, respectively.


% The table shows that in terms of EM, \ChatGPTFineTune~achieves 114.05\% ($\frac{37.93-17.72}{17.72}$), 63.91\% ($\frac{22.16-13.52}{13.52}$) and 129.77\% ($\frac{6.02-2.62}{2.62}$) higher EM than \ChatGPTZeroShot~on the \CodeReviewerData, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, \ChatGPTFineTune~achieves at least 377.55\% ($\frac{2.34-0.49}{0.49}$) higher EM than \ChatGPTZeroShot~on the \DACTData~dataset.
% The table also shows that \ChatGPTFineTune~achieves 43.29\% \newline ($\frac{37.93-26.47}{26.47}$) and 11.98\% ($\frac{22.16-19.79}{19.79}$) higher EM than GPT-3.5\textsubscript{few-shot} on the \CodeReviewerData~and \tufanoData~(with comment) datasets, respectively.
% On the other hand, GPT-3.5\textsubscript{fine-tuned} achieves 32.81\% ($\frac{6.02-8.96}{8.96}$) lower EM than \ChatGPTFewShot~on the \tufanoData~(without comment) dataset.
% For the \DACTData~dataset, GPT-3.5\textsubscript{fine-tuned} achieves similar EM to \ChatGPTFewShot~on the Android project while achieving at least 85.98\% ($\frac{3.05-1.64}{1.64}$) higher EM on the Google and Ovirt projects.
% In terms of CodeBLEU,  GPT-3.5\textsubscript{fine-tuned} achieves 10.94\% ($\frac{49.00-44.17}{44.17}$), 5.91\% ($\frac{82.99-78.36}{78.36}$) and 6.53\% \newline ($\frac{79.81-74.92}{74.92}$) higher CodeBLEU than \ChatGPTZeroShot~on the Code\-Reviewer\textsubscript{data}, \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% Similarly, GPT-3.5\textsubscript{fine-tuned} achieves at least 19.89\% ($\frac{74.15-61.85}{61.85}$) higher CodeBLEU than \ChatGPTZeroShot~on the \DACTData~dataset.
% The table also shows that GPT-3.5\textsubscript{fine-tuned} achieves 3.05\% ($\frac{49.00-47.55}{47.55}$), 1.87\% \newline ($\frac{82.99-81.47}{81.47}$) and 0.76\% ($\frac{79.81-79.21}{79.21}$) higher CodeBLEU than \ChatGPTFewShot~on the \CodeReviewerData, Tufano\textsubscript{data} (with comment) and Tufano\textsubscript{data (without comment) datasets, respectively.
% However, \ChatGPTFineTune~achieves 1.57\% ($\frac{74.15-75.33}{75.33}$) and 0.39\% ($\frac{81.08-81.40}{81.40}$) lower CodeBLEU than \ChatGPTFewShot~on the Android and Google projects, respectively while achieving 1.14\% ($\frac{74.67-73.83}{73.83}$) higher CodeBLEU on the Ovirt project of the \DACTData~dataset.


%% for new figure
Figure~\ref{fig:RQ3-analysis-with-persona} and Figure~\ref{fig:RQ3-analysis-without-persona} shows the characteristic of the code changes of the improved code that \ChatGPTZeroShot, GPT-3.5\textsubscript{few-shot} and \ChatGPTFineTune~correctly generate.
The figures show that for the \tufanoData(with comment), \CodeReviewerData~and \hspace{0.5pt} D-ACT\textsubscript{data}, \ChatGPTFineTune~achieves the highest EM for the code changes of \textit{Refactoring} and \textit{Other}, which is at least 5.90\% and 36.16\%, respectively for GPT-3.5 that we include persona in the input prompts; and at least 4.43\% and 36.88\%, respectively for GPT-3.5 that we do not include persona in the input prompts.
However, for the \tufanoData(without comment) dataset, GPT-3.5\textsubscript{few-shot} achieves the highest EM for the code changes of all categories.



The results indicate that in overall, model fine-tuning could help GPT-3.5 to generate more correct improved code and generate more similar improved code to actual improved code than 0-shot learning and few-shot learning.
% The above results indicate that model fine-tuning could help GPT-3.5 to generate more correct improved code when compared to 0-shot and few-shot learning.




\noindent \textbf{(RQ4) \rqfour}

\noindent \smallsection{Approach}
To address this RQ, we compare \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~with the existing code review automation approaches (i.e., \Tufanomodel~\cite{tufano2022using}, \DACTmodel~\cite{pornprasit2023d} and \CodeReviewerModel~\cite{li2022automating}).
To do so, we select the results of \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~that persona is not included in the input prompts since they achieve higher EM and CodeBLEU than the ones that persona is included in the input prompts (as shown in RQ2).
Then, we obtain the results of the existing code review automation approaches.
In particular, we obtain the results of \Tufanomodel~and \DACTmodel~from the replication packages.
However, since Li~\ea~\cite{li2022automating} do not make their results publicly available, we obtain the results from Guo~\ea~\cite{guo2023exploring} instead.
% After that, we compare the results of GPT-3.5 with the existing code review automation approaches by using the same evaluation measures as RQ1-RQ3.
Similar to RQ1-RQ3, we measure EM and CodeBLEU of the results obtained from GPT-3.5 and the existing code review automation approaches.





\noindent \smallsection{Result}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms the existing code review automation approaches in \tufanoData~and \DACTData.}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms \Tufanomodel~and \DACTmodel.}
\textbf{The existing code review automation approaches achieve at least 5.47\% higher EM than \ChatGPTZeroShot while \ChatGPTFineTune~achieves at least 11.48\% higher EM than the existing code review automation approaches.}
Table~\ref{tab:rq4-result} shows the results of \ChatGPTZeroShot, \ChatGPTFewShot, GPT-3.5\textsubscript{fine-tuned} and the existing code review automation approaches.
The table shows that the existing code review automation approaches achieve EM of 0.65\% - 33.23\%, which is at least 5.47\% \\($\frac{14.26-13.52}{13.52}$) higher than \ChatGPTZeroShot.
The table also shows that the existing code review automation approaches achieve CodeBLEU of 55.43\% - 81.85\%, which is at least 1.43\% ($\frac{79.48-78.36}{78.36}$) higher than \ChatGPTZeroShot.
% The table shows that in terms of EM, \CodeReviewerModel~achieves 87.53\% ($\frac{33.23-17.72}{17.72}$) higher EM than \ChatGPTZeroShot; and \Tufanomodel~and \DACTmodel~achieve at least 5.47\% ($\frac{14.29-13.52}{13.52}$) and 32.65\% ($\frac{0.65-0.49}{0.49}$) higher EM than \ChatGPTZeroShot, respectively.
% In terms of CodeBLEU, CodeReviewer achieves 25.49\% ($\frac{55.43-44.17}{44.17}$) higher CodeBLEU than \ChatGPTZeroShot; and \Tufanomodel~and \DACTmodel~achieve at least 1.43\% ($\frac{79.48-78.36}{78.36}$) and 22.86\% ($\frac{75.99-61.85}{61.85}$) higher EM than \hspace{3pt} GPT-3.5\textsubscript{0-shot}, respectively.

We observe from the table that in terms of EM, \CodeReviewerModel~and \DACTmodel~achieve at least 9.15\% ($\frac{1.79-1.64}{1.64}$) higher than \ChatGPTFewShot.
In contrast, \ChatGPTFewShot~achieves at least 38.78\% ($\frac{19.79-14.26}{14.26}$) higher EM than \Tufanomodel.
In terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~achieve at least 0.55\% ($\frac{81.85-81.4}{81.4}$) higher than \ChatGPTFewShot.
On the contrary, \ChatGPTFewShot~achieves at least 2.5\% ($\frac{81.47-79.48}{79.48}$) higher CodeBLEU than \Tufanomodel.


% We observe from the table that in terms of EM, \CodeReviewerModel~achieves 25.16\% ($\frac{33.23-26.55}{26.55}$) higher than \hspace{2pt} GPT-3.5\textsubscript{few-shot}.
% In contrast, \ChatGPTFewShot~achieves at least 38.78\% ($\frac{19.79-14.26}{14.26}$) higher EM than \Tufanomodel.
% On the other hand, GPT-3.5\textsubscript{few-shot} achieves 260\% ($\frac{2.34-0.65}{0.65}$) higher EM than \DACTmodel~on the Android project, while \DACTmodel~achieves at least 9.15\% \\ ($\frac{1.79-1.64}{1.64}$) higher EM than \ChatGPTFewShot~on the Google and Ovirt projects.
% In terms of CodeBLEU, \CodeReviewerModel~achieves 16.69\% ($\frac{55.43-47.50}{47.50}$) higher CodeBLEU than \ChatGPTFewShot.
% \DACTmodel~also achieves at least 0.55\% ($\frac{81.85-81.4}{81.4}$) higher CodeBLEU than \ChatGPTFewShot.
% On the contrary, \ChatGPTFewShot~achieves at least 2.5\% ($\frac{81.47-79.48}{79.48}$) higher CodeBLEU than \Tufanomodel.

The table also shows that GPT-3.5\textsubscript{fine-tuned} achieves EM of 2.34\% - 37.93\%, which is at least 
12.21\% ($\frac{6.71-5.98}{5.98}$) higher than the existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d}.
% 14.14\% ($\frac{37.93-33.23}{33.23}$) higher EM than \CodeReviewerModel.
% Similarly, \ChatGPTFineTune~achieves at least 11.48\% ($\frac{6.02-5.4}{5.4}$) and 12.21\% ($\frac{6.71-5.98}{5.98}$) higher EM than \Tufanomodel~and \DACTmodel, respectively.
However, in terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~achieves at least 0.95\% ($\frac{81.85-81.08}{81.08}$) \hspace{0.5pt} higher than GPT-3.5\textsubscript{fine-tuned}.
% \CodeReviewerModel~achieves 13.12\% ($\frac{55.43-49.00}{49.00}$) higher CodeBLEU than \ChatGPTFineTune.
% Likewise, \DACTmodel~achieves at least 0.95\% ($\frac{81.85-81.08}{81.08}$) higher CodeBLEU than \ChatGPTFineTune.
In contrast, GPT-3.5\textsubscript{fine-tuned} achieves at least 3.3\% ($\frac{79.81-77.26}{77.26}$) higher CodeBLEU than \Tufanomodel.

% The above results indicate that \ChatGPTZeroShot~still underperforms the existing code review automation approaches.
% However, using few-shot learning and fine-tuning GPT-3.5 does not always help GPT-3.5 to outperform \CodeReviewerModel~and \DACTmodel, but could help GPT-3.5 to outperform \Tufanomodel.
The above results indicate that the existing code review automation approaches can generate more correct improved code and generate more similar improved code to actual improved code than GPT-3.5 that we perform 0-shot learning.
In contrast, performing few-shot learning with GPT-3.5 does not always help GPT-3.5 outperform the existing code review automation approaches.
On the other hand, fine-tuning GPT-3.5 could help GPT-3.5 generate more correct improved code than the existing code review automation approaches.
% In contrast, \ChatGPTFewShot~can generate more correct improved code than the existing code review automation approaches On the other hand, such approaches can generate more similar improved code to actual improved code than \ChatGPTFewShot~and \ChatGPTFineTune.



==> section-exp-only/Result-old-4.tex <==


\section{Result} \label{sec:results}


In this section, we present the experiment results of the follwing four research questions.

\noindent \textbf{(RQ1) \rqone}

\noindent \smallsection{Approach}
To address this RQ, we use the prompts in Figure~\ref{fig:prompt-templates} by not including persona to enable GPT-3.5 to perform zero-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
Then, we measure EM and CodeBLEU of the results obtained from GPT-3.5.
% The results of zero-shot and few-shot learning are denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
GPT-3.5 that zero-shot learning and few-shot learning is performed is denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.



% To address this RQ, we do zero-shot and few-shot learning by first creating the input prompts from the prompt templates in Figure~\ref{fig:zero-shot prompt} and~\ref{fig:few-shot prompt}, respectively without using persona.
% To do few-shot learning,  we use BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to select three pairs of input and output from the training set for each testing sample.
% We do so since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform a random sample selection approach.
% Then, we obtain the improved code from GPT-3.5 by using the created input prompts.

% After that, we compare the results of \ChatGPTZeroShot~and \ChatGPTFewShot~in terms of EM and CodeBLEU.

\noindent \smallsection{Result}
\textbf{When few-shot learning is performed, GPT-3.5 achieves at least 46.38\% higher EM and at least 3.97\% higher CodeBLEU than GPT-3.5 that zero-shot learning is perf\-ormed.}
% \textbf{Few-shot learning helps increase EM and CodeBLEU by at least 46.38\% and 3.97\%, respectively.}
Table~\ref{tab:rq1-result} shows the evaluation results of GPT-3.5\textsubscript{Zero-shot} and GPT-3.5\textsubscript{Few-shot} in terms of EM and CodeBLEU.
The table shows that GPT-3.5\textsubscript{Few-shot} achieves at least 46.38\% higher EM than \ChatGPTZeroShot.
The table also shows that GPT-3.5\textsubscript{Few-shot} achieves 3.97\% - 33.36\% higher CodeBLEU than \ChatGPTZeroShot.
Figure~\ref{fig:RQ1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ1-EM-intersection-D-ACT} show the Venn diagram of the improved code that GPT-3.5\textsubscript{Zero-shot} and GPT-3.5\textsubscript{Few-shot} correctly generate.
The figures show that the number of improved code that only \ChatGPTFewShot~correctly generates is at least 280.8\% higher than \ChatGPTZeroShot.

The results indicate that performing few-shot learning with GPT-3.5 could help GPT-3.5 to generate more correct and similar improved code to actual improved code compared to performing zero-shot learning with GPT-3.5.
% The results indicate that when few-shot learning is performed with GPT-3.5, GPT-3.5 generates more correct and similar improved code to actual improved code compared to when zero-shot learning is performed with GPT-3.5.
% few-shot learning could help GPT-3.5 to generate more correct and unique improved code, and generate more similar improved code to actual improved code than zero-shot learning.
% The increase in EM and CodeBLEU has to do with performing few-shot learning with GPT-3.5.
% When few-shot learning is performed with GPT-3.5, 
The reason for this indication is that GPT-3.5 learns to generate improved code from given example input/output pairs in an input prompt.
Such example input/output pairs in an input prompt could help GPT-3.5 to adapt to the code refinement task that it never learns during the model pre-training phase.
In contrast, when zero-shot learning is performed with GPT-3.5, GPT-3.5 has to rely on what it learned during the model pre-training phase, which is not specific to the code refinement task.
% does not have additional information to learn how improved code is generated from a given submitted code (and reviewer comment if available).
Thus, GPT-3.5 has to rely on what it learned during the model pre-training phase, which is not specific to the code refinement task.
% Thus, it is implied that GPT-3.5 does not adapt to the task that it never learns during the model pre-training phase.




% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  % \makegapedcells
  \centering
  \caption{(RQ2) The evaluation results of \ChatGPTZeroShot~(persona is included and not included in input prompts).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShotWithPersona & 17.07\% & 43.11\% & 12.49\% & 77.32\% & 2.29\% & 73.21\% & \textbf{0.57\%} & 55.88\% & 0.00\% & 50.65\% & 0.22\% & 45.73\% \\
    \hline
    \ChatGPTZeroShotWithoutPersona & \textbf{17.72\%} & \textbf{44.17\%} & \textbf{13.52\%} & \textbf{78.36\%} & \textbf{2.62\%} & \textbf{74.92\%} & 0.49\% & \textbf{61.85\%} & \textbf{0.16\%} & \textbf{61.04\%} & \textbf{0.48\%} & \textbf{56.55\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq2-result-zero-shot}%
\end{table*}%



% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ2) The evaluation results of \ChatGPTFewShot~(persona is included and not included in input prompts).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTFewShotWithPersona & 26.28\% & 47.43\% & \textbf{20.03\%} & 81.61\% & \textbf{9.18\%} & 78.98\% & 1.62\% & 74.65\% & 2.45\% & 81.07\% & \textbf{1.67\%} & 73.29\% \\
    \hline
    \ChatGPTFewShotWithoutPersona & \textbf{26.55\%} & \textbf{47.50\%} & 19.79\% & \textbf{81.47\%} & 8.96\% & \textbf{79.21\%} & \textbf{2.34\%} & \textbf{75.33\%} & \textbf{2.89\%} & \textbf{81.40\%} & 1.64\% & \textbf{73.83\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq2-result-few-shot}%
\end{table*}%

\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ2.pdf}
         \caption{\CodeReviewerData~dataset}
         \label{fig:RQ2-1-EM-intersection-CodeRec}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ2.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (with comment)}
         \label{fig:RQ2-1-EM-intersection-tufano-code-comment}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (without comment)}
         \label{fig:RQ2-1-EM-intersection-tufano-code}
     \end{subfigure}
    \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
         \caption{\DACTData~dataset}
         \label{fig:RQ2-1-EM-intersection-D-ACT}
     \end{subfigure}
     
     \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTZeroShotWithPersona~and \ChatGPTZeroShotWithoutPersona.}
    \label{fig:RQ2-1-EM-intersection}
\end{figure*}



\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=5]{figure/EM-RQ2.pdf}
         \caption{\CodeReviewerData~dataset}
         \label{fig:RQ2-2-EM-intersection-CodeRec}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=6]{figure/EM-RQ2.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
      \caption{\tufanoData~dataset (with comment)}
     \label{fig:RQ2-2-EM-intersection-tufano-code-comment}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=7]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
          \caption{\tufanoData~dataset (without comment)}
         \label{fig:RQ2-2-EM-intersection-tufano-code}
     \end{subfigure}
    \begin{subfigure}[]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=8]{figure/EM-RQ2.pdf}
         % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
         \caption{\DACTData~dataset}
         \label{fig:RQ2-2-EM-intersection-D-ACT}
     \end{subfigure}
     
     \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTFewShotWithPersona~and \ChatGPTFewShotWithoutPersona.}
    \label{fig:RQ2-2-EM-intersection}
\end{figure*}


\noindent \textbf{(RQ2) \rqtwo}

\noindent \smallsection{Approach}
% To address this RQ, similar to RQ1, we create the input prompts for GPT-3.5 by using the prompt templates in Figure~\ref{fig:prompt-templates} with persona.
% Then, we obtain the improved code from GPT-3.5 by using the created input prompts.
To address this RQ, we use the prompts in Figure~\ref{fig:prompt-templates} by including persona to enable GPT-3.5 to perform zero-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
% we do zero-shot and few-shot learning with GPT-3.5 as explained in Section~\ref{sec:study-design} by using persona in the input prompts. 
% Then, similar to RQ1, we measure EM and CodeBLEU of the results obtained from GPT-3.5 that generates improved code from the prompts with persona and GPT-3.5 that generates improved code from the prompts without persona.
% The results obtained from \ChatGPTZeroShot~and \ChatGPTFewShot~that we include persona in the input prompts are denoted as \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
% Similarly, the results obtained from \ChatGPTZeroShot~and \ChatGPTFewShot~that we do not include persona in the input prompts are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.
\ChatGPTZeroShot~and \ChatGPTFewShot~that generate improved code from the prompts with persona are denoted as \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
Similarly, \hspace{1.5pt} \ChatGPTZeroShot~and GPT-3.5\textsubscript{Few-shot} that generate improved code from the prompts without persona are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.

\noindent \smallsection{Result}
% \textbf{In overall, \ChatGPTZeroShot~and \ChatGPTFewShot~that we use input prompts with persona achieve higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot~that we use input prompts without persona.}
% \textbf{In overall, \ChatGPTZeroShotWithoutPersona~and GPT-3.5-NP\textsubscript{Few-shot} achieve higher EM and CodeBLEU than GPT-3.5-WP\textsubscript{Few-shot} and \ChatGPTFewShotWithPersona}
\textbf{When persona is included in input prompts to generate improved code, GPT-3.5 achieves at least 1.02\% lower EM and 0.15\% lower CodeBLEU than when persona is not included in the input prompts.}
% \textbf{When GPT-3.5 generates improved code from the input prompts that persona is included, GPT-3.5 achieves at least 1.02\% and 0.15\% lower EM and CodeBLEU compared to when persona is not included in the input prompts.}
% Table~\ref{tab:rq2-result-zero-shot} shows the evaluation results of GPT-3.5\textsubscript{Zero-shot} that generates improved code from the input prompts with persona and without persona.
Table~\ref{tab:rq2-result-zero-shot} shows the evaluation results of GPT-3.5 that zero-shot learning is performed by using input prompts with and without persona.
The table shows that \ChatGPTZeroShotWithPersona~achieves at least 3.67\% and 1.33\% lower EM and CodeBLEU than \ChatGPTZeroShotWithoutPersona, respectively.
Figure~\ref{fig:RQ2-1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-1-EM-intersection-D-ACT} show the Venn diagram of the improved code that \ChatGPTZeroShotWithPersona~and GPT-3.5-NP\textsubscript{Zero-shot} correctly generate.
The figures show that the number of improved code that only~\ChatGPTZeroShotWithPersona~correctly generates is at least 22.02\% lower than~\ChatGPTZeroShotWithoutPersona



Table~\ref{tab:rq2-result-few-shot} shows the evaluation results of GPT-3.5 that few-shot learning is performed by using input prompts with and without persona.
The table shows that GPT-3.5-WP\textsubscript{Few-shot} ach\-ieves at least 1.02\% and 0.15\% lower EM and CodeBLEU than \ChatGPTFewShotWithoutPersona, respectively.
However, we observe that for the \tufanoData~dataset, \hspace{0.5pt} \ChatGPTFewShotWithPersona~achieves 1.21\% - 2.46\% higher EM than \ChatGPTFewShotWithoutPersona.
Figure~\ref{fig:RQ2-2-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-2-EM-intersection-D-ACT} show the Venn diagram of the improved code that GPT-3.5-WP\textsubscript{Few-shot} and \ChatGPTFewShotWithoutPersona~correctly generate.
The figures show that the number of improved code that only GPT-3.5-WP\textsubscript{Few-shot} correctly generates is at least 16.48\% \hspace{2pt} lower than GPT-3.5-NP\textsubscript{Few-shot}.
Nevertheless, for the Tufano\textsubscript{Data}\\dataset, the number of improved code that only GPT-3.5-WP\textsubscript{Few-shot} correctly generates is 20.1\% - 26.06\% higher than GPT-3.5-NP\textsubscript{Few-shot}.


% The table shows that in terms of EM, \ChatGPTFewShot~that does not use persona achieves 0.88\% \newline ($\frac{26.46-26
% 32}{26.32}$) higher EM than \ChatGPTFewShot~that uses persona on the CodeReviewer\textsubscript{data} dataset, while achieving 1.2\% ($\frac{19.79-20.03}{20.03}$) and 2.4\% ($\frac{8.96-9.18}{9.18}$) lower EM than \ChatGPTFewShot~that uses persona on the \tufanoData~(with comment) and \tufanoData~(without comment) datasets, respectively.
% On the other hand, \ChatGPTFewShot~that does not use persona achieves at least 17.96\% ($\frac{2.89-2.45}{2.45}$) higher EM than \ChatGPTFewShot~that uses persona on the Android and Google projects while achieving 1.8\% ($\frac{1.64-1.67}{1.67}$) lower EM than \ChatGPTFewShot~that uses persona on the Ovirt project.
% In terms of CodeBLEU, \ChatGPTFewShot~that does not use persona achieves 0.19\% ($\frac{47.55-47.46}{47.46}$) and 0.29\% ($\frac{79.21-78.98}{78.98}$) higher CodeBLEU than \ChatGPTFewShot~that uses persona on the CodeReviewer\textsubscript{data} and \tufanoData~(without comment) datasets, respectively, while achieving 0.17\% ($\frac{47.55-47.47}{47.47}$) lower CodeBLEU than \ChatGPTFewShot~that uses persona on the Tufano\textsubscript{data} (with comment) dataset.
% On the other hand, \ChatGPTFewShot~that does not use persona achieves at least 0.41\% ($\frac{81.4-81.07}{81.07}$) higher than \ChatGPTFewShot~that uses persona on the \DACTData~dataset.
% The above results indicate that using persona does not always help GPT-3.5 to correctly generate more improved code.


The above results indicate that including persona in input prompts when performing zero-shot and few-shot learning does not guarantee that GPT-3.5 could generate more correct and similar improved code to actual improved code.
The reason for this indication is that when persona is included in input prompts, GPT-3.5 is instructed to generate source code like how a software developer would do.
In a zero-shot learning scenario, having persona in input prompts tends to decrease the likelihood of GPT-3.5 generating more correct and similar improved code to actual improved code.
On the contrary, in a few-shot learning scenario, having persona in input prompts does not always increase the likelihood of GPT-3.5 generating more correct and similar improved code to actual improved code like in zero-shot learning.
% The reason for this uncertainty is that the increase in the likelihood only occurs in non-project-specific Java datasets.


% GPT-3.5 has to act as a developer without context (i.e., example of input/output pairs) to generate improved code.
% Thus, GPT-3.5 tends to generate incorrect improved code when compared to the actual improved code.
% On the contrary, in a few-shot learning scenario, GPT-3.5 has context to help it understand how improved code is generated from the given input code (and comment if available).
% Thus, 

% The results indicate that performing zero-shot learning with GPT-3.5 by using input prompts with persona does not help GPT-3.5 to generate more correct and similar improved code to actual improved code.
% However, performing few-shot learning with GPT-3.5 by using input prompts with persona does not guarantee that GPT-3.5 could generate more correct and similar improved code to actual improved code.
% The reason for this indication is that when persona is included in input prompts, GPT-3.5 is instructed to generate source code like a software developer would do.
% In a zero-shot learning scenario, \textbf{???}



% GPT-3.5 has to act as a software developer without additional information



% tends to lead to generating improved code.



% when zero-shot learning is performed with GPT-3.5 by using input prompts with persona, GPT-3.5 generates less correct and similar improved code to actual improved code compared to performing zero-shot learning with GPT-3.5 by using input prompts without persona.
% However, when few-shot learning is performed with GPT-3.5 by using input prompts with persona, GPT-3.5 does not always generate less correct and similar improved code to actual improved code compared to performing few-shot learning with GPT-3.5 by using input prompts without persona.

% (explain indication of few-shot learning here) ... \textbf{(continue from here)}

% The results indicate that in overall, \ChatGPTZeroShot~and \ChatGPTFewShot~that persona is not included in the input prompts can generate more correct and unique improved code and generate more similar improved code to actual improved code than GPT-3.5\textsubscript{Zero-shot} and \ChatGPTFewShot~that persona is included in the input prompts.


% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ3) The evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot, and \ChatGPTFineTune~(persona is included in input prompts).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShot & 17.07\% & 43.11\% & 12.49\% & 77.32\% & 2.29\% & 73.21\% & 0.57\% & 55.88\% & 0.00\% & 50.65\% & 0.22\% & 45.73\% \\
    \hline
    \ChatGPTFewShot & 26.28\% & 47.43\% & 20.03\% & 81.61\% & \textbf{9.18\%} & 78.98\% & 1.62\% & 74.65\% & 2.45\% & \textbf{81.07\%} & 1.67\% & 73.29\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.70\%} & \textbf{49.20\%} & \textbf{21.98\%} & \textbf{83.04\%} & 6.04\% & \textbf{79.76\%} & \textbf{2.29\%} & \textbf{74.74\%} & \textbf{6.14\%} & 81.02\% & \textbf{2.64\%} & \textbf{74.95\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq3-with-persona}%
\end{table*}%




% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ3) The evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot, and \ChatGPTFineTune~(persona is not included in input prompts).}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[1]{*}{Approach}} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}      & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\
    \hline
    \ChatGPTZeroShot & 17.72\% & 44.17\% & 13.52\% & 78.36\% & 2.62\% & 74.92\% & 0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\
    \hline
    \ChatGPTFewShot & 26.55\% & 47.50\% & 19.79\% & 81.47\% & \textbf{8.96\%} & 79.21\% & 2.34\% & \textbf{75.33\%} & 2.89\% & \textbf{81.40\%} & 1.64\% & 73.83\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.93\%} & \textbf{49.00\%} & \textbf{22.16\%} & \textbf{82.99\%} & 6.02\% & \textbf{79.81\%} & 2.34\% & 74.15\% & \textbf{6.71\%} & 81.08\% & \textbf{3.05\%} & \textbf{74.67\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq3-without-persona}%
\end{table*}%


\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0.5cm 0.7cm 0 0}, clip]{figure/fine-tuned-vs-0-shot-and-few-shot-with-persona-analysis.pdf}
         \caption{The results of GPT-3.5 (persona is included in input prompts)}
         \label{fig:RQ3-analysis-with-persona}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim = {0.5cm 0.7cm 0 0}, clip]{figure/fine-tuned-vs-0-shot-and-few-shot-without-persona-analysis.pdf}
     %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
      \caption{The results of GPT-3.5 (persona is not included in input prompts)}
     \label{fig:RQ3-analysis-without-persona}
     \end{subfigure}
     % \par\bigskip 

     \caption{(RQ3) The EM achieved by \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~categorized by types of code change.}
    \label{fig:RQ3-analysis}
\end{figure*}



\begin{figure*}[!h]
     \centering
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {1 25cm 0 0}, clip, page=1]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{bug fixing} (modify if condition)}
         \label{fig:RQ3-bug-fix-1}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 26cm
         0 0 0}, clip, page=2]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{bug fixing} (remove \texttt{synchronized} keyword)}
         \label{fig:RQ3-bug-fix-2}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 25cm 0 0}, clip, page=3]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{refactoring} (change variable name)}
         \label{fig:RQ3-refactor-1}
     \end{subfigure}
    \begin{subfigure}[]{\columnwidth}
         \centering
        \includegraphics[width=\columnwidth, trim = {0 25cm 0 0}, clip, page=4]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{refactoring} (remove \texttt{this} qualifier)}
         \label{fig:RQ3-refactor-2}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 15cm 0 0}, clip, page=5]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{other} (remove if condition)}
         \label{fig:RQ3-other-1}
     \end{subfigure}
    \begin{subfigure}[]{\columnwidth}
         \centering
        \includegraphics[width=\columnwidth, trim = {0 15cm 0 0}, clip, page=6]{figure/sample-code-change-each-type.pdf}
         \caption{Example of code change for \textit{other} (remove method call)}
         \label{fig:RQ3-other-2}
     \end{subfigure}
     
    \caption{(RQ3) Example of code changes for each type}
    \label{fig:RQ3-code-change-example}
\end{figure*}



\noindent \textbf{(RQ3) \rqthree}

\noindent \smallsection{Approach}
To address this RQ, we fine-tune GPT-3.5 as explained in Section~\ref{sec:study-design}.
% We do so by using prompts that contain persona and do not contain persona similar to RQ2.
Then, similar to RQ1 and RQ2, we measure EM and CodeBLEU of the results obtained from the fine-tuned GPT-3.5 (the fine-tuned GPT-3.5 models are denoted as \ChatGPTFineTune).
In addition, we analyze the improved code that \ChatGPTZeroShot, \ChatGPTFewShot~and \ChatGPTFineTune~correctly generate to understand the characteristics of code changes of such improved code.
To do so, we randomly select the improved code that is only correctly generated by a particular model (e.g., we randomly obtain the improved code that only \ChatGPTZeroShot~correctly generates while the others do not.) by using the confidence level of 95\% and the confidence interval of 5\%.
% Then, we classify the code change of the selected improved code into three categories (i.e., \textit{fixing bug}, \textit{refactoring} and \textit{other}) by following the taxonomy of code change created by Tufano~\ea~\cite{tufano2019learning}.
\revised{R2-2}{
Then, we classify the code change of the selected improved code into the following categories by following the taxonomy of code change created by Tufano~\ea~\cite{tufano2019learning} (the examples of the code changes in each category are shown in Figure~\ref{fig:RQ3-code-change-example}):

\begin{itemize}
    \item \textit{fixing bug}: The code changes in this category involve fixing bugs in the past.
    The following sub-categories are related to this category: exception handling, conditional statement, lock mechanism, method return value, and me\-thod invocation.
    \item \textit{refactoring}: The code changes in this category involve making changes to code structure without changing the behavior of the changed code.
    The following sub-categories are related to this category: inheritance; encapsulation; methods interaction; readability; and renaming parameter, method and variable.
    \item \textit{other}: The code changes that cannot be classified as neither \textit{fixing bug} nor \textit{refactoring} will fall into this category.
\end{itemize}
}






\noindent \smallsection{Result}
% \textbf{In overall, \ChatGPTFineTune~achieve higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot.}
% \textbf{\ChatGPTFineTune~always achieves higher EM and CodeBLEU than \ChatGPTZeroShot, but does not always achieve higher EM and CodeBLEU than \ChatGPTFewShot.}
\textbf{Fine-tuned GPT-3.5 achieves at least 9.74\% higher EM and 0.12\% higher CodeBLEU than GPT-3.5 that zero-shot and few-shot learning is performed.}
% \textbf{\ChatGPTFineTune~achieves at least 9.74\% and 0.12\% higher EM and CodeBLEU than \ChatGPTZeroShot~and \ChatGPTFewShot.}
Table~\ref{tab:rq3-with-persona} shows the evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot~and GPT-3.5\textsubscript{Fine-tuned}  that generate improved code from input prompts with persona.
% The table shows that for the \tufanoData~(with comment), CodeRe\-viewer\textsubscript{data} and \DACTData~datasets, \hspace{2pt} GPT-3.5\textsubscript{Fine-tuned} achieves at least 75.98\% and 9.74\% higher EM than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
The table shows that GPT-3.5\textsubscript{Fine-tuned} achieves at least 75.98\% and 9.74\% higher EM than GPT-3.5\textsubscript{Zero-shot} and \ChatGPTFewShot, respectively.
However, for the Tufa\-no\textsubscript{data} (without comment) dataset, we observe that GPT-3.5\textsubscript{Few-shot} achieves 51.99\% higher EM than \hspace{1pt}GPT-3.5\textsubscript{Fine-tuned}.
The table also \hspace{1pt} shows that GPT-3.5\textsubscript{Fine-tuned} achieves at least 7.4\% and 0.12\% higher CodeBLEU than GPT-3.5\textsubscript{Zero-shot} and GPT-3.5\textsubscript{Few-shot}, respectively.



Table~\ref{tab:rq3-without-persona} shows the evaluation results of \ChatGPTZeroShot, \ChatGPTFewShot~and GPT-3.5\textsubscript{Fine-tuned} that generate improved code from input prompts without persona.
% The table shows that for the Tufano\textsubscript{data} (with comment), CodeRev\-iewer\textsubscript{Data} and \DACTData~datasets, GPT-3.5\textsubscript{Fine-tuned} achieves at least 63.91\% and 11.98\% higher EM than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
The table shows that GPT-3.5\textsubscript{Fine-tuned} achieves at least 63.91\% and 11.98\% higher EM than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
However, for the Tufano\textsubscript{data} (without comment), we observe that GPT-3.5\textsubscript{Few-shot} achieves 48.84\% higher EM than GPT-3.5\textsubscript{Fine-tuned}.
% The table also shows that \ChatGPTFineTune~achieves CodeBLEU of 49.00\% - 82.99\%, which is 5.91\% ($\frac{82.99-78.36}{78.36}$) - 32.83\% ($\frac{81.08-61.04}{61.04}$) and 1.14\% ($\frac{74.67-56.55}{56.55}$) - 3.05\% ($\frac{49.00-47.55}{47.55}$) higher than \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.
The table also shows that GPT-3.5\textsubscript{Fine-tuned} achieves at least 5.91\% and 1.14\% higher CodeBLEU than GPT-3.5\textsubscript{Zero-shot} and GPT-3.5\textsubscript{Few-shot}, respectively.


%% for new figure
Finally, we show the characteristic of the code changes (i.e., \textit{Fixing Bug}, \textit{Refactoring} and \textit{Other}) of the improved code that \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \\GPT-3.5\textsubscript{Fine-tuned}~correctly generate in Figure~\ref{fig:RQ3-analysis-with-persona} and Figure~\ref{fig:RQ3-analysis-without-persona}.
% Figure~\ref{fig:RQ3-analysis-with-persona} and Figure~\ref{fig:RQ3-analysis-without-persona} show the characteristic of the code changes of the improved code that \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \ChatGPTFineTune~correctly generate.
The figures show that for the \tufanoData(with comment), \CodeReviewerData~and \hspace{0.5pt} D-ACT\textsubscript{data}, \ChatGPTFineTune~\\achieves the highest EM for the code changes of \textit{Refactoring} and \textit{Other}.
In contrast, for the Tufano\textsubscript{data} (without comment) dataset, GPT-3.5\textsubscript{Few-shot} achieves the highest EM for the code changes of all categories.
% ทุก approach ได้ em สูงสุดสำหรับ other category ในทุก dataset
% 	●	ก็เพราะว่าไม่ได้บอกให้ GPT-3.5 มันสร้าง improved code ขึ้นมาเพื่อการแก้ bug หรือ refactor code โดยเฉพาะ
% 	●	ดังนั้น GPT-3.5 มันสร้าง improved code แบบใดก็ได้ (ซึ่งอาจจะไม่ได้เป็นเพื่อการแก้ bug หรือ refactor code)
% 	●	ในภายหลังพอเอา improved code อันที่ GPT-3.5 สร้างมาถูกมาจัดประเภท code change เลยพบว่าส่วนใหญ่แล้วมันเป็นแบบ other
\revised{R2-2}{
Figure~\ref{fig:RQ3-analysis-with-persona} and Figure~\ref{fig:RQ3-analysis-without-persona} also show that \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \ChatGPTFineTune~achieve the highest EM for the code change of type \textit{other} across all studied datasets.
The reason for this result is that we do not specify the characteristics of the improved code (i.e., \textit{fixing bug} and \textit{refactoring}) in input prompts.
Thus, such models possibly generate improved code that is not specific to \textit{fixing bug} or \textit{refactoring}.
Therefore, the majority of the code change of the generated improved code are categorized as \textit{other}.
% Later, when the improved code that is correctly generated by such approaches are categorized based on the taxonomy of code change created by Tufano~\ea~\cite{tufano2019learning}, the majority of the generated improved code :
}

The above results indicate that in overall, model fine-tuning could help GPT-3.5 to generate more correct improved code and generate more similar improved code to actual improved code than GPT-3.5 that zero-shot learning and few-shot learning is performed.
% performing zero-shot learning and few-shot learning.
The reason for this indication is that when GPT-3.5 is fine-tuned, it directly learns how to generate improved code from a given input code (and comment if available) from thousands of examples in a training set.
Different from model fine-tuning, GPT-3.5 has no additional information to learn how improved code is generated when zero-shot learning is performed.
On the other hand, when few-shot learning is performed, GPT-3.5 has only a few examples to learn how improved code is generated.
% when few-shot learning is performed.

% Different from model fine-tuning, there is no additional information or a few example input/output pairs when performing zero-shot learning or few-shot learning, respectively.


% Thus, fine-tuned GPT-3.5 can adapt to the code refinement task better than performing zero-shot learning and few-shot learning that relies on a few example input/output pairs.

% The above results indicate that model fine-tuning could help GPT-3.5 to generate more correct improved code when compared to zero-shot and few-shot learning.


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The statistical details of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \begin{tabular}{|c|c|}
    \hline
    Model & \# parameters \\
    \hline
    TufanoT5~\cite{tufano2022using} & 60.5 M \\
    \hline
    CodeReviewer~\cite{li2022automating} & 222.8 M \\
    \hline
    D-ACT~\cite{pornprasit2023d} & 222.8 M \\
    \hline
    Magicoder~\cite{wei2023magicoder} & 6.7 B \\ 
    \hline
    GPT-3.5 & 175 B \\
    \hline
    \end{tabular}%
  \label{tab:model-detail}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'results each RQ new format'
\begin{table*}[h]
  \centering
  \caption{(RQ4) The evaluation results of GPT-3.5, Magicoder and the existing code review automation approaches.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-13}    \multicolumn{1}{r|}{} & \multicolumn{2}{c|}{\CodeReviewerData} & \multicolumn{2}{c|}{\tufanoData (with comment)} & \multicolumn{2}{c|}{\tufanoData (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} & \multicolumn{1}{c|}{EM} & \multicolumn{1}{c|}{CodeBLEU} \\
    \hline
    \ChatGPTZeroShot & 17.72\% & 44.17\% & 13.52\% & 78.36\% & 2.62\% & 74.92\% & 0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\
    \hline
    \ChatGPTFewShot & 26.55\% & 47.50\% & 19.79\% & 81.47\% & \textbf{8.96\%} & 79.21\% & \textbf{2.34\%} & 75.33\% & 2.89\% & 81.40\% & 1.64\% & 73.83\% \\
    \hline
    \ChatGPTFineTune & \textbf{37.93\%} & 49\% & \textbf{22.16\%} & \textbf{82.99\%} & 6.02\% & \textbf{79.81\%} & \textbf{2.34\%} & 74.15\% & \textbf{6.71\%} & 81.08\% & \textbf{3.05\%} & 74.67\% \\
    \hline
    \MagicoderZeroShot & 9.75\% & 39.43\% & 8.65\% & 73.90\% & 0.81\% & 59.50\% & 0.16\% & 47.30\% & 0.08\% & 48.85\% & 0.04\% & 44.38\% \\
    \hline
    \MagicoderFewShot & 15.97\% & 36.24\% & 2.93\% & 4.36\% & 1.99\% & 7.50\% & 0.22\% & 37.56\% & 0.49\% & 42.52\% & 0.74\% & 40.45\% \\
    \hline
    \MagicoderFineTune & 27.43\% & 44.85 & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\
    \hline
    \CodeReviewerModel & 33.23\% & \textbf{55.43\%} & 15.17\% & 80.83\% & 4.14\% & 78.76\% & 0.54\% & 75.24\% & 0.81\% & 80.1\% & 1.23\% & 75.32\%  \\
    \hline
    \Tufanomodel & 11.9\% & 43.39\% & 14.26\% & 79.48\% & 5.4\% & 77.26\% & 0.27\% & 75.88\% & 1.37\% & \textbf{82.25\%} & 0.19\% & 73.53\% \\
    \hline
    \DACTmodel & - & - & - & - & - & - & 0.65\% & \textbf{75.99\%} & 5.98\% & 81.85\% & 1.79\% & \textbf{79.77\%} \\
    \hline
    \end{tabular}%
  }
  \label{tab:rq4-result}%
\end{table*}%


\begin{figure*}[h]
    \centering
    \includegraphics[trim = {0.8cm 0 0 0}, clip, width=\textwidth]{figure/code_len_count_plot_updated.pdf}
    \caption{Exact Match categorized by the length of revised code.}
    \label{fig:code-len-count}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[trim = {0.8cm 0 0 0}, clip, width=\textwidth]{figure/changed_token_count_plot_updated.pdf}
    \caption{Exact Match categorized by the number of changed tokens.}
    \label{fig:changed-token-count}
\end{figure*}



\noindent \textbf{(RQ4) \rqfour}

\noindent \smallsection{Approach}
To address this RQ, we evaluate the performance of GPT-3.5 against \revised{R2-4}{an open-source LLM called Magicoder~\cite{wei2023magicoder}} and the existing code review automation approaches (\revised{R2-3}{
The details of GPT-3.5, Magicoder and the existing code review automation approaches are shown in Table~\ref{tab:model-detail}.
}).
\revised{R2-4}{
% In addition, we conduct experiments with an open-source LLM called Magicoder~\cite{wei2023magicoder}.
We choose Magicoder~\cite{wei2023magicoder} in our experiment since it outperforms other recent open-source instruction-tuned LLMs (e.g., Starcoder~\cite{li2023starcoder}, Deep\-Seek-Coder~\cite{guo2024deepseek} or CodeLLaMa~\cite{roziere2023codeLLaMa}).
When we perform zero-shot and few-shot learning with Magicoder, we follow the same process as we perform zero-shot and few-shot learning with GPT-3.5.
For fine-tuning Magicoder, we use the recently proposed parameter-efficient fine-tuning approach called DoRA~\cite{liu2024dora}, which is shown to outperform the LoRA approach.~\cite{hu2021lora}
}

% In this RQ, we select the results of \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \ChatGPTFineTune~that is generated from input prompts without persona.
% We select such results since they achieve higher EM and CodeBLEU than the ones that are generated from input prompts with persona (as shown in RQ2).
In this RQ, we evaluate the performance of GPT-3.5 and Magicoder that is generated from input prompts without persona.
We do so since RQ2 shows that the performance of GPT-3.5 that persona is not included in input prompts is higher than the performance of GPT-3.5 that persona is included in input prompts.


Then, we obtain the results of the existing code review automation approaches.
In particular, we obtain the results of \Tufanomodel~and \DACTmodel~from the replication packages.
However, since Li~\ea~\cite{li2022automating} do not make their results publicly available, we obtain the results from Guo~\ea~\cite{guo2023exploring} instead.
% After that, we compare the results of GPT-3.5 with the existing code review automation approaches by using the same evaluation measures as RQ1-RQ3.
\revised{R1-4}{
In addition, we evaluate the existing code review automation approaches across the studied datasets (e.g., we evaluate \CodeReviewerModel~on the Tufano\textsubscript{Data}~\\and \DACTData~datasets).
However, we do not evaluate \DACTmodel~with the \tufanoData~and \CodeReviewerData~datasets since such datasets do not contain code diff information, which is the component of \DACTmodel.
}

Similar to RQ1-RQ3, we measure EM and CodeBLEU of the results obtained from GPT-3.5 and the existing code review automation approaches.





\noindent \smallsection{Result}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms the existing code review automation approaches in \tufanoData~and \DACTData.}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms \Tufanomodel~and \DACTmodel.}
% \textbf{The existing code review automation approaches achieve at least 5.47\% higher EM than GPT-3.5 that zero-shot learning is performed while fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.}
\textbf{Fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.}
Table~\ref{tab:rq4-result} shows the results of GPT-3.5, Magicoder and the existing co\-de review automation approaches.
The table shows that in terms of EM, the existing code review automation approaches achieve at least 5.47\% and 22.05\% higher than GPT-3.5\textsubscript{Zero-shot} and Magicoder\textsubscript{Zero-shot}, respectively.
Moreover, in terms of CodeBLEU, the existing code review automation approaches achieve at least 1.43\% and 7.55\% higher than GPT-3.5\textsubscript{Zero-shot} and Magicoder\textsubscript{Zero-shot}, respectively.
The results indicate that the existing code review automation approaches can generate more correct improved code and generate more similar improved code to actual improved code than performing zero-shot learning with GPT-3.5 and Magicoder.

%% old version
% Table~\ref{tab:rq4-result} shows the results of \ChatGPTZeroShot, \ChatGPTFewShot, GPT-3.5\textsubscript{Fine-tuned} and the existing co\-de review automation approaches.
% The table shows that the existing code review automation approaches achieve at least 5.47\% and 1.43\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot}, respectively, indicating that the existing code review automation approaches can generate more correct improved code and generate more similar improved code to actual improved code than performing zero-shot learning with GPT-3.5.


We observe from the table that in terms of EM, D-ACT achieves at least 9.15\% higher than GPT-3.5\textsubscript{Few-shot} while GPT-3.5\textsubscript{Few-shot} achieves at least 30.45\% higher EM than \Tufanomodel~and\CodeReviewerModel.
On one hand, the existing code review automation approaches achieve at least 22.73\% higher EM than Magi\-coder\textsubscript{FewShot}.
In terms of CodeBLEU, \DACTmodel~achieves at least 0.55\% higher than \ChatGPTFewShot while \ChatGPTFewShot~achieves at least 2.5\% higher CodeBLEU than \Tufanomodel~and \CodeReviewerModel.
On the other hand, the existing code review automation approaches achieve at least 19.73\% higher CodeBLEU than \MagicoderFewShot.
The results indicate that performing few-shot learning with GPT-3.5 does not always help GPT-3.5 and Magicoder generate more correct and similar improved code to actual improved code than the existing code review automation approaches.
% In contrast, performing few-shot learning with Magicoder does not help Magicoder generate more correct and similar improved code to actual improved code than the existing code review automation approaches.

%% old one
% We observe from the table that in terms of EM, \DACTmodel~achieve at least 9.15\% higher than \ChatGPTFewShot.
% In contrast, \ChatGPTFewShot~achieves at least 30.45\% higher EM than \Tufanomodel~and\CodeReviewerModel.
% In terms of CodeBLEU, \DACTmodel~achieve at least 0.55\% higher than \ChatGPTFewShot.
% On the contrary, \ChatGPTFewShot~achieves at least 2.5\% higher CodeBLEU than \Tufanomodel~and\CodeReviewerModel.
% The results indicate that performing few-shot learning with GPT-3.5 does not always help GPT-3.5 generate more correct and similar improved code to actual improved code than the existing code review automation approaches.


The table also shows that in terms of EM, GPT-3.5\textsubscript{Fine-tuned} achieves at least 11.48\% higher EM than the existing code review automation approaches while such approaches achieve at least 21.14\% higher than Magicoder.
In terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~achieves at least 0.95\% higher than GPT-3.5\textsubscript{Fine-tuned} while GPT-3.5\textsubscript{Fine-tuned} ac\-hieves at least 3.3\% higher than \Tufanomodel.
In contrast, the existing code review automation approaches achieve at least 11.57\% higher CodeBLEU than Magicoder.
The results indicate that model fine-tuning could only help GPT-3.5 generate more correct improved code than the existing code review automation approaches.


%% old one
% The table also shows that GPT-3.5\textsubscript{Fine-tuned} achieves at least 
% 11.48\% higher EM than the existing code review automation approaches.
% However, \CodeReviewerModel~and \DACTmodel~achieves at least 0.95\% higher CodeBLEU than GPT-3.5\textsubscript{Fine-tuned} while GPT-3.5\textsubscript{Fine-tuned} achieves at least 3.3\% higher CodeBLEU than \Tufanomodel.
% The results indicate that fine-tuning GPT-3.5 could help GPT-3.5 generate more correct improved code than the existing code review automation approaches.

% The above results indicate that \ChatGPTZeroShot~still underperforms the existing code review automation approaches.
% However, using few-shot learning and fine-tuning GPT-3.5 does not always help GPT-3.5 to outperform \CodeReviewerModel~and \DACTmodel, but could help GPT-3.5 to outperform \Tufanomodel.
% The above results indicate that the existing code review automation approaches can generate more correct improved code and generate more similar improved code to actual improved code than performing zero-shot learning with GPT-3.5.
% In contrast, performing few-shot learning with GPT-3.5 does not always outperform the existing code review automation approaches.
% On the other hand, fine-tuning GPT-3.5 could help GPT-3.5 generate more correct improved code than the existing code review automation approaches.




==> section-exp-only/Result-old-5.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The statistical details of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \begin{tabular}{|c|c|}
    \hline
    Model & \# parameters \\
    \hline
    TufanoT5~\cite{tufano2022using} & 60.5 M \\
    \hline
    CodeReviewer~\cite{li2022automating} & 222.8 M \\
    \hline
    D-ACT~\cite{pornprasit2023d} & 222.8 M \\
    \hline
    Magicoder~\cite{wei2023magicoder} & 6.7 B \\ 
    \hline
    GPT-3.5 & 175 B \\
    \hline
    \end{tabular}%
  \label{tab:model-detail}%
\end{table}%

\begin{table*}[!h]
    \centering
    \caption{The evaluation results of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{Approach} & \multirow{2}{*}{Fine-Tuned?} & \multirow{2}{*}{Prompting} & \multirow{2}{*}{Use Persona?} & \multicolumn{2}{c|}{CodeReviewer} & \multicolumn{2}{c|}{Tufano (with comment)} & \multicolumn{2}{c|}{Tufano (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
        \cline{5-16}    
        ~ & ~ & ~ & ~ & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\ \hline
        \multirow{6}{*}{GPT-3.5} & \cmark   & \multirow{4}{*}{Zero-shot} & \xmark    & 37.93\% & 49.00\% & 22.16\% & 82.99\% & 6.02\% & 79.81\% & 2.34\% & 74.15\% & 6.71\% & 81.08\% & 3.05\% & 74.67\% \\
        \cline{2-2}\cline{4-16}
        ~ & \cmark & ~ & \cmark & 37.70\% & 49.20\% & 21.98\% & 83.04\% & 6.04\% & 79.76\% & 2.29\% & 74.74\% & 6.14\% & 81.02\% & 2.64\% & 74.95\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \xmark & 17.72\% & 44.17\% &  13.52\% & 78.36\% &  2.62\% & 74.92\% &  0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \cmark & 17.07\% & 43.11\% &  12.49\% & 77.32\% &  2.29\% & 73.21\% &  0.57\% & 55.88\% & 0.00\% & 50.65\% &  0.22\% & 45.73\% \\ \cline{2-16}
        ~ & \xmark & \multirow{2}{*}{Few-shot} & \xmark & 26.55\% & 47.50\% & 19.79\% & 81.47\% & 8.96\% & 79.21\% & 2.34\% & 75.33\% & 2.89\% & 81.40\% & 1.64\% & 73.83\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \cmark & 26.28\% & 47.43\% & 20.03\% & 81.61\% & 9.18\% & 78.98\% & 1.62\% & 74.65\% & 2.45\% & 81.07\% & 1.67\% & 73.29\% \\ 
        \hline
        \multirow{3}{*}{Magicoder} & \cmark & \multirow{2}{*}{Zero-shot} & \xmark & 27.43\% & 44.85\% & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\ 
        \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \xmark & 9.75\% & 39.43\% & 8.65\% & 73.90\% & 0.81\% & 59.50\% & 0.16\% & 47.30\% & 0.08\% & 48.85\% & 0.04\% & 44.38\% \\ \cline{2-16}
        ~ & \xmark & Few-shot & \xmark & 15.97\% & 36.24\% & 2.93\% & 4.36\% & 1.99\% & 7.50\% & 0.22\% & 37.56\% & 0.49\% & 42.52\% & 0.74\% & 40.45\% \\ 
        \hline
        CodeReviewer & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & 33.23\% & 55.43\% & 15.17\% & 80.83\% & 4.14\% & 78.76\% & 0.54\% & 75.24\% & 0.81\% & 80.10\% & 1.23\% & 75.32\% \\
        \cline{1-1}\cline{5-16}
        TufanoT5 & ~ & ~ & ~ & 11.90\% & 43.39\% & 14.26\% & 79.48\% & 5.40\% & 77.26\% & 0.27\% & 75.88\% & 1.37\% & 82.25\% & 0.19\% & 73.53\% \\
        \cline{1-1}\cline{5-16}
        D-ACT & ~ & ~ & ~ & - & - & - & - & - & - & 0.65\% & 75.99\% & 5.98\% & 81.85\% & 1.79\% & 79.77\% \\ \hline
    \end{tabular}
    }
    \label{tab:result}%
\end{table*}

\section{Result} \label{sec:results}




% % Table generated by Excel2LaTeX from sheet 'result new design'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}[4]{*}{Approach} & \multirow{2}[4]{*}{Fine-Tuned?} & \multirow{2}[4]{*}{prompting} & \multirow{2}[4]{*}{use persona?} & \multicolumn{2}{c|}{CodeReviewer} & \multicolumn{2}{c|}{Tufano (with comment)} & \multicolumn{2}{c|}{Tufano (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
% \cmidrule{5-16}          &       &       &       & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU \\
%     \toprule
%     \multirow{6}[6]{*}{GPT-3.5} & yes   & \multirow{2}[4]{*}{0-shot} & no    & 27.43\% & 44.85 & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\
%     \hline
%     \multirow{3}[6]{*}{Magicoder} & yes   & \multirow{2}[4]{*}{0-shot} & no    & 27.43\% & 44.85 & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\
% \cmidrule{2-2}\cmidrule{4-16}          & no    &       & no    & 9.75\% & 39.43\% & 8.65\% & 73.90\% & 0.81\% & 59.50\% & 0.16\% & 47.30\% & 0.08\% & 48.85\% & 0.04\% & 44.38\% \\
% \cmidrule{2-16}          & no    & few-shot & no    & 15.97\% & 36.24\% & 2.93\% & 4.36\% & 1.99\% & 7.50\% & 0.22\% & 37.56\% & 0.49\% & 42.52\% & 0.74\% & 40.45\% \\
%     \midrule
%     CodeReviewer & \multirow{3}[6]{*}{-} & \multirow{3}[6]{*}{-} & \multirow{3}[6]{*}{-} & 33.23\% & 55.43\% & 15.17\% & 80.83\% & 4.14\% & 78.76\% & 0.54\% & 75.24\% & 0.81\% & 80.10\% & 1.23\% & 75.32\% \\
% \cmidrule{1-1}\cmidrule{5-16}    TufanoT5 &       &       &       & 11.90\% & 43.39\% & 14.26\% & 79.48\% & 5.40\% & 77.26\% & 0.27\% & 75.88\% & 1.37\% & \textbf{82.25\%} & 0.19\% & 73.53\% \\
% \cmidrule{1-1}\cmidrule{5-16}    D-ACT &       &       &       & -     & -     & -     & -     & -     & -     & 0.65\% & \textbf{75.99\%} & 5.98\% & 81.85\% & 1.79\% & \textbf{79.77\%} \\
%     \bottomrule
%     \end{tabular}%
% }
%   \label{tab:addlabel}%
% \end{table*}%



In this section, we present the
% \kla{this word appears again! how should I feel?} 
results of the following three research questions.

\noindent \textbf{(RQ1) \rqone}

\noindent \smallsection{Approach}
To address this RQ, we evaluate the performance of GPT-3.5 against \revised{R2-4}{an open-source LLM called Magicoder~\cite{wei2023magicoder}} and the existing code review automation approaches \revised{R2-3}{
(The details of GPT-3.5, Magicoder and the existing code review automation approaches are shown in Table~\ref{tab:model-detail})
}.
% \revised{R2-4}{
% % In addition, we conduct experiments with an open-source LLM called Magicoder~\cite{wei2023magicoder}.
% We choose Magicoder~\cite{wei2023magicoder} in our experiment since it outperforms other recent open-source instruction-tuned LLMs (e.g., Starcoder~\cite{li2023starcoder}, Deep\-Seek-Coder~\cite{guo2024deepseek} or CodeLLaMa~\cite{roziere2023codeLLaMa}).
% When we perform zero-shot and few-shot learning with Magicoder, we follow the same process as we perform zero-shot and few-shot learning with GPT-3.5.
% For fine-tuning Magicoder, we use the recently proposed parameter-efficient fine-tuning approach called DoRA~\cite{liu2024dora}, which is shown to outperform the LoRA approach.~\cite{hu2021lora}
% }

% In this RQ, we select the results of \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \ChatGPTFineTune~that is generated from input prompts without persona.
% We select such results since they achieve higher EM and CodeBLEU than the ones that are generated from input prompts with persona (as shown in RQ2).

% In this RQ, we evaluate the performance of GPT-3.5 and Magicoder that is generated from input prompts without persona.
% We do so since RQ2 shows that the performance of GPT-3.5 that persona is not included in input prompts is higher than the performance of GPT-3.5 that persona is included in input prompts.


Then, we obtain the results of the existing code review automation approaches.
In particular, we obtain the results of \Tufanomodel~and \DACTmodel~from the replication packages.
However, since Li~\ea~\cite{li2022automating} do not make their results publicly available, we obtain the results from Guo~\ea~\cite{guo2023exploring} instead.
% After that, we compare the results of GPT-3.5 with the existing code review automation approaches by using the same evaluation measures as RQ1-RQ3.
\revised{R1-4}{
In addition, we evaluate the existing code review automation approaches across the studied datasets (e.g., we evaluate \CodeReviewerModel~on the Tufano\textsubscript{Data}~\\and \DACTData~datasets).
However, we do not evaluate \DACTmodel~with the \tufanoData~and \CodeReviewerData~datasets since such datasets do not contain code diff information, which is the component of \DACTmodel.
}

Finally, we measure EM and CodeBLEU of the results obtained from GPT-3.5, Magicoder and the existing code review automation approaches.





\noindent \smallsection{Result}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms the existing code review automation approaches in \tufanoData~and \DACTData.}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms \Tufanomodel~and \DACTmodel.}
% \textbf{The existing code review automation approaches achieve at least 5.47\% higher EM than GPT-3.5 that zero-shot learning is performed while fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.}
\textbf{Fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts achieves at least 11.48\% higher EM than Magicoder and the existing code review automation approaches.}
Table~\ref{tab:result} shows the results of GPT-3.5, Magicoder and the existing co\-de review automation approaches.
The table shows that in terms of EM, fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts achieves at least 38.28\% and 11.48\% higher EM than Magicoder and the existing code review automation approaches, respectively.

In terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~ac\-hieves at least 0.95\% higher than fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts.
In contrast, fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts ac\-hieves at least 9.25\% and 3.3\% higher than Magicoder and \Tufanomodel, respectively.

% The results indicate that model fine-tuning could help GPT-3.5 and Magicoder generate more correct improved code than Magicoder and the existing code review automation approaches.


\noindent \textbf{(RQ2) \rqtwo}

\noindent \smallsection{Approach}
To address this RQ, we fine-tune GPT-3.5 and Magicoder as explained in Section~\ref{sec:study-design}.
% We do so by using prompts that contain persona and do not contain persona similar to RQ2.
Then, similar to RQ1, we measure EM and CodeBLEU of the results obtained from the fine-tuned GPT-3.5\textsubscript{Zero-shot}, GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, fine-tuned Magicoder\textsubscript{Zero-shot} and Magicoder\textsubscript{Zero-shot} that is not fine-tuned.
In this RQ, we evaluate the results of the above approaches that persona is not included in input prompts.


%% fine-tuned Magicoder\textsubscript{Zero-shot} achieves at least 28.79\% higher EM and 13.75\% higher CodeBLEU than Magicoder\textsubscript{Zero-shot} that is not fine-tuned

\noindent \smallsection{Result}
% \textbf{Fine-tuned GPT-3.5\textsubscript{Zero-shot} achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
\textbf{Fine-tuned GPT-3.5\textsubscript{Zero-shot} and fine-tuned Magicoder\textsubscript{Zero-shot} achieves at least 63.91\% and 28.79\% higher EM than those that are not fine-tuned.}

% achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
Table~\ref{tab:result} shows that in terms of EM, fine-tuned GPT-3.5\textsubscript{Zero-shot} achieves at least 63.91\% higher than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned.
Similarly, Magicoder\textsubscript{Zero-shot} achieves at least 63.91\% higher than Magicoder\textsubscript{Zero-shot} that is not fine-tuned.

In terms of CodeBLEU, fine-tuned GPT-3.5\textsubscript{Zero-shot} achieves at least 5.91\% -higher than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned.
Likewise, Magicoder\textsubscript{Zero-shot} achieves at least 13.75\%  higher than Magicoder\textsubscript{Zero-shot} that is not fine-tuned.


The results indicate that model fine-tuning can improve the performance of GPT-3.5 over GPT-3.5 that is not fine-tuned.


% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-1-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (with comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-1-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTZeroShotWithPersona~and \ChatGPTZeroShotWithoutPersona.}
%     \label{fig:RQ2-1-EM-intersection}
% \end{figure*}



% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=5]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-2-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=6]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%       \caption{\tufanoData~dataset (with comment)}
%      \label{fig:RQ2-2-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=7]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-2-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=8]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-2-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ3) Venn diagrams showing EM achieved by \ChatGPTFewShotWithPersona~and \ChatGPTFewShotWithoutPersona.}
%     \label{fig:RQ2-2-EM-intersection}
% \end{figure*}

\noindent \textbf{(RQ3) \rqthree}

\noindent \smallsection{Approach}
To address this RQ, we do zero-shot prompting and few-shot prompting with GPT-3.5 and Magicoder \textbf{(no fine-tuning)} to generate improved code from the prompts in Figure~\ref{fig:prompt-templates} as explained in Section~\ref{sec:study-design}.
% we use the prompts in Figure~\ref{fig:prompt-templates} to enable GPT-3.5 to perform zero-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
Then, we measure EM and CodeBLEU of the results obtained from GPT-3.5.
We use the following symbols to refer to GPT-3.5 in different settings

\begin{itemize}
    \item \ChatGPTZeroShot~for GPT-3.5 that we do zero-shot prompting.
    \item \ChatGPTFewShot~for GPT-3.5 that we do few-shot prompting.
    % \item \ChatGPTZeroShotWithPersona~for GPT-3.5 that we do zero-shot prompting with persona in input prompts.
    % \item \ChatGPTZeroShotWithoutPersona~for GPT-3.5 that we do zero-shot prompting without persona in input prompts.
    % \item \ChatGPTFewShotWithPersona~for GPT-3.5 that we do few-shot prompting with persona in input prompts.
    % \item \ChatGPTFewShotWithoutPersona~for GPT-3.5 that we do few-shot prompting with persona in input prompts.
    \item \MagicoderZeroShot~for Magicoder that we do zero-shot prompting.
    \item \MagicoderFewShot~for Magicoder that we do few-shot prompting.
\end{itemize}

% \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
% Similarly, \hspace{1.5pt} \ChatGPTZeroShot~and GPT-3.5\textsubscript{Few-shot} that generate improved code from the prompts without persona are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.

% GPT-3.5 that zero-shot learning and few-shot learning is performed is denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.



\noindent \smallsection{Result}
\textbf{\ChatGPTFewShot~achieves at least 46.38\% higher EM and 3.97\% higher CodeBLEU than \ChatGPTZeroShot.}
Table~\ref{tab:result} shows that in terms of EM, \ChatGPTFewShot~achieves at least 46.38\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is not included in input prompts, and at least 53.95\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
% Figure~\ref{fig:RQ2-1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-1-EM-intersection-D-ACT} present the Venn diagram of the improved code that \ChatGPTZeroShotWithPersona~and GPT-3.5-NP\textsubscript{Zero-shot} correctly generate.
% The figures show that the number of improved code that only~\ChatGPTZeroShotWithPersona~correctly generates is at least 22.02\% lower than~\ChatGPTZeroShotWithoutPersona.
% Similarly, Figure~\ref{fig:RQ2-2-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-2-EM-intersection-D-ACT} present the Venn diagram of the improved code that GPT-3.5-WP\textsubscript{Few-shot} and \ChatGPTFewShotWithoutPersona~correctly generate.
% The figures show that the number of improved code that only GPT-3.5-WP\textsubscript{Few-shot} correctly generates is at least 16.48\% \hspace{2pt} lower than GPT-3.5-NP\textsubscript{Few-shot}.
On the other hand, \MagicoderFewShot achieves at least 37.5\% higher EM than \MagicoderZeroShot (we use prompts that do not include persona).

In terms of CodeBLEU, \ChatGPTFewShot~achieves at least 3.97\% higher than \ChatGPTZeroShot~when persona is not included in input prompts, and at least 5.55\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
In contrast, \MagicoderFewShot achieves at least 8.8\% lower CodeBLEU than \MagicoderZeroShot (we use prompts that do not include persona).
The possible reason for these results is that GPT-3.5 has a large context size (i.e., 16K tokens) to fit input prompts for few-shot learning.
On the contrary, Magicoder has a small context size (i.e., 2K tokens) which does not fit input prompts for few-shot learning that are longer than 2K tokens.

The results indicate that few-shot prompting can help GPT-3.5 and Magicoder to generate more correct improved code over zero-shot prompting.
However, few-shot learning can only help GPT-3.5 to generate improved code more similar to actual improved code over zero-shot prompting.

% increase the performance of GPT-3.5 over zero-shot prompting.


\textbf{When persona is used in input prompts, the EM and CodeBLEU that GPT-3.5 achieves decrease by at least 3.67\% and 1.33\%, respectively.}
We also observe from the table that GPT-3.5 achieves less EM and CodeBLEU when using prompts that include persona.
In terms of EM, \ChatGPTZeroShot~and \ChatGPTFewShot~achieve at least 3.67\% and 1.02\% lower, respectively.
Similarly, in terms of CodeBLEU, GPT-3.5\textsubscript{ZeroShot} and \ChatGPTFewShot~achieve at least 1.33\% and 0.15\% lower, respectively.
The results indicate that using persona in input prompts has a negative impact on the performance of GPT-3.5.

The above results indicate that the best prompting strategy when using GPT-3.5 without fine-tuning is using few-shot prompting without using persona in input prompts.

==> section-exp-only/Result-old-6.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The statistical details of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \begin{tabular}{|c|c|}
    \hline
    Model & \# parameters \\
    \hline
    GPT-3.5 & 175 B \\
    \hline
    Magicoder~\cite{wei2023magicoder} & 6.7 B \\ 
    \hline
    TufanoT5~\cite{tufano2022using} & 60.5 M \\
    \hline
    CodeReviewer~\cite{li2022automating} & 222.8 M \\
    \hline
    D-ACT~\cite{pornprasit2023d} & 222.8 M \\
    \hline
    \end{tabular}%
  \label{tab:model-detail}%
\end{table}%

\begin{table*}[!h]
    \centering
    \caption{The evaluation results of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{Approach} & \multirow{2}{*}{Fine-Tuning} & \multicolumn{2}{c|}{Inference Technique} & \multicolumn{2}{c|}{CodeReviewer} & \multicolumn{2}{c|}{Tufano (with comment)} & \multicolumn{2}{c|}{Tufano (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
        \cline{3-16}    
         &    & Prompting & Use Persona? & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU & EM & CodeBLEU \\ \hline
        \multirow{6}{*}{GPT-3.5} & \cmark   & \multirow{4}{*}{Zero-shot} & \xmark    & 37.93\% & 49.00\% & 22.16\% & 82.99\% & 6.02\% & 79.81\% & 2.34\% & 74.15\% & 6.71\% & 81.08\% & 3.05\% & 74.67\% \\
        \cline{2-2}\cline{4-16}
        ~ & \cmark & ~ & \cmark & 37.70\% & 49.20\% & 21.98\% & 83.04\% & 6.04\% & 79.76\% & 2.29\% & 74.74\% & 6.14\% & 81.02\% & 2.64\% & 74.95\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \xmark & 17.72\% & 44.17\% &  13.52\% & 78.36\% &  2.62\% & 74.92\% &  0.49\% & 61.85\% & 0.16\% & 61.04\% & 0.48\% & 56.55\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \cmark & 17.07\% & 43.11\% &  12.49\% & 77.32\% &  2.29\% & 73.21\% &  0.57\% & 55.88\% & 0.00\% & 50.65\% &  0.22\% & 45.73\% \\ \cline{2-16}
        ~ & \xmark & \multirow{2}{*}{Few-shot} & \xmark & 26.55\% & 47.50\% & 19.79\% & 81.47\% & 8.96\% & 79.21\% & 2.34\% & 75.33\% & 2.89\% & 81.40\% & 1.64\% & 73.83\% \\ \cline{2-2}\cline{4-16}
        ~ & \xmark & ~ & \cmark & 26.28\% & 47.43\% & 20.03\% & 81.61\% & 9.18\% & 78.98\% & 1.62\% & 74.65\% & 2.45\% & 81.07\% & 1.67\% & 73.29\% \\ 
        \hline
        \multirow{6}{*}{Magicoder} & \cmark   & \multirow{4}{*}{Zero-shot} & \xmark    & 27.43\% & 44.86\% & 11.14\% & 69.77\% & 1.97\% & 69.25\% & 0.27\% & 65.39\% & 0.57\% & 69.30\% & 0.30\% & 64.19\% \\
        \cline{2-2}\cline{4-16}          & \cmark   &       & \cmark   &       &       &       &       &       &       &       &       &       &       &       &  \\
        \cline{2-2}\cline{4-16}          & \xmark    &       & \xmark    & 9.75\% & 39.45\% & 8.65\% & 73.90\% & 0.81\% & 59.49\% & 0.16\% & 47.37\% & 0.08\% & 48.82\% & 0.04\% & 44.38\% \\
        \cline{2-2}\cline{4-16}          & \xmark    &       & \cmark   & 9.93\% & 39.48\% & 8.71\% & 73.57\% & 1.51\% & 67.65\% & 0.27\% & 47.46\% & 0.08\% & 48.58\% & 0.11\% & 43.65\% \\
        \cline{2-16}          & \xmark    & \multirow{2}{*}{Few-shot} & \xmark    & 15.89\% & 36.24\% & 2.93\% & 4.36\% & 1.99\% & 7.49\% & 0.22\% & 37.61\% & 0.49\% & 42.50\% & 0.74\% & 40.33\% \\
        \cline{2-2}\cline{4-16}          & \xmark    &       & \cmark   & 17.80\% & 38.93\% & 2.89\% & 3.70\% & 1.84\% & 6.96\% & 0.27\%  & 16.59\% & 0.65\% & 18.83\% & 0.82\% & 19.55\% \\
        \hline
        CodeReviewer & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & 33.23\% & 55.43\% & 15.17\% & 80.83\% & 4.14\% & 78.76\% & 0.54\% & 75.24\% & 0.81\% & 80.10\% & 1.23\% & 75.32\% \\
        \cline{1-1}\cline{5-16}
        TufanoT5 & ~ & ~ & ~ & 11.90\% & 43.39\% & 14.26\% & 79.48\% & 5.40\% & 77.26\% & 0.27\% & 75.88\% & 1.37\% & 82.25\% & 0.19\% & 73.53\% \\
        \cline{1-1}\cline{5-16}
        D-ACT & ~ & ~ & ~ & - & - & - & - & - & - & 0.65\% & 75.99\% & 5.98\% & 81.85\% & 1.79\% & 79.77\% \\ \hline
    \end{tabular}
    }
    \label{tab:result}%
\end{table*}

\section{Result} \label{sec:results}




% % Table generated by Excel2LaTeX from sheet 'result new design'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}[4]{*}{Approach} & \multirow{2}[4]{*}{Fine-Tuned?} & \multirow{2}[4]{*}{prompting} & \multirow{2}[4]{*}{use persona?} & \multicolumn{2}{c|}{CodeReviewer} & \multicolumn{2}{c|}{Tufano (with comment)} & \multicolumn{2}{c|}{Tufano (without comment)} & \multicolumn{2}{c|}{Android} & \multicolumn{2}{c|}{Google} & \multicolumn{2}{c|}{Ovirt} \\
% \cline{5-16}          &       &       &       & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU & EM    & CodeBLEU \\
%     \toprule
%     \multirow{6}[6]{*}{GPT-3.5} & yes   & \multirow{2}[4]{*}{0-shot} & no    & 27.43\% & 44.85 & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\
%     \hline
%     \multirow{3}[6]{*}{Magicoder} & yes   & \multirow{2}[4]{*}{0-shot} & no    & 27.43\% & 44.85 & 11.14\% & 69.76\% & 1.97\% & 69.25\% & 0.27\% & 65.33\% & 0.57\% & 69.32\% & 0.30\% & 64.21\% \\
% \cline{2-2}\cline{4-16}          & no    &       & no    & 9.75\% & 39.43\% & 8.65\% & 73.90\% & 0.81\% & 59.50\% & 0.16\% & 47.30\% & 0.08\% & 48.85\% & 0.04\% & 44.38\% \\
% \cline{2-16}          & no    & few-shot & no    & 15.97\% & 36.24\% & 2.93\% & 4.36\% & 1.99\% & 7.50\% & 0.22\% & 37.56\% & 0.49\% & 42.52\% & 0.74\% & 40.45\% \\
%     \midrule
%     CodeReviewer & \multirow{3}[6]{*}{-} & \multirow{3}[6]{*}{-} & \multirow{3}[6]{*}{-} & 33.23\% & 55.43\% & 15.17\% & 80.83\% & 4.14\% & 78.76\% & 0.54\% & 75.24\% & 0.81\% & 80.10\% & 1.23\% & 75.32\% \\
% \cline{1-1}\cline{5-16}    TufanoT5 &       &       &       & 11.90\% & 43.39\% & 14.26\% & 79.48\% & 5.40\% & 77.26\% & 0.27\% & 75.88\% & 1.37\% & \textbf{82.25\%} & 0.19\% & 73.53\% \\
% \cline{1-1}\cline{5-16}    D-ACT &       &       &       & -     & -     & -     & -     & -     & -     & 0.65\% & \textbf{75.99\%} & 5.98\% & 81.85\% & 1.79\% & \textbf{79.77\%} \\
%     \bottomrule
%     \end{tabular}%
% }
%   \label{tab:addlabel}%
% \end{table*}%



In this section, we present the
% \kla{this word appears again! how should I feel?} 
results of the following three research questions.

\noindent \textbf{(RQ1) \rqone}

\noindent \smallsection{Approach}
To address this RQ, we evaluate the performance of GPT-3.5 against \revised{R2-4}{an open-source LLM called Magicoder~\cite{wei2023magicoder}} and the existing code review automation approaches \revised{R2-3}{
(The details of GPT-3.5, Magicoder and the existing code review automation approaches are shown in Table~\ref{tab:model-detail})
}.
% \revised{R2-4}{
% % In addition, we conduct experiments with an open-source LLM called Magicoder~\cite{wei2023magicoder}.
% We choose Magicoder~\cite{wei2023magicoder} in our experiment since it outperforms other recent open-source instruction-tuned LLMs (e.g., Starcoder~\cite{li2023starcoder}, Deep\-Seek-Coder~\cite{guo2024deepseek} or CodeLLaMa~\cite{roziere2023codeLLaMa}).
% When we perform zero-shot and few-shot learning with Magicoder, we follow the same process as we perform zero-shot and few-shot learning with GPT-3.5.
% For fine-tuning Magicoder, we use the recently proposed parameter-efficient fine-tuning approach called DoRA~\cite{liu2024dora}, which is shown to outperform the LoRA approach.~\cite{hu2021lora}
% }

% In this RQ, we select the results of \ChatGPTZeroShot, GPT-3.5\textsubscript{Few-shot} and \ChatGPTFineTune~that is generated from input prompts without persona.
% We select such results since they achieve higher EM and CodeBLEU than the ones that are generated from input prompts with persona (as shown in RQ2).

% In this RQ, we evaluate the performance of GPT-3.5 and Magicoder that is generated from input prompts without persona.
% We do so since RQ2 shows that the performance of GPT-3.5 that persona is not included in input prompts is higher than the performance of GPT-3.5 that persona is included in input prompts.


Then, we obtain the results of the existing code review automation approaches.
In particular, we obtain the results of \Tufanomodel~and \DACTmodel~from the replication packages.
However, since Li~\ea~\cite{li2022automating} do not make their results publicly available, we obtain the results from Guo~\ea~\cite{guo2023exploring} instead.
% After that, we compare the results of GPT-3.5 with the existing code review automation approaches by using the same evaluation measures as RQ1-RQ3.
\revised{R1-4}{
In addition, we evaluate the existing code review automation approaches across the studied datasets (e.g., we evaluate \CodeReviewerModel~on the Tufano\textsubscript{Data}~\\and \DACTData~datasets).
However, we do not evaluate \DACTmodel~with the \tufanoData~and \CodeReviewerData~datasets since such datasets do not contain code diff information, which is the component of \DACTmodel.
}

Finally, we measure EM and CodeBLEU of the results obtained from GPT-3.5, Magicoder and the existing code review automation approaches.





\noindent \smallsection{Result}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms the existing code review automation approaches in \tufanoData~and \DACTData.}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms \Tufanomodel~and \DACTmodel.}
% \textbf{The existing code review automation approaches achieve at least 5.47\% higher EM than GPT-3.5 that zero-shot learning is performed while fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.}
\textbf{Fine-tuned GPT-3.5 that we leverage zero-shot learning without persona achieves 11.48\% - 8,287.5\% higher EM than Magicoder and the existing code review automation approaches.}
Table~\ref{tab:result} shows the results of GPT-3.5, Magicoder and the existing co\-de review automation approaches.
The table shows that in terms of EM, fine-tuned GPT-3.5 that we leverage zero-shot learning without persona achieves 38.28\% - 8,287.5\% and 11.48\% - 1,505.26\% higher than Magicoder and the existing code review automation approaches, respectively.
Similarly, in terms of CodeBLEU, fine-tuned GPT-3.5 that we leverage zero-shot learning without persona achieves 9.25\% - 1,803.44\% and 1.22\% - 12.93\% higher than Magicoder and the existing code review automation approaches, respectively.

The results indicate that leveraging model fine-tuning and zero-shot learning without persona for GPT-3.5 could help GPT-3.5 to achieve the highest EM and CodeBLEU when compared to Magicoder and the existing code review automation approaches.
The highest EM and CodeBLEU achieved by the fine-tuned GPT-3.5 has to do with the size of GPT-3.5.
As presented in Table~\ref{tab:model-detail}, GPT-3.5 has the highest number of parameters (175 billion) when compared to Magicoder and the existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d}
% (6.7 billion) and the existing code review automation approaches (60.5 million for \Tufanomodel~\cite{tufano2022using} and 222.8 million for \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d}).
Thus, larger LLMs tend to achieve higher EM and CodeBLEU than smaller LLMs.



% In terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~ac\-hieves at least 0.95\% higher than fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts.
% In contrast, fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts ac\-hieves at least 9.25\% and 3.3\% higher than Magicoder and \Tufanomodel, respectively.

% The results indicate that model fine-tuning could help GPT-3.5 and Magicoder generate more correct improved code than Magicoder and the existing code review automation approaches.


\noindent \textbf{(RQ2) \rqtwo}

\noindent \smallsection{Approach}
To address this RQ, we fine-tune GPT-3.5 and Magicoder as explained in Section~\ref{sec:study-design}.
% We do so by using prompts that contain persona and do not contain persona similar to RQ2.
Then, similar to RQ1, we measure EM and CodeBLEU of the results obtained from the fine-tuned GPT-3.5 and Magicoder that we leverage zero-shot learning, and the non fine-tuned GPT-3.5 and Magicoder that we leverage zero-shot learning.
% GPT-3.5\textsubscript{Zero-shot}, GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, fine-tuned Magicoder\textsubscript{Zero-shot} and Magicoder\textsubscript{Zero-shot} that is not fine-tuned.
In this RQ, we evaluate the results of the above approaches that persona is not included in prompts.


%% fine-tuned Magicoder\textsubscript{Zero-shot} achieves at least 28.79\% higher EM and 13.75\% higher CodeBLEU than Magicoder\textsubscript{Zero-shot} that is not fine-tuned

\noindent \smallsection{Result}
% \textbf{Fine-tuned GPT-3.5\textsubscript{Zero-shot} achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
% Fine-tuned GPT-3.5 that we leverage zero-shot learning without persona achieves
\textbf{Fine-tuned GPT-3.5 and Magicoder that we leverage zero-shot learning achieves 63.91\% - 1,100\% and ...\% - ...\% higher EM than non fine-tuned GPT-3.5 and Magicoder that we leverage zero-shot learning, respectively.}

% achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
Table~\ref{tab:result} shows that in terms of EM, fine-tuned GPT-3.5 that we leverage zero-shot learning achieves 63.91\% - 1,100\% higher than those that are not fine-tuned.
Similarly, fine-tuned Magicoder that we leverage zero-shot learning achieves ...\% - ...\% higher than those that are not fine-tuned.

In terms of CodeBLEU, fine-tuned GPT-3.5 that we leverage zero-shot learning achieves 5.91\% - 63.9\% higher than those that are not fine-tuned.
Likewise, fine-tuned Magicoder that we leverage zero-shot learning achieves ...\% - ...\% higher than those that are not fine-tuned.


The results indicate that fine-tuned GPT-3.5 and Magicoder achieve higher EM and CodeBLEU than those that are not fine-tuned.
During the model fine-tuning process, GPT-3.5 and Magicoder directly learn the relationship between the input (i.e., code submitted for review and a reviewer's comment) and output (i.e., revised code) from a number of examples in a training set.
In contrast, non fine-tuned GPT-3.5 and Magicoder are given only instruction and input which are not presented during model pre-training.
Therefore, fine-tuned GPT-3.5 and Magicoder can better adapt to the code review automation task than those that are not fine-tuned.
% Therefore, the results imply that model fine-tuning could help GPT-3.5 and Magicoder to adapt to the code review automation task.


% model fine-tuning can improve the performance of GPT-3.5 and Magicoder over those that are not fine-tuned.



% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-1-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (with comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-1-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTZeroShotWithPersona~and \ChatGPTZeroShotWithoutPersona.}
%     \label{fig:RQ2-1-EM-intersection}
% \end{figure*}



% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=5]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-2-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=6]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%       \caption{\tufanoData~dataset (with comment)}
%      \label{fig:RQ2-2-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=7]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-2-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=8]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-2-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ3) Venn diagrams showing EM achieved by \ChatGPTFewShotWithPersona~and \ChatGPTFewShotWithoutPersona.}
%     \label{fig:RQ2-2-EM-intersection}
% \end{figure*}


\begin{figure*}[h]
     \centering
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=1]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 that we leverage zero-shot learning without persona correctly generates.}
         \label{fig:RQ2-0-shot-no-persona}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0
         0 0 0}, clip, page=2]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 that we leverage zero-shot learning with persona incorrectly generates.}
         \label{fig:RQ2-0-shot-with-persona}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=3]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 that we leverage few-shot learning without persona correctly generates.}
        \label{fig:RQ2-few-shot-no-persona}
     \end{subfigure}
    \begin{subfigure}[]{\columnwidth}
         \centering
        \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=4]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 that we leverage few-shot learning with persona  incorrectly generates.}
         \label{fig:RQ2-few-shot-with-persona}
     \end{subfigure}
     
    \caption{(RQ3) Example of the difference between code submitted for review and revised code generated by GPT-3.5 that we leverage zero-shot and few-shot learning.}
    \label{fig:RQ2-code-change-with-and-without-persona}
\end{figure*}

\noindent \textbf{(RQ3) \rqthree}

\noindent \smallsection{Approach}
To address this RQ, we leverage zero-shot learning and few-shot learning with \textit{non fine-tuned} GPT-3.5 and Magicoder to generate revised code from the prompts in Figure~\ref{fig:prompt-templates} as explained in Section~\ref{sec:study-design}.
% we use the prompts in Figure~\ref{fig:prompt-templates} to enable GPT-3.5 to perform zero-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
Then, we measure EM and CodeBLEU of the results obtained from GPT-3.5 and Magicoder.
% We use the following symbols to refer to GPT-3.5 in different settings

% \begin{itemize}
%     \item \ChatGPTZeroShot~for GPT-3.5 that we do zero-shot prompting.
%     \item \ChatGPTFewShot~for GPT-3.5 that we do few-shot prompting.
%     % \item \ChatGPTZeroShotWithPersona~for GPT-3.5 that we do zero-shot prompting with persona in input prompts.
%     % \item \ChatGPTZeroShotWithoutPersona~for GPT-3.5 that we do zero-shot prompting without persona in input prompts.
%     % \item \ChatGPTFewShotWithPersona~for GPT-3.5 that we do few-shot prompting with persona in input prompts.
%     % \item \ChatGPTFewShotWithoutPersona~for GPT-3.5 that we do few-shot prompting with persona in input prompts.
%     \item \MagicoderZeroShot~for Magicoder that we do zero-shot prompting.
%     \item \MagicoderFewShot~for Magicoder that we do few-shot prompting.
% \end{itemize}

% \ChatGPTZeroShotWithPersona~and \ChatGPTFewShotWithPersona, respectively.
% Similarly, \hspace{1.5pt} \ChatGPTZeroShot~and GPT-3.5\textsubscript{Few-shot} that generate improved code from the prompts without persona are denoted as \ChatGPTZeroShotWithoutPersona~and \ChatGPTFewShotWithoutPersona, respectively.

% GPT-3.5 that zero-shot learning and few-shot learning is performed is denoted as \ChatGPTZeroShot~and \ChatGPTFewShot, respectively.



\noindent \smallsection{Result}
\textbf{GPT-3.5 and Magicoder that we leverage few-shot learning achieve 46.38\% - 659.09\% and ...\% - ...\% higher EM than those that we leverage zero-shot learning, respectively.}


Table~\ref{tab:result} shows that in terms of EM, GPT-3.5 that we leverage few-shot learning achieves 46.38\% - 241.98\% and 53.95\% - 659.09\% higher than GPT-3.5 that we leverage zero-shot learning without persona and with persona, respectively.
Similarly, Magicoder that we leverage few-shot learning achieves 37.5\% - 1,750\% and 21.85\% - 645.45\% higher than Magicoder that we leverage zero-shot learning without persona and with persona, respectively.

In terms of CodeBLEU, GPT-3.5 that we leverage few-shot learning achieves 3.97\% - 33.36\% and 5.55\% - 60.27\% higher than GPT-3.5 that we leverage zero-shot learning without persona and with persona, respectively.
In contrast, Magicoder that we leverage few-shot learning achieves 8.14\% - 94.1\% and 1.39\% - 94.97\% lower than Magicoder that we leverage zero-shot learning without persona and with persona, respectively.
% The possible reason for these results is that GPT-3.5 has a large context size (i.e., 16K tokens) to fit input prompts for few-shot learning.
% On the contrary, Magicoder has a small context size (i.e., 2K tokens) which does not fit input prompts for few-shot learning that are longer than 2K tokens.

The results indicate that GPT-3.5 and Magicoder that we leverage few-shot learning can achieve higher EM than those that leverage zero-shot learning.
When few-shot learning is leveraged to generate revised code from GPT-3.5 and Magicoder, such models have more information from given demonstration examples in a prompt to guide the generation of revised code from given code submitted for review.
In other words, such demonstration examples could help GPT-3.5 and Magicoder to generate more correct revised code.

% However, the results indicate that only GPT-3.5 that we leverage few-shot learning can achieve higher CodeBLEU than those that leverage zero-shot learning.
% The higher CodeBLEU achieved by GPT-3.5 has to do with the context length of GPT-3.5 that fits the given demonstration examples in a prompt.
However, the results indicate that only Magicoder that we leverage few-shot learning achieves lower CodeBLEU than those that leverage zero-shot learning.
The lower CodeBLEU achieved by Magicoder has to do with the length of prompts and output that exceed the context length of Magicoder (i.e., 2,048 tokens).
Thus, it is possible that the output from Magicoder that we leverage few-shot learning does not contain the revised code that Magicoder is expected to generate.

% generates revised code that does not look similar to the actual revised code in a testing set.

% understand the relationship between submitted code and revised code.

% Such given examples could help GPT-3.5 and Magicoder to generate more correct revised code.




% The results indicate that few-shot  can help GPT-3.5 and Magicoder to generate more correct improved code over zero-shot prompting.
% However, few-shot learning can only help GPT-3.5 to generate improved code more similar to actual improved code over zero-shot prompting.

% Table~\ref{tab:result} shows that in terms of EM, \ChatGPTFewShot~achieves at least 46.38\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is not included in input prompts, and at least 53.95\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
% Figure~\ref{fig:RQ2-1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-1-EM-intersection-D-ACT} present the Venn diagram of the improved code that \ChatGPTZeroShotWithPersona~and GPT-3.5-NP\textsubscript{Zero-shot} correctly generate.
% The figures show that the number of improved code that only~\ChatGPTZeroShotWithPersona~correctly generates is at least 22.02\% lower than~\ChatGPTZeroShotWithoutPersona.
% Similarly, Figure~\ref{fig:RQ2-2-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-2-EM-intersection-D-ACT} present the Venn diagram of the improved code that GPT-3.5-WP\textsubscript{Few-shot} and \ChatGPTFewShotWithoutPersona~correctly generate.
% The figures show that the number of improved code that only GPT-3.5-WP\textsubscript{Few-shot} correctly generates is at least 16.48\% \hspace{2pt} lower than GPT-3.5-NP\textsubscript{Few-shot}.
% On the other hand, \MagicoderFewShot achieves at least 37.5\% higher EM than \MagicoderZeroShot (we use prompts that do not include persona).

% In terms of CodeBLEU, \ChatGPTFewShot~achieves at least 3.97\% higher than \ChatGPTZeroShot~when persona is not included in input prompts, and at least 5.55\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
% In contrast, \MagicoderFewShot achieves at least 8.8\% lower CodeBLEU than \MagicoderZeroShot (we use prompts that do not include persona).
% The possible reason for these results is that GPT-3.5 has a large context size (i.e., 16K tokens) to fit input prompts for few-shot learning.
% On the contrary, Magicoder has a small context size (i.e., 2K tokens) which does not fit input prompts for few-shot learning that are longer than 2K tokens.

% The results indicate that few-shot prompting can help GPT-3.5 and Magicoder to generate more correct improved code over zero-shot prompting.
% However, few-shot learning can only help GPT-3.5 to generate improved code more similar to actual improved code over zero-shot prompting.

% increase the performance of GPT-3.5 over zero-shot prompting.

% \textbf{When persona is used in input prompts, the EM and CodeBLEU that GPT-3.5 achieves decrease by at least 3.67\% and 1.33\%, respectively.}
\textbf{When a persona is included in input prompts, GPT-3.5 achieves 0.15\% - 30.77\% lower EM than when the persona is not included in input prompts.}
% We also observe from the table that GPT-3.5 and Magicoder achieves less EM and CodeBLEU when a persona is included in prompts.
Table~\ref{tab:result} also shows that in terms of EM, GPT-3.5 that we leverage zero-shot and few-shot learning without persona achieves 3.67\% - 54.17\% and 1.02\% - 30.77\% lower than GPT-3.5 that we leverage zero-shot and few-shot learning with persona, respectively.
In contrast, Magicoder that we leverage zero-shot and few-shot learning with persona achieves 0.69\% - 175\% and 10.81\% - 32.65\% higher than Magicoder that we leverage zero-shot and few-shot learning with persona, respectively.


In terms of CodeBLEU, GPT-3.5 that we leverage zero-shot and few-shot learning with persona achieves 1.33\% - 19.13\% and 0.15\% - 0.90\% lower than GPT-3.5 that we leverage zero-shot and few-shot learning without persona, respectively.
In addition, Magicoder that we leverage few-shot learning with persona achieves 7.08\% - 55.89\% lower CodeBLEU than Magicoder that we leverage zero-shot learning without persona.
On the contrary, Magicoder that we leverage zero-shot learning with persona achieves 0.08\% - 13.72\% higher CodeBLEU than Magicoder that we leverage zero-shot without persona.


% The results indicate that GPT-3.5 and Magicoder that we leverage zero-shot learning and few-shot learning achieve lower EM and CodeBLEU when a persona is included in prompts.
The results imply that ...
\revised{R2-1}{
To illustrate the impact of the persona, we present an example of the revised code generated by GPT-3.5 that we leverage zero-shot learning with and without persona, and an example of the revised code generated by GPT-3.5 that we leverage few-shot learning with and without persona below.

Figure~\ref{fig:RQ2-0-shot-no-persona} presents the revised code that GPT-3.5 that we leverage zero-shot learning without persona correctly generates by suggesting an alternative way to initialize variable \texttt{logArg}.
In contrast, Figure~\ref{fig:RQ2-0-shot-with-persona} presents the revised code that GPT-3.5 that we leverage zero-shot learning with persona incorrectly generates by suggesting changing the variable type from \texttt{Boolean} to \texttt{boolean} and changing the variable name from \texttt{sample\_name} to \texttt{sampleName}, in addition to suggesting an alternative way to initialize variable \texttt{logArg}.
% by suggesting the same change to \ChatGPTZeroShot~(without persona) and additional cha\-nges (i.e., changing variable type from \texttt{Boolean} to \texttt{boolean} and changing variable name from \texttt{sample\_name} to \texttt{sampleName}).

Figure~\ref{fig:RQ2-few-shot-no-persona} presents another example of the revised code that GPT-3.5 that we leverage few-shot learning without persona correctly generates by suggesting new \texttt{if} condition.
On the contrary, Figure~\ref{fig:RQ2-few-shot-with-persona} presents the revised code that GPT-3.5 that we leverage few-shot learning with persona incorrectly generates by suggesting an additional \texttt{if} statement and additional \texttt{else} block.

The above examples imply that when a persona is included in prompts, GPT-3.5 tends to suggest additional incorrect changes to the submitted code compared to when a persona is not included in prompts
}

% using persona in input prompts has a negative impact on the performance of GPT-3.5.


The above results indicate that the best prompting strategy when using GPT-3.5 and Magicoder without fine-tuning is using few-shot learning without a persona.

==> section-exp-only/Result-old-7.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[ht]
  \centering
  \caption{The statistical details of GPT-3.5, Magicoder and the existing code review automation approaches.}
    \begin{tabular}{|c|c|}
    \hline
    Model & \# parameters \\
    \hline
    GPT-3.5 & 175 B \\
    \hline
    Magicoder~\cite{wei2023magicoder} & 6.7 B \\ 
    \hline
    TufanoT5~\cite{tufano2022using} & 60.5 M \\
    \hline
    CodeReviewer~\cite{li2022automating} & 222.8 M \\
    \hline
    D-ACT~\cite{pornprasit2023d} & 222.8 M \\
    \hline
    \end{tabular}%
  \label{tab:model-detail}%
\end{table}%

\section{Result} \label{sec:results}


In this section, we present the
% \kla{this word appears again! how should I feel?} 
results of the following three research questions.

\noindent \textbf{(RQ1) \rqone}

\noindent \smallsection{Approach}
To address this RQ, we evaluate GPT-3.5, Magicoder~\cite{wei2023magicoder} and the existing code review automation approaches~\cite{pornprasit2023d, li2022automating, tufano2022using} \revised{R2-5}{
(The details of GPT-3.5, Magicoder and the existing code review automation approaches are shown in Table~\ref{tab:model-detail})
}.
For the existing code review automation approaches, we obtain the results of \Tufanomodel~\cite{tufano2022using}~and \DACTmodel~\cite{pornprasit2023d}~from the replication packages of such approaches.
On the other hand, we obtain the results of \CodeReviewerModel~\cite{li2022automating}~from the replication package of Guo~\ea~\cite{guo2023exploring} since Li~\ea~\cite{li2022automating} do not make their results publicly available.
\revised{R1-3}{
In addition, we evaluate such approaches on the datasets that are not included in original studies (e.g., we evaluate \CodeReviewerModel~on the Tufano\textsubscript{Data}~and \DACTData~datasets that are not included in Li~\ea's study~\cite{li2022automating}).
However, we do not evaluate \DACTmodel~on the \CodeReviewerData~and \tufanoData~datasets since such datasets lack token-level code difference, which is the component of \DACTmodel.
}
Finally, we measure EM and CodeBLEU of the results obtained from GPT-3.5, Magicoder and the existing code review automation approaches.



\begin{figure*}[h]
     \centering
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=1]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 correctly generates when we use zero-shot learning without a persona.}
         \label{fig:RQ3-0-shot-no-persona}
     \end{subfigure}
     % \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0
         0 0 0}, clip, page=2]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 incorrectly generates when we use zero-shot learning with a persona.}
         \label{fig:RQ3-0-shot-with-persona}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=3]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 correctly generates when we use few-shot learning without a persona.}
        \label{fig:RQ3-few-shot-no-persona}
     \end{subfigure}
    \begin{subfigure}[]{\columnwidth}
         \centering
        \includegraphics[width=\columnwidth, trim = {0 0 0 0}, clip, page=4]{figure/sample-diff-with-and-without-persona.pdf}
         \caption{The difference between code submitted for review and revised code that GPT-3.5 incorrectly generates when we use few-shot learning with a persona.}
         \label{fig:RQ3-few-shot-with-persona}
     \end{subfigure}
     
    \caption{(RQ3) Examples of the difference between code submitted for review and revised code generated by GPT-3.5 that zero-shot learning and few-shot learning are used.}
    \label{fig:RQ3-code-change-with-and-without-persona}
\end{figure*}


\noindent \smallsection{Result}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms the existing code review automation approaches in \tufanoData~and \DACTData.}
% \textbf{The existing code review automation approaches always outperform \ChatGPTZeroShot~while \ChatGPTFineTune~outperforms \Tufanomodel~and \DACTmodel.}
% \textbf{The existing code review automation approaches achieve at least 5.47\% higher EM than GPT-3.5 that zero-shot learning is performed while fine-tuned GPT-3.5 achieves at least 11.48\% higher EM than the existing code review automation approaches.}
\textbf{Fine-tuned GPT-3.5 that zero-shot learning is used without a persona achieves 11.48\% - 8,287.5\% higher EM than Magicoder and the existing code review automation approaches.}
Table~\ref{tab:result} shows the results of EM and CodeBLEU achieved by GPT-3.5, Magicoder and the existing code review automation approaches across the studied datasets (i.e., CodeReview\-er\textsubscript{Data}, \tufanoData, and \DACTData).
% the results of GPT-3.5, Magicoder and the existing co\-de review automation approaches.
The table shows that in terms of EM, fine-tuned GPT-3.5 that zero-shot learning is used without a persona achieves 38.28\% - 8,287.5\% and 11.48\% - 1,505.26\% higher than Magicoder and the existing code review automation approaches, respectively.
Similarly, in terms of CodeBLEU, fine-tuned GPT-3.5 that zero-shot learning is used without a persona achieves 9.25\% - 1,803.44\% and 1.22\% - 12.93\% higher than Magicoder and the existing code review automation approaches, respectively.

The results indicate that model fine-tuning and zero-shot learning without a persona could help GPT-3.5 to achieve the highest EM and CodeBLEU when compared to Magicoder and the existing code review automation approaches.
The highest EM and CodeBLEU achieved by the fine-tuned GPT-3.5 has to do with the size of GPT-3.5.
As presented in Table~\ref{tab:model-detail}, GPT-3.5 has the highest number of parameters (175 billion) when compared to Magicoder and the existing code review automation approaches~\cite{pornprasit2023d, li2022automating, tufano2022using}.
% (6.7 billion) and the existing code review automation approaches (60.5 million for \Tufanomodel~\cite{tufano2022using} and 222.8 million for \CodeReviewerModel~\cite{li2022automating} and \DACTmodel~\cite{pornprasit2023d}).
% Thus, larger LLMs tend to achieve higher EM and CodeBLEU than smaller LLMs.
Thus, fine-tuned GPT-3.5 can better learn the relationship between inputs (i.e., code submitted for review and a reviewer comment) and an output (i.e., revised code) than Magicoder and the existing code review automation approaches.


% In terms of CodeBLEU, \CodeReviewerModel~and \DACTmodel~ac\-hieves at least 0.95\% higher than fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts.
% In contrast, fine-tuned GPT-3.5\textsubscript{Zero-shot} that persona is not included in input prompts ac\-hieves at least 9.25\% and 3.3\% higher than Magicoder and \Tufanomodel, respectively.

% The results indicate that model fine-tuning could help GPT-3.5 and Magicoder generate more correct improved code than Magicoder and the existing code review automation approaches.




\noindent \textbf{(RQ2) \rqtwo}

\noindent \smallsection{Approach}
To address this RQ, we fine-tune GPT-3.5 as explained in Section~\ref{sec:study-design}.
% We do so by using prompts that contain persona and do not contain persona similar to RQ2.
Then, similar to RQ1, we measure EM and CodeBLEU of the results obtained from the fine-tuned GPT-3.5 and the non fine-tuned GPT-3.5 that zero-shot learning is used. % without a persona.
% GPT-3.5\textsubscript{Zero-shot}, GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, fine-tuned Magicoder\textsubscript{Zero-shot} and Magicoder\textsubscript{Zero-shot} that is not fine-tuned.
% In this RQ, we evaluate the results of the above approaches that persona is not included in prompts.


%% fine-tuned Magicoder\textsubscript{Zero-shot} achieves at least 28.79\% higher EM and 13.75\% higher CodeBLEU than Magicoder\textsubscript{Zero-shot} that is not fine-tuned

\noindent \smallsection{Result}
% \textbf{Fine-tuned GPT-3.5\textsubscript{Zero-shot} achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
% Fine-tuned GPT-3.5 that we leverage zero-shot learning without a persona achieves
\textbf{Fine-tuned GPT-3.5 that zero-shot learning is used achieves 63.91\% - 1,100\% higher EM than those that are not fine-tuned.}
% achieves at least 63.91 \% and 5.91\% higher EM and CodeBLEU than GPT-3.5\textsubscript{Zero-shot} that is not fine-tuned, respectively.}
Table~\ref{tab:result} shows that in terms of EM, fine-tuned GPT-3.5 that zero-shot learning is used achieves 63.91\% - 1,100\% higher than those that are not fine-tuned.
In terms of CodeBLEU, fine-tuned GPT-3.5 that zero-shot learning is used achieves 5.91\% - 63.9\% higher than those that are not fine-tuned.


The results indicate that fine-tuned GPT-3.5 achieve higher EM and CodeBLEU than those that are not fine-tuned.
During the model fine-tuning process, GPT-3.5 adapt to the code review automation task by directly learning the relationship between inputs (i.e., code submitted for review and a reviewer's comment) and an output (i.e., revised code) from a number of examples in a training set.
In contrast, non fine-tuned GPT-3.5 is given only an instruction and inputs which are not presented during model pre-training.
Therefore, fine-tuned GPT-3.5 can better adapt to the code review automation task than those that are not fine-tuned.
% Therefore, the results imply that model fine-tuning could help GPT-3.5 and Magicoder to adapt to the code review automation task.


% model fine-tuning can improve the performance of GPT-3.5 and Magicoder over those that are not fine-tuned.



% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=1]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-1-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=2]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (with comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=3]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-1-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=4]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-1-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ2) Venn diagrams showing EM achieved by \ChatGPTZeroShotWithPersona~and \ChatGPTZeroShotWithoutPersona.}
%     \label{fig:RQ2-1-EM-intersection}
% \end{figure*}



% \begin{figure*}[!h]
%      \centering
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=5]{figure/EM-RQ2.pdf}
%          \caption{\CodeReviewerData~dataset}
%          \label{fig:RQ2-2-EM-intersection-CodeRec}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=6]{figure/EM-RQ2.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%       \caption{\tufanoData~dataset (with comment)}
%      \label{fig:RQ2-2-EM-intersection-tufano-code-comment}
%      \end{subfigure}
%      % \par\bigskip 
%      \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=7]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%           \caption{\tufanoData~dataset (without comment)}
%          \label{fig:RQ2-2-EM-intersection-tufano-code}
%      \end{subfigure}
%     \begin{subfigure}[]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth, trim = {0 0 0 0}, clip, page=8]{figure/EM-RQ2.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{\DACTData~dataset}
%          \label{fig:RQ2-2-EM-intersection-D-ACT}
%      \end{subfigure}
     
%      \caption{(RQ3) Venn diagrams showing EM achieved by \ChatGPTFewShotWithPersona~and \ChatGPTFewShotWithoutPersona.}
%     \label{fig:RQ2-2-EM-intersection}
% \end{figure*}






\noindent \textbf{(RQ3) \rqthree}

\noindent \smallsection{Approach}
To address this RQ, we use zero-shot learning and few-shot learning with \textit{non fine-tuned} GPT-3.5,  where each inference technique is used with and without a persona, to generate revised code as explained in Section~\ref{sec:study-design}.
% we use the prompts in Figure~\ref{fig:prompt-templates} to enable GPT-3.5 to perform zero-shot and few-shot learning as explained in Section~\ref{sec:study-design}.
Then, similar to RQ2, we measure EM and CodeBLEU of the results obtained from GPT-3.5.


\noindent \smallsection{Result}
\textbf{GPT-3.5 that few-shot learning is used achieve 46.38\% - 659.09\% higher EM than those that zero-shot learning is used.}
Table~\ref{tab:result} shows that in terms of EM, GPT-3.5 that few-shot learning is used achieves 46.38\% - 241.98\% and 53.95\% - 659.09\% higher than GPT-3.5 that zero-shot learning without a persona and with a persona is used, respectively.
In terms of CodeBLEU, GPT-3.5 that few-shot learning is used achieves 3.97\% - 33.36\% and 5.55\% - 60.27\% higher than GPT-3.5 that zero-shot learning without a persona and with a persona is used, respectively.

The results indicate that GPT-3.5 that few-shot learning is used can achieve higher EM and CodeBLEU than those that zero-shot learning is used.
When few-shot learning is used to generate revised code from GPT-3.5, GPT-3.5 has more information from given demonstration examples in a prompt to guide the generation of revised code from given code submitted for review and a reviewer's comment.
In other words, such demonstration examples could help GPT-3.5 to correctly generate revised code from a given code submitted for review and a reviewer's comment.

% generates revised code that does not look similar to the actual revised code in a testing set.

% understand the relationship between submitted code and revised code.

% Such given examples could help GPT-3.5 and Magicoder to generate more correct revised code.




% The results indicate that few-shot  can help GPT-3.5 and Magicoder to generate more correct improved code over zero-shot prompting.
% However, few-shot learning can only help GPT-3.5 to generate improved code more similar to actual improved code over zero-shot prompting.

% Table~\ref{tab:result} shows that in terms of EM, \ChatGPTFewShot~achieves at least 46.38\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is not included in input prompts, and at least 53.95\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
% Figure~\ref{fig:RQ2-1-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-1-EM-intersection-D-ACT} present the Venn diagram of the improved code that \ChatGPTZeroShotWithPersona~and GPT-3.5-NP\textsubscript{Zero-shot} correctly generate.
% The figures show that the number of improved code that only~\ChatGPTZeroShotWithPersona~correctly generates is at least 22.02\% lower than~\ChatGPTZeroShotWithoutPersona.
% Similarly, Figure~\ref{fig:RQ2-2-EM-intersection-CodeRec} - Figure~\ref{fig:RQ2-2-EM-intersection-D-ACT} present the Venn diagram of the improved code that GPT-3.5-WP\textsubscript{Few-shot} and \ChatGPTFewShotWithoutPersona~correctly generate.
% The figures show that the number of improved code that only GPT-3.5-WP\textsubscript{Few-shot} correctly generates is at least 16.48\% \hspace{2pt} lower than GPT-3.5-NP\textsubscript{Few-shot}.
% On the other hand, \MagicoderFewShot achieves at least 37.5\% higher EM than \MagicoderZeroShot (we use prompts that do not include persona).

% In terms of CodeBLEU, \ChatGPTFewShot~achieves at least 3.97\% higher than \ChatGPTZeroShot~when persona is not included in input prompts, and at least 5.55\% higher than GPT-3.5\textsubscript{Zero-shot}~when persona is included in input prompts.
% In contrast, \MagicoderFewShot achieves at least 8.8\% lower CodeBLEU than \MagicoderZeroShot (we use prompts that do not include persona).
% The possible reason for these results is that GPT-3.5 has a large context size (i.e., 16K tokens) to fit input prompts for few-shot learning.
% On the contrary, Magicoder has a small context size (i.e., 2K tokens) which does not fit input prompts for few-shot learning that are longer than 2K tokens.

% The results indicate that few-shot prompting can help GPT-3.5 and Magicoder to generate more correct improved code over zero-shot prompting.
% However, few-shot learning can only help GPT-3.5 to generate improved code more similar to actual improved code over zero-shot prompting.

% increase the performance of GPT-3.5 over zero-shot prompting.

% \textbf{When persona is used in input prompts, the EM and CodeBLEU that GPT-3.5 achieves decrease by at least 3.67\% and 1.33\%, respectively.}
\textbf{When a persona is included in input prompts, GPT-3.5 achieves 1.02\% - 54.17\% lower EM than when the persona is not included in input prompts.}
% We also observe from the table that GPT-3.5 and Magicoder achieves less EM and CodeBLEU when a persona is included in prompts.
Table~\ref{tab:result} also shows that in terms of EM, GPT-3.5 that zero-shot and few-shot learning with a persona are used achieves 3.67\% - 54.17\% and 1.02\% - 30.77\% lower than GPT-3.5 that zero-shot and few-shot learning without a persona are used, respectively.
In terms of CodeBLEU, GPT-3.5 that zero-shot and few-shot learning with a persona are used achieves 1.33\% - 19.13\% and 0.15\% - 0.90\% lower than GPT-3.5 that zero-shot and few-shot learning without a persona are used, respectively.


The results indicate that GPT-3.5 that zero-shot learning and few-shot learning with a persona are used achieves lower EM and CodeBLEU.
\revised{R2-2}{
To illustrate the impact of the persona, we present an example of the revised code that GPT-3.5 generates when zero-shot learning with and without a persona are used, and an example of the revised code that GPT-3.5 generates when few-shot learning with and without a persona are used in Figure~\ref{fig:RQ3-code-change-with-and-without-persona}.

Figure~\ref{fig:RQ3-0-shot-no-persona} presents the revised code that GPT-3.5 correctly generates when zero-shot learning without a persona is used.
In this figure, GPT-3.5 suggests an alternative way to initialize variable \texttt{logArg}.
In contrast, Figure~\ref{fig:RQ3-0-shot-with-persona} presents the revised code that GPT-3.5 incorrectly generates when zero-shot learning with a persona is used.
In this figure, GPT-3.5 suggests changing the variable type from \texttt{Boolean} to \texttt{boolean} and changing the variable name from \texttt{sample\_name} to \texttt{sampleName} in addition to suggesting an alternative way to initialize variable \texttt{logArg}.
% by suggesting the same change to \ChatGPTZeroShot~(without a persona) and additional cha\-nges (i.e., changing variable type from \texttt{Boolean} to \texttt{boolean} and changing variable name from \texttt{sample\_name} to \texttt{sampleName}).

Figure~\ref{fig:RQ3-few-shot-no-persona} presents another example of the revised code that GPT-3.5 correctly generates when few-shot learning without a persona is used.
In this figure, GPT-3.5 suggests a new \texttt{if} condition.
On the contrary, Figure~\ref{fig:RQ3-few-shot-with-persona} presents the revised code that GPT-3.5 incorrectly generates when few-shot learning with a persona is used.
In this figure, GPT-3.5 suggests an additional \texttt{if} statement and an additional \texttt{else} block.

The above examples imply that when a persona is included in prompts, GPT-3.5 tends to suggest additional incorrect changes to the submitted code compared to when a persona is not included in prompts.
}

% using persona in input prompts has a negative impact on the performance of GPT-3.5.


The above results indicate that the best prompting strategy when using GPT-3.5 without fine-tuning is few-shot learning without a persona.

==> section-exp-only/Result-old.tex <==
\section{Result} \label{sec:result}

In this section, we present the approach and the findings with respect to our three research questions.

\begin{table*}[ht]
  \centering
  \caption{(RQ1) \#perfect match of the existing code transformation approaches for the time-ignore and the time-wise evaluation scenarios.}
%   \chen{To small to see clearly, may use the abbreviation of ``beam size'', e.g., ``bs''}}
  \resizebox{\textwidth}{!}{
       \begin{tabular}{|c|c|ccc|ccc|ccc|}
\cline{3-11}    \multicolumn{1}{r}{} &       & \multicolumn{3}{c|}{Google} & \multicolumn{3}{c|}{Ovirt} & \multicolumn{3}{c|}{Android} \\
    \hline
    Approach & evaluation scenario & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} \\
    \hline
    \multirow{3}[2]{*}{TufanoT5} & time-ignore & 152   & 263   & 293   & 442   & 638   & 718   & 316   & 462   & 501 \\
          & time-wise & 16    & 98    & 125   & 5     & 46    & 58    & 1     & 15    & 28 \\
          & \% decrease & 89.47 & 62.74 & 57.34 & 98.87 & 92.79 & 91.92 & 99.68 & 96.75 & 94.41 \\
    \hline
    \multirow{3}[2]{*}{AutoTransform} & time-ignore & 114   & 208   & 233   & 578   & 794   & 854   & 344   & 489   & 516 \\
          & time-wise & 3     & 14    & 18    & 4     & 30    & 51    & 0     & 13    & 27 \\
          & \% decrease & 97.37 & 93.27 & 92.27 & 99.31 & 96.22 & 94.03 & 100   & 97.34 & 94.77 \\
    \hline
    \end{tabular}%
    }
  \label{tab:rq1-result}%
\end{table*}%


\begin{table*}[ht]
  \centering
  \caption{(RQ2) \#perfect match of our approach and the baseline (TufanoT5) for the time-wise evaluation scenario.}
  \resizebox{\textwidth}{!}{
        \begin{tabular}{|c|ccc|ccc|ccc|}
\cline{2-10}    \multicolumn{1}{r|}{} & \multicolumn{3}{c|}{Google} & \multicolumn{3}{c|}{Ovirt} & \multicolumn{3}{c|}{Android} \\
\hline
    Approach &\multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10}\\
    \hline
    TufanoT5 & 16    & 98    & 125   & 5     & 46    & 58    & 1     & 15    & 28 \\
    AutoTransform & 3 & 14 & 18 & 4 & 30 & 51 & 0 & 13 & 27 \\
    % Our approach & 90    & 174   & 214   & 50    & 194   & 245   & 10    & 65    & 107 \\
    Our approach & \textbf{74} & \textbf{165} & \textbf{202} & \textbf{48} & \textbf{187} & \textbf{238} & \textbf{12} & \textbf{70} & \textbf{101}\\
    % \% increase & 462.5 & 77.55 & 71.2  & 900   & 321.74 & 322.41 & 900   & 333.33 & 282.14 \\
    \hline
    \end{tabular}%
    }
  \label{tab:rq2-result}%
\end{table*}%


\noindent \textbf{(RQ1) \rqone}\\
\noindent \smallsection{Approach}
To answer this RQ, we focus on the time-ignore and the time-wise evaluation scenarios.
For the time-ignore evaluation scenario, the triplets in the dataset are randomly shuffled and then split to train/validation/test set by the proportion of 80\%/10\%/10\%, respectively. 
% \kla{how are these train/validation/test set splits? I can't find it.}
On the other hand, for the time-wise evaluation scenario, the triplets are first sorted in chronological order by the commit date of their corresponding patches.
Then, the triplets are split to train/validation/test set by the same proportion as the time-ignore evaluation scenario.
% Both types of evaluation scenarios are applied to both AutoTransform~\cite{AutoTransform} and TufanoT5~\cite{tufano2022using}.
In this RQ, we evaluate the following code transformation approaches: AutoTransform~\cite{AutoTransform} and TufanoT5.
AutoTransform leverages a Vanilla Transformer architecture~\cite{Vaswani2017} and Byte-Pair Encoding (BPE) subword tokenization~\cite{Sennrich2016}.
On the other hand, TufanoT5~\cite{tufano2022using} is a T5 model pre-trained on source code.

% \begin{itemize}
%     \item AutoTransform~\cite{AutoTransform}: AutoTransform leverages a Transformer model~\cite{Vaswani2017} and Byte-Pair Encoding (BPE) subword tokenization~\cite{Sennrich2016}.
    
%     \item TufanoT5~\cite{tufano2022using}: TufanoT5 is T5 model pre-trained on source code.
% \end{itemize}

% Therefore, we build AutoTransform~\cite{AutoTransform} and TufanoT5~\cite{tufano2022using} for both evaluation scenarios.
Therefore, we build both approaches for the time-ignore and the time-wise evaluation scenarios.
In total, we build 12 NMT models (i.e., 2 approaches $\times$ 2 evaluation scenarios $\times$ 3 datasets).
To select a model for evaluation, we choose the model that achieves the lowest loss on the validation set.
Finally, we measure \#perfect match (as explained in Section~\ref{sec:eval-measure}) on the test set.
In particular, we measure \#perfect match of the time-ignore scenario ($PM_{time-ignore}$) and the time-wise  scenario ($PM_{time-wise}$).
We also compute the percentage decrease of \#perfect match as follows: 
% \kla{PM is not defined?, you called \#perfect match, not PM in 4.2.4}

$$\frac{PM_{time-ignore} - PM_{time-wise}}{PM_{time-ignore}}\times100\%$$

% We also compute the percentage of perfect match as
% \changed{
% $$\frac{\text{\#correctly generated }   m_{app}}{\text{\#total }  m_{app}\text{ in test set}}\times100\%$$
% }
% \kla{bad formatting :(}
% \oat{I wrote like in AutoTransform paper to save space}

\noindent \smallsection{Result}
\textbf{When the existing code transformation approaches
% \kla{why only 2?, while the RQ said approaches - lack of consistency} 
% \kla{if said two, why AutoTransform is not introduced in the Background section --- right now, no one knows what is AutoTransform} 
are evaluated in the time-wise scenario, \#perfect match of these approaches decreases by at least 57\% (for TufanoT5) and 92\% (for AutoTransform).}
Table~\ref{tab:rq1-result} shows the results of \#perfect match of the existing code transformation approaches across the three datasets (i.e., Google, Ovirt and Android), based on the beam sizes of 1, 5 and 10.
The table shows that when the beam size is 1, \#perfect match of TufanoT5 drops by at least 89.97\% ($\frac{152-16}{152}$; for Google) and \#perfect match of AutoTransform drops by at least 97.37\% ($\frac{114-3}{114}$; for Google).
Even the beam size increases to 5 and 10,  \#perfect match of TufanoT5 drops by at least from 57.34\% ($\frac{293-125}{293}$; for Google at beam size of 10) to 62.74\% ($\frac{263-98}{263}$; for Google at beam size of 5) 
Likewise, \#perfect match of AutoTransform  drops by at least from 91.92\% ($\frac{718-58}{718}$; for Ovirt at beam size of 10) to 93.27\% ($\frac{208-14}{208}$; for Google at beam size of 5).
% The results imply that the existing code transformation approaches still do not perform well in time-wise evaluation scenario. 
The results imply that \#perfect match of the existing code transformation approaches dramatically decreases when being evaluated in the time-wise evaluation scenario. 
Thus, future work should consider the time-wise scenario when evaluating proposed approaches to ensure that they are applicable in the real practice.

% \kla{sure, but what does it mean to the community? - only implication but no suggestions. what do you suggest?} 
% Thus, there is still a room for improvement so that automated code review approaches can perform well in this scenario.



% \begin{table*}[htbp]
%   \centering
%   \caption{(RQ2) The perfect match of TufanoT5 and our approach}
%     \begin{tabular}{c|ccc|ccc|ccc}
%     \hline
%           & \multicolumn{3}{c|}{Android} & \multicolumn{3}{c|}{Google} & \multicolumn{3}{c}{Ovirt} \\
%     Approach & \multicolumn{1}{c}{beam size = 1} & \multicolumn{1}{c}{beam size = 5} & \multicolumn{1}{c|}{beam size = 10} & \multicolumn{1}{c}{beam size = 1} & \multicolumn{1}{c}{beam size = 5} & \multicolumn{1}{c|}{beam size = 10} & \multicolumn{1}{c}{beam size = 1} & \multicolumn{1}{c}{beam size = 5} & \multicolumn{1}{c}{beam size = 10} \\
%     \hline
%     TufanoT5 & 1 (0.05\%) & 15 (0.82\%) & 28 (1.53\%) & 16 (1.29\%) & 98 (7.92\%) & 125 (10.11\%) & 5 (0.19\%) & 46 (1.71\%) & 58 (2.16\%) \\
%     Our approach & \textbf{10 (0.54\%)} & \textbf{65 (3.54\%)} & \textbf{107 (5.83\%)} & \textbf{90 (7.28\%)} & \textbf{174 (14.07\%)} & \textbf{214 (17.30\%)} & \textbf{50 (1.86\%)} & \textbf{194 (7.21\%)} & \textbf{245 (9.11\%)} \\
%     \hline
%     \end{tabular}%
%   \label{tab:rq2-result}%
% \end{table*}%


% \noindent \textbf{(RQ2) \rqtwo}\\
% \noindent \smallsection{Approach}
% To answer this RQ, we evaluate how well our \AppName can transform \mInit to \mApproved compared to TufanoT5~\cite{tufano2022using}.
% To do so, we build model of TufanoT5 and \AppName for each studied dataset (the dataset is split time-wise).
% For each approach and for each dataset, we select
% the model that achieves the
% lowest loss computed based on the validation set.
% Then, we measure \#perfect match of TufanoT5 and \AppName on test data. 

\begin{table*}
  \centering
  \caption{(RQ3) \#perfect match of our approach and the CodeT5 model (here, the CodeT5 model is trained without code diff) for the time-wise evaluation scenario; the number in the parenthesis indicates the percentage change compared to our approach.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|}
\cline{2-10}    \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Google} & \multicolumn{3}{c|}{Ovirt} & \multicolumn{3}{c|}{Android} \\
    \hline
    Approach & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} \\
    \hline
    % CodeT5 (without code diff) & 5 (-94.44\%) & 71 (-59.2\%) & 111 (-48.13\%) & 14 (-72\%) & 128 (-34.02\%) & 189 (-22.86\%) & 0 (-100\%) & 52 (-20\%) & 86 (-19.63\%) \\
    % Our approach & 90    & 174   & 214   & 50    & 194   & 245   & 10    & 65    & 107 \\
     CodeT5 (without code diff) & 5 (-93.24\%) & 71 (-56.97\%) & 111 (-45.05\%) & 14 (-70.83\%) & 128 (-31.55\%) & 189 (-20.59\%) & 0 (-100\%) & 52 (-25.71\%) & 86 (-14.85\%)\\
    Our approach & 74 & 165 & 202 & 48 & 187 & 238 & 12 & 70 & 101\\
    \hline
    \end{tabular}%
    }
  \label{tab:rq3-1-result}%
\end{table*}


\begin{table*}
  \centering
%   \caption{(RQ3) The perfect match of our approach and the pre-trained PL model (here the pre-trained PL models are trained with code diff) for time-wise evaluation scenario; the number in the parenthesis indicates the percentage change compared to our approach}
    \caption{(RQ3) \#perfect match of our approach and the variants of our approach, where CodeT5 is changed to other pre-trained PL models or other code transformation approaches (trained with the code diff) for the time-wise evaluation scenario; the number in the parenthesis indicates the percentage change compared to our approach.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|}
\cline{2-10}    \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Google} & \multicolumn{3}{c|}{Ovirt} & \multicolumn{3}{c|}{Android} \\
    \hline
    Approach &\multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} & \multicolumn{1}{c}{$k$ = 1} & \multicolumn{1}{c}{$k$ = 5} & \multicolumn{1}{c|}{$k$ = 10} \\
    \hline
    CodeBERT & 48 (-35.14\%) & 76 (-53.94\%) & 78 (-61.39\%) & 15 (-68.75\%) & 49 (-73.8\%) & 64 (-73.11\%) & 1 (-91.67\%) & 10 (-85.71\%) & 18 (-82.18\%)\\
    GraphCodeBERT & 45 (-39.19\%) & 83 (-49.7\%) & 92 (-54.46\%) & 17 (-64.58\%) & 46 (-75.4\%) & 62 (-73.95\%) & 3 (-75\%) & 19 (-72.86\%) & 28 (-72.28\%)\\
    PLBART & 3 (-95.95\%) & 49 (-70.3\%) & 84 (-58.42\%) & 19 (-60.42\%) & 89 (-52.41\%) & 129 (-45.8\%) & 12 (-0\%) & 51 (-27.14\%) & 78 (-22.77\%)\\
    TufanoT5 & 16 (-78.38\%) & 88 (-46.67\%) & 122 (-39.6\%) & 16 (-66.67\%) & 85 (-54.55\%) & 113 (-52.52\%) & 2 (-83.33\%) & 33 (-52.86\%) & 55 (-45.54\%)\\
    AutoTransform & 13 (-82.43\%) & 38 (-76.97\%) & 50 (-75.25\%) & 26 (-45.83\%) & 64 (-65.78\%) & 92 (-61.34\%) & 3 (-75\%) & 33 (-52.86\%) & 46 (-54.46\%)\\
    Our approach & 74 & 165 & 202 & 48 & 187 & 238 & 12 & 70 & 101\\
    \hline
    \end{tabular}%
    }
  \label{tab:rq3-2-result}%
\end{table*}%

\noindent \textbf{(RQ2) \rqtwo}\\
\noindent \smallsection{Approach}
To answer this RQ, we build and evaluate our approach and the baselines (i.e., TufanoT5~\cite{tufano2022using} and AutoTransform~\cite{AutoTransform}) in the time-wise scenario.
We follow the steps in RQ1 to build and select the model for evaluation.
% The steps to build and select the model for our approach is similar to the steps in RQ1.
In this RQ, we evaluate our approach and the baselines by using \#perfect match like in RQ1.
However, we also compute the percentage increase of \#perfect match as

$$\frac{PM_{ours} - PM_{baseline}}{PM_{baseline}}\times100\%$$

where $PM_{ours}$ is \#perfect match of our approach, and $PM_{baseline}$ is \#perfect match of the baselines.

\noindent \smallsection{Result}
\textbf{Our \AppName can achieve \#perfect match at least 61.6\% higher than TufanoT5 and at least 274.07\% higher than AutoTransform.}
Table~\ref{tab:rq2-result} shows the results of \#perfect match of our \AppName and the baselines across three datasets (i.e., Google, Ovirt and Android), based on the beam sizes of 1, 5 and 10.
The table shows that for the beam size of 1, \AppName can achieve \#perfect match of 12 (Android) - 74 (Google), which is at least 362.5\% higher than TufanoT5 and 1200\% higher than AutoTransform.
On the other hand, for the beam size of 5, our \AppName can achieve \#perfect match of 70 (Android) - 187 (Ovirt), which is at least 68.37\% higher than TufanoT5 and 438.46\% higher than AutoTransform.
Likewise, we find that for the beam size of 10, our approach can achieve \#perfect match of 101 (Android) - 238 (Ovirt), which is at least 61.6\% higher than TufanoT5 and 274.07\% higher than AutoTransform.
%%% old one
% \textbf{Our \AppName can achieve perfect match higher than TufanoT5~\cite{tufano2022using} at least 462\%.}
% Table~\ref{tab:rq2-result} shows the results of \#perfect match of TufanoT5 and \AppName across three datasets (i.e., Google, Ovirt, Android), based on beam sizes of 1, 5 and 10.
% The table shows that for beam size of 1, \AppName can achieve 462.5\% ($\frac{90-16}{16}$; for Google) - 900\% ($\frac{50-5}{5}$; for Ovirt) higher perfect match than TufanoT5.
% On the other hand, \AppName can achieve 77.55\% ($\frac{174-98}{98}$; for Google) - 321.74\% ($\frac{194-46}{46}$; for Ovirt) and 71.20\% ($\frac{214-125}{125}$; for Google) - 322.41\% ($\frac{245-58}{58}$; for Ovirt) higher perfect match than TufanoT5 for beam size of 5 and 10, respectively.
The results indicate that the number of \mInit that our \AppName can correctly transform to \mApproved is substantially higher than the TufanoT5 and AutoTransform approaches.

% To investigate why our approach can achieve \#perfect match higher than the TufanoT5 approach, we manually analyze the kinds of \mInit that our approach and TufanoT5 can correctly transform to $m_{app}$.
% We find that in the majority cases, our approach can correctly remove newly added code tokens (as shown in the code diff) better than the TufanoT5 approach.
% In particular, our approach can correctly transform 101 methods (62 for Google, 33 for Ovirt, and 6 for Android) by removing the newly added code tokens.
% On the other hand, TufanoT5 can correctly transform 15 methods (13 for Google, 2 for Ovirt, and 0 for Android) by removing code the newly added tokens. \chen{Need double check}

\changed{
To investigate why our approach can achieve \#perfect match higher than the TufanoT5 approach, we manually analyze the \mApproved generated by our approach and the TufanoT5 approach ($k$ = 1). 
To do so, we observe the \mApproved that our approach can correctly generate while the TufanoT5 approach cannot.
We find that there are 65, 39, and 12 \mApproved of Google, Ovirt, and Android, respectively, that our approach can correctly generate while the TufanoT5 approach cannot.
The results suggest that the higher \#perfect match of our approach has to do with the code diff component and the NMT model (i.e., CodeT5~\cite{wang2021codet5}) of our approach.
}

% The higher \#perfect match of our approach has to do with the code diff information of \mInit that are modified from the codebase.
% The higher \#perfect match of our approach has to do with the code diff representation that is inserted to $m_{init}$.
% We find that our approach can correctly transform 102 $m_{init}$, which are modified from the codebase, having newly added code tokens revised in the approved version (62 for Google, 34 for Ovirt, and 6 for Android).


\noindent \textbf{(RQ3) \rqthree}\\
\noindent \smallsection{Approach}
To answer this RQ, we investigate the changes of \#perfect match when a component of our \AppName is varied.
In particular, we extend our experiment by removing the code diff component from our approach to examine the impact of the code diff component on our approach.
We also conduct experiment by changing CodeT5 to AutoTransform~\cite{AutoTransform}, TufanoT5~\cite{tufano2022using}, and the following pre-trained programming language models: CodeBERT~\cite{codebert}, GraphCodeBERT~\cite{guo2020graphcodebert} and PLBART~\cite{ahmad2021plbart}.
CodeBERT and GraphCodeBERT are the pre-trained encoder models based on BERT~\cite{devlin2018bert} architecture, while PLBART is the pre-trained encoder-decoder model  based on BART~\cite{lewis2020bart} architecture.
% while keeping the code diff, to observe the impact of the NMT model on \#perfect match of our approach.

% \begin{itemize}

%     \item \textbf{CodeBERT}~\cite{codebert}: 
%     CodeBERT is a transformer encoder based on BERT~\cite{devlin2018bert} architecture, which is pre-trained on the source code of six programming languages (including Java) and natural language that are obtained from Github.
    
%     \item \textbf{GraphCodeBERT}~\cite{guo2020graphcodebert}:
%     GraphCodeBERT has the same architecture as CodeBERT. However, GraphCodeBERT differs from CodeBERT by being pre-trained with data flow graph in addition to source code and natural language, and having a modified self-attention mechanism. 
    
%     \item \textbf{PLBART}~\cite{ahmad2021plbart}: 
%     PLBART is a transformer encoder-decoder based on BART~\cite{lewis2020bart} architecture, which is pre-trained on the source code of Java and Python obtained from Github, and natural language obtained from StackOverflow Dump.

% \end{itemize}

% In total, we build additional 18 models in this RQ (i.e., 2 existing code transformation approaches + 4 pre-trained programming language models for the 3 studied datasets).
Similar to RQ1 and RQ2, we evaluate our approach and the variation of our approach in the time-wise scenario.
Besides, we choose the model that achieves the lowest loss on the validation set, and measure \#perfect match on the test set.
In addition, we calculate the percentage change of \#perfect match as

$$\frac{PM_{varients} - PM_{ours}}{PM_{ours}}\times100\%$$

where $PM_{varients}$ is \#perfect match of the variation of our approach explained above, and $PM_{ours}$ is \#perfect match of our approach.


\noindent \smallsection{Result}
\textbf{When the code diff component is removed from our approach, \#perfect match of our approach decreases by at least 14.85\%.}
Table~\ref{tab:rq3-1-result} shows \#perfect match of our approach and the CodeT5~\cite{wang2021codet5} model across the three datasets (i.e., Google, Ovirt and Android), based on the beam sizes of 1, 5 and 10.
The table shows that when code diff component is removed, at beam size of 1, \#perfect match is decreased by 70.83\% ($\frac{14-48}{48}$; for Ovirt) - 100\% ($\frac{0-12}{12}$; for Android).
Similarly, for the beam size of 5 and 10, \#perfect match is decreased by 25.71\% ($\frac{52-70}{70}$; for Android) - 56.97\% ($\frac{71-165}{165}$; for Google) and 14.85\% ($\frac{86-101}{101}$; for Android) - 45.05\% ($\frac{111-202}{202}$; for Google), respectively.
The results indicate that the removal of the code diff component has a negative impact on the performance of our approach.

\textbf{When the pre-trained model of our approach is changed to the other pre-trained PL models,  \#perfect match decreases by at least 22.77\%.}
Table~\ref{tab:rq3-2-result} shows \#perfect match of our approach and the other pre-trained PL models  (here, the pre-trained PL models are trained with the code diff).
When the pre-trained PL model of our approach (i.e., CodeT5~\cite{wang2021codet5}) is changed to CodeBERT~\cite{codebert}, we find that \#perfect match decreases by at least 35.14\% ($\frac{48-74}{74}$; for Google), 53.94\% ($\frac{76-165}{165}$; for Google), and 61.39\% ($\frac{78-202}{202}$; for Google) for the beam size of 1, 5, and 10, respectively.
Similarly, when the CodeT5 is changed to GraphCodeBERT~\cite{guo2020graphcodebert}, we find that \#perfect match decreases by at least 39.19\% ($\frac{45-74}{74}$; for Google), 49.7\% ($\frac{83-165}{165}$; for Google), and 61.39\% ($\frac{78-202}{202}$; for Google) for beam size of 1, 5, and 10, respectively.
Lastly, when the CodeT5 is changed to PLBART~\cite{ahmad2021plbart}, we find that \#perfect match decreases by at least 60.42\% ($\frac{19-48}{48}$; for Ovirt), 27.14\% ($\frac{51-70}{70}$; for Android), and 22.77\% ($\frac{78-101}{101}$; for Android) for beam size of 1, 5, and 10, respectively.
% Even though we observe an increasing of \#perfect match by 20\% ($\frac{12-10}{10}$) in Ovirt dataset, \#perfect match most likely decreases when CodeT5 is changed to PLBART.
The results indicate that when the CodeT5 is changed to the other pre-trained PL models, the performance of our approach decreases.


\textbf{When the pre-trained PL model of our approach is changed to the existing code transformation approaches for code review (i.e., AutoTransform~\cite{AutoTransform} and TufanoT5~\cite{tufano2022using}), \#perfect match decreases by at least 56.92\% and 38.51\%, respectively.}
Table~\ref{tab:rq3-1-result} shows that when the pre-trained model of our approach (i.e., CodeT5~\cite{wang2021codet5}) is changed to TufanoT5, \#perfect match decreases by at least 66.67\% ($\frac{16-48}{48}$; for Ovirt), 46..67\% ($\frac{88-165}{165}$; for Google), and 39.6\% ($\frac{122-202}{202}$; for Google) for beam size of 1, 5, and 10, respectively.
The similar observation can be seen when the CodeT5 is changed to AutoTransform.
In particular, we find that \#perfect match decreases by at least 45.83\% ($\frac{26-48}{48}$; for Ovirt), 52.86\% ($\frac{33-70}{70}$; for Android), and 54.46\% ($\frac{46-101}{101}$; for Android) for the beam size of 1, 5, and 10, respectively.


% To answer this RQ, we build and evaluate the following pre-trained programming language models in time-wise scenario.


    
%     \item \textbf{CodeT5}~\cite{wang2021codet5}: 
%     CodeT5 is a transformer encoder-decoder based on T5 architecture~\cite{raffel2020exploring}, which is pre-trained on source code obtained from CodeSearchNet containing six programming languages (including Java) and natural language. CodeT5 is also pre-trained with identifier-aware pre-training tasks in addition to pre-training task for natural language (e.g., mask span prediction).



% In total, we build 12 models (i.e., 4 pre-trained models $\times$ 3 datasets).
% Similar to RQ1, for each model, we select the one that achieves the lowest loss computed based on the validation set.
% Then, we measure the perfect match of the pre-trained models and \AppName.

% \noindent \smallsection{Result}
% \textbf{Our approach can achieve perfect match higher than the existing pre-trained models at least 143\%.}
% Table~\ref{tab:rq3-result} shows perfect match of the pre-trained models and \AppName.
% From the table, when consider beam size of 1, our \AppName achieves at least 200\% ($\frac{90-30}{30}$; for Google), 143.24\% ($\frac{90-37}{37}$; for Google), 284.62\% ($\frac{50-13}{13}$; for Ovirt), and 257.14\% ($\frac{50-14}{14}$; for Ovirt) higher perfect match when compared to CodeBERT, GraphCodeBERT, PLBART and CodeT5, respectively.
% When beam size is increased to 5, our approach achieves 25\% ($\frac{65-52}{52}$; for Android when compared to CodeT5) - 2,325\% ($\frac{194-8}{8}$; for Ovirt when compared to CodeBERT).
% Similarly, for beam size of 10, our approach achieves 24.42\% ($\frac{107-86}{86}$; for Android when compared to CodeT5) - 2,622.22\% ($\frac{245-9}{9}$; for Ovirt when compared to CodeBERT).
% The results imply that \AppName can more accurately transform \mInit to \mApproved than the pre-trained models.



==> section-exp-only/Study-design-old.tex <==


\begin{table*}
  \centering
  % \caption{An overview statistic of the studied datasets (the Android, Google and Ovirt projects are obtained from~\cite{pornprasit2023d}).}
  \caption{A statistic of the studied datasets (the dataset of Android, Google and Ovirt are from \DACTData~\cite{pornprasit2023d}).}
%   \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
\hline   Dataset  & \# Train & \# Validation & \# Test & \# Language & Granularity & Has Comment\\
    \hline
    % \CodeReviewerDataNew~\cite{guo2023exploring} & - & - & 14,945\footnote{The number is from the dataset provided in replication package} \\
    \CodeReviewerData~\cite{li2022automating} & 150,405 & 13,102 & 13,104 & 9 & Diff Hunk & Yes\\
    \tufanoData~\cite{tufano2022using} & 134,238 & 16,779 & 16,779 & 1 & Function & Yes/No\\
    Android~\cite{pornprasit2023d} & 14,690 & 1,836 & 1,835 & 1 & Function & No\\
    Google~\cite{pornprasit2023d} & 9,899 & 1,237 & 1,235 & 1 & Function & No\\
    Ovirt~\cite{pornprasit2023d}  & 21,509 & 2,686 & 2,688 & 1 & Function & No\\
    % Gerrit & 3,144 & 544 & 370 \\
    \hline
    \end{tabular}%
    % }
  \label{tab:dataset}%
\end{table*}%



\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/new-overall-study-3.pdf}
    % \caption{An overview of our study design. \kla{consistency!!!!! study design or experimental design?}}
    \caption{An overview of our experimental design.}
    \label{fig:study-design}
\end{figure*}


% \begin{figure}
%      \centering
%      \begin{subfigure}[]{\columnwidth}
%         \centering
%         \includegraphics[trim = {0 3cm 0 0}, clip,width=\columnwidth]{figure/overview-study-zero-shot.pdf}
%          \caption{zero-shot learning approach}
%          \label{fig:zero-shot-app}
%      \end{subfigure}
%      \par\bigskip 
%      \begin{subfigure}[]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figure/overview-study-few-shot.pdf}
%      %     % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{few-shot learning approach}
%          \label{fig:few-shot-app}
%      \end{subfigure}
%      \par\bigskip 
%      \begin{subfigure}[]{\columnwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figure/overview-study-fine-tune.pdf}
%          % \includegraphics[width=\textwidth]{figure/TufanoT5-paper_Code_Refinement_output_len_count.pdf}
%          \caption{GPT-3.5 fine-tuning}
%          \label{fig:fine-tune-app}
%      \end{subfigure}
     
%     \caption{Overview of our study design}
%     \label{fig:study-design}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figure/overview-study-new.pdf}
%     \caption{An overview of our study}
%     \label{fig:overview-study}
% \end{figure}

\begin{figure}[!h]
    \centering
    \begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page = 1, trim = {0 3cm 0 0}, clip]{figure/0-shot-prompt-templates_new.pdf}
         \caption{A prompt template for zero-shot learning (when a reviewer comment is available).}
         \label{fig:zero-shot prompt with comment}
     \end{subfigure}
    \par\bigskip
    \begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page = 2, trim = {0 4cm 0 0}, clip]{figure/0-shot-prompt-templates_new.pdf}
         \caption{A prompt template for zero-shot learning (when a reviewer comment is not available).}
         \label{fig:zero-shot prompt without comment}
     \end{subfigure}
     \par\bigskip
     \begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page = 1, trim = {0 3cm 0 0}, clip]{figure/few-shot-prompt-templates_new.pdf}
         \caption{A prompt template for few-shot learning (when a reviewer comment is available).}
         \label{fig:few-shot prompt with comment}
     \end{subfigure}
     \par\bigskip 
     \begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, page = 2, trim = {0 5cm 0 0}, clip]{figure/few-shot-prompt-templates_new.pdf}
         \caption{A prompt template for few-shot learning (when a reviewer comment is not available).}
         \label{fig:few-shot prompt without comment}
     \end{subfigure}

    \caption{Prompt templates for performing zero-shot learning and few-shot learning with GPT-3.5 and Magicoder (\textit{lang} refers to a programming language).}
    \label{fig:prompt-templates}
\end{figure}

% \kla{the paper does not have any motivation, no research questions formulation, no goal....}


% \section{Research Methodology} \label{sec:study-design}

% Table generated by Excel2LaTeX from sheet 'exp setting'
\begin{table}[htbp]
  \centering
  \caption{Experiment settings in our study.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|}
    \hline
    {\multirow{2}{*}{ \makecell{Experimental\\setting}}} & \multirow{2}{*}{Fine-Tuned?} & \multirow{2}{*}{Prompting} & \multirow{2}{*}{\makecell{Use persona?}} \\
          &       &       &  \\
    \hline
    Setting \#1 & yes   & \multirow{4}{*}{0-shot} & no \\
\cline{1-2}\cline{4-4}    Setting \#2 & yes   &       & yes \\
\cline{1-2}\cline{4-4}    Setting \#3 & no    &       & no \\
\cline{1-2}\cline{4-4}    Setting \#4 & no    &       & yes \\
    \hline
    Setting \#5 & no    & \multirow{2}{*}{few-shot} & no \\
\cline{1-2}\cline{4-4}    Setting \#6 & no    &       & yes \\
    \hline
    \end{tabular}%
  }
  \label{tab:exp-setting}%
\end{table}%


\section{Experimental Design} \label{sec:study-design}


%% will check after finishing the whole section

% In this section, we provide the motivation of our research questions; and describe our overview of our study design, prompt design, zero-shot learning, few-shot learning and fine-tuning GPT-3.5.

% In this section, we provide the motivation \kla{need to update} of our research questions and describe our study design.

In this section, we provide an overview and details of our experimental design.

% In this section, we explain the overview of our study design, the prompt design, zero-shot learning, few-shot learning and model fine-tuning.\kla{to revise}

% \subsection{Goals and Research Questions}

% The goal of this paper is to investigate which LLMs perform best based on two contexts, i.e., when a code review dataset is (and is not) available for model fine-tuning.
% To achieve this goal, we present the motivation and formulate the following research questions.

% \kla{can you give me a quick motivation / keypoints for our research questions?}


% \begin{enumerate}[]
%     \item \textbf{RQ1: \rqone}\\
%     % \kla{what is the motivation?}
%     \textbf{Motivation.}
%     % Recent studies proposed several LLMs for code review automation~\cite{pornprasit2023d, li2022automating, tufano2022using}.
%     Recently, Guo~\ea~\cite{guo2023exploring} conducted an empirical study of GPT-3.5 for code review automation.
%     However, their study is not comprehensive, as explained in Section~\ref{sec:background}.
%     Therefore, little is known about which LLM is the most effective for code review automation.
%     % In particular, they evaluate GPT-3.5 that uses zero-shot prompting against an LLM for code review automation called CodeReviewer~\cite{li2022automating}.
%     % However, their study still lacks the evaluation of GPT-3.5 with other LLMs for code review automation~\cite{pornprasit2023d, tufano2022using}.
%     % In addition, their study did not investigate the 
%     % performance of GPT-3.5 when being fine-tuned or using other prompting techniques (i.e., few-shot learning).
%     % \revised{explain problem here}{...}
%     % \revised{I explained problem of the gap here}{Thus, little is known about which LLMs for code review automation can achieve the highest performance.}
%     Thus, in this RQ, we empirically evaluate the performance of GPT-3.5 and Magicoder (when not being fine-tuned and fine-tuned) against the existing code review automation approaches~\cite{pornprasit2023d, tufano2022using, li2022automating} to find which approach performs best.
%     % Thus, little is known about which LLMs perform best for code review automation.
%     % \textit{(Oat) continue from here}
%     % For example, Pornprasit~\ea~\cite{pornprasit2023d} proposed D-ACT, which leverages CodeT5~\ea~\cite{wang2021codet5} and code difference. Tufano et al.~\ea~\cite{tufano2022using} presented a pre-trained T5 model~\ea~\cite{raffel2020exploring} to address the limitations in the previous work~\cite{tufano2021towards} (we will call this model TufanoT5 henceforth). Similarly, Li~\ea~\cite{li2022automating} proposed CodeReviewer, a pre-trained model that is based on the CodeT5 [48] model.
%     % However, there is a lack of a systematic evaluation of the above code review automation approaches and GPT-3.5.
%     % Thus, little is know about 
%     % However, little is known about the capabilities of GPT-3.5 when compared to the above code review automation approaches.
    
%     % While previous work showed that GPT-3.5 outperforms the existing approaches for different software engineering tasks~\cite{eliseeva2023commit, schafer2023empirical}, little is known about the capabilities of GPT-3.5 when compared to the above code review automation approaches.
%     % \kla{do you mean they don't compare with the existing one? That's even weird. I don't think so.}
    
%     % \textit{(Oat): I mean recent work compare GPT-3.5 on different SE tasks, but still lack comparison between GPT-3.5 and other code review automation approaches.}
    
%     \item \textbf{RQ2: \rqtwo}\\
%     % \kla{what is the motivation?}
%     \textbf{Motivation.}
%     % Prior work~\cite{chowdhery2023palm, wei2021finetuned} found that model fine-tuning can increase the performance of LLMs over LLMs that are not fine-tuned on natural language processing tasks.
%     % However, fine-tuning LLMs requires more resources (e.g., time and budget) than using LLMs without fine-tuning.
%     Fine-tuning LLMs requires more resources (e.g., time and budget) than using LLMs without fine-tuning.
%     Thus, little is known whether it is worth investing in fine-tuning LLMs for code review automation.
%     Therefore, in this RQ, we evaluate the performance of fine-tuned LLMs and LLMs that are not fine-tuned.
    
%     % Prior work~\cite{chowdhery2023palm, wei2021finetuned, chen2021evaluating} conducted empirical studies of fine-tuning LLMs on downstream tasks. 
%     % For example, Chen~\ea~\cite{chen2021evaluating} conducted an experimental study of an LLM (i.e., GPT-3) fine-tuned on source code. 
%     % However, little is known about the benefit of fine-tuning GPT-3.5 for code review automation.
%     % whether model fine-tuning could help GPT-3.5 to achieve higher performance for code review automation.
    
%     \item \textbf{RQ3: \rqthree}\\
%     % \kla{what is the motivation?}
%     \textbf{Motivation.}
%     It is possible that model fine-tuning is infeasible due to a lack of a code review dataset or budget.
%     Thus, prompting techniques can be considered as an alternative to using LLMs for code review automation.
%     However, it is still unknown which prompting strategy (i.e., zero-shot learning, few-shot learning, or persona) is the most effective for code review automation.
%     Therefore, in this RQ, we evaluate the performance of LLMs when using different prompting strategies.

    
% \end{enumerate}


% \subsection{Overview}

% Figure~\ref{fig:overview-study} shows an overview of our study.
% In this study, we use \ChatGPTGuo~and \ChatGPTFewShot~to generate the revised code from a given submitted code.
% To use \ChatGPTGuo, we adapt the best prompt and temperature value presented by Guo~\ea~\cite{guo2023exploring} to testing samples.
% For \ChatGPTFewShot, we first select examples of each testing sample from the training set, using the BM25~\cite{robertson2009probabilistic} technique.
% Then, we adapt the prompt of \ChatGPTGuo~to the testing samples and the obtained examples to generate revised code.


% In this study, we do zero-shot learning and few-shot learning with \GPT-3.5.
% To do zero-shot learning, we use the prompt proposed by Guo~\ea~\cite{guo2023exploring} with testing set to generate revised code from \GPT-3.5.
% For the few-shot learning, we first select examples of each testing sample from the training set, using the BM25~\cite{robertson2009probabilistic} technique.
% Then, we use the prompt proposed by Guo~\ea~\cite{guo2023exploring} with testing set and add the obtained examples to generate revised code from \GPT-3.5.


% \subsection{Research Questions}

% In this work we aim to investigate the impact of provided examples, persona prompt, and model fine-tuning for code review automation.
% We conduct experiments to answer the
% following questions:

% \textbf{(RQ1) \rqone}

% \textbf{(RQ2) \rqtwo}

% \textbf{(RQ3) \rqthree}

% \textbf{(RQ4) \rqfour}



% \subsection{Experimental Design}-

\subsection{Overview}
% \kla{the goal of this work is to investigate which fried rice are more delicious so I taste 10 fried rice. do you get what I'm doing? will anyone/readers what I'm doing? can they reproduce the paper?}
% The goal of this work is to investigate which LLMs perform best based on two contexts, i.e., when a code review dataset is (and is not) available for model fine-tuning.
The goal of this work is to investigate which LLMs perform best when using model fine-tuning and inference techniques (i.e., zero-shot learning, few-shot learning, and persona).
To achieve this goal, we conduct experiments with two LLMs (i.e., GPT-3.5 and Magicoder~\cite{wei2023magicoder}) under six experimental settings as presented in Table~\ref{tab:exp-setting}, which accounts for 2 $\times$ 6 = 12 experiments in total.
We conduct the above experiments on the following datasets that are widely studied in the code review automation literature~\cite{llamareviewer, zhou2023generation, guo2023exploring, pornprasit2023d}: \CodeReviewerData~\cite{li2022automating}, \tufanoData~\cite{tufano2022using} and \DACTData~\cite{pornprasit2023d}.
% To achieve this goal, we conduct 45 experiments \kla{what is the definition of experiment here?} \kla{how do you come up with the 45? we need a detail here.} in total on the three studied code review datasets \kla{why three? what are they. why we need more datasets?}.
We explain the overview of our experimental design below.
% (2 LLMs $\times$ 6 settings (i.e., model fine-tuning and two prompting techniques) $+$ 3 code review automation approaches on the three studied code review datasets).


Figure~\ref{fig:study-design} provides an overview of our experimental design.
Each studied dataset is divided into a training set (containing submitted code as input and improved code as output) and a testing set (containing only submitted code).
The training set is used to select training examples for model fine-tuning and select demonstration examples for few-shot learning.
On the other hand, the testing set is used to select demonstration examples for few-shot learning, and is used for model fine-tuning and prompting.
%% may not need
% In this study, we conduct experiments with the following LLMs: GPT-3.5 and Magicoder~\cite{wei2023magicoder}, a state-of-the-art instruction-tuned model.
% We choose GPT-3.5 since prior work~\cite{guo2023exploring} showed that GPT-3.5 is capable for code review automation task.
% \revised{R2-4}{
% On the other hand, we choose Magicoder~\cite{wei2023magicoder} in our experiment since it outperforms other recent open-source instruction-tuned LLMs (e.g., Starcoder~\cite{li2023starcoder}, Deep\-Seek-Coder~\cite{guo2024deepseek} or CodeLLaMa~\cite{roziere2023codeLLaMa}).
% }
% We explain the study design for zero-shot learning, few-shot learning, and model fine-tuning below.
% We explain our prompt design; example selection for few-shot learning and model fine-tuning; prompting; and model fine-tuning below.
% We explain the details of our datasets, experimental design and evaluation measures below.
We explain the details of our datasets, model fine-tuning, prompting techniques, and evaluation measures below.

\subsection{Studied Datasets}

% We explain the details of the studied datasets below 
% \kla{why these datasets are chosen? what are the reasons? why not only one or two, why three and not four? we need REASONS!!!!! (I emphasized this million times. the Section 3 title called Experimental DESIGN, not experimental DESCRIPTION. Please justify your design, not just describe what you do.)}


%% my old idea, may not ok
% Recently, different datasets were released in the code review automation literature~\cite{tufano2019learning, tufano2021towards, tufano2022using, li2022automating, pornprasit2023d}.
% Thus, we choose the following datasets that are released in the latest conferences
In this study, we use the Code\-Reviewer\textsubscript{Data}~\cite{li2022automating}, Tu\-fano\textsubscript{Data}~\cite{tufano2022using} and \DACTData~\cite{pornprasit2023d} datasets since that are used in the experiments of the recently proposed code review automation approaches (i.e., CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, and D-ACT~\cite{pornprasit2023d}).
The details of the studied datasets are as follows (the statistic of the studied datasets is presented in Table~\ref{tab:dataset}).

\begin{itemize}
        % \item Guo~\ea's dataset (should we include it?)
        
        \item \textbf{\CodeReviewerData}: Li~\ea~\cite{li2022automating} collected this dataset from the GitHub projects across nine programming languages (i.e., C, C++, C\#, Java, Python, Ruby, php, Go, and Javascript).
    % that contain at least 1,500 pull requests.
    % The dataset contains the following information.
        The dataset contains triplets of the current version of code (diff hunk granularity), the reviewers' comment, and the revised version of code (diff hunk granularity).
        
        \item \textbf{\tufanoData}: Tufano~\ea~\cite{tufano2022using} collected this dataset from Java projects in GitHub containing at least 50 pull requests, and 6,388 Java projects hosted in Gerrit.
        Each record in the dataset contains a triplet of code submitted for review (function granularity), a reviewer's comment, and code after being revised (function granularity).
        Tufano~\ea~\cite{tufano2022using} created two types of this dataset (i.e., Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment)).
        
        \item  \textbf{\DACTData}: Pornprasit~\ea~\cite{pornprasit2023d} collected this dataset from the three Java projects hosted on Gerrit (i.e., Android, Google and Ovirt).
        Each record in the dataset contains a triplet of codebase (function granularity), code of the first version of a patch (function granularity), and code of the approved version of a patch (function granularity).
    \end{itemize}


% \kla{the paragraph below is not well structured in the right order. Prompt is mentioned in many sections, for crossing purposes, and lacks of high level structure. you basically explain each box, but not the flow of the experiment.}

% \smallsection{Studied Dataset}
%     In this study, we use the following datasets which are summarized in Table~\ref{tab:dataset}: \tufanoData~\cite{tufano2022using}, \DACTData~\cite{pornprasit2023d} and Code\-Reviewer\textsubscript{data}~\cite{li2022automating}.
%     % \CodeReviewerData~\cite{li2022automating}.
%     We describe the details of these datasets below.

    %  \textbf{\CodeReviewerDataNew}: Guo~\ea~\cite{guo2023exploring} collected the dataset from GitHub pull requests that appear after January 1, 2022.
    % The pull requests are obtained from the repositories in \CodeReviewerData~dataset and new repositories that have different programming languages (e.g., SQL and Perl) with the repositories in  \CodeReviewerData~dataset

    % \begin{itemize}
    %     \item Guo~\ea's dataset (???)
        
    %     \item \textbf{\CodeReviewerData}: Li~\ea~\cite{li2022automating} collected this dataset from the GitHub projects across nine programming languages (i.e., C, C++, C\#, Java, Python, Ruby, php, Go, and Javascript).
    % % that contain at least 1,500 pull requests.
    % % The dataset contains the following information.
    %     The dataset contains triplets of the current version of code (diff hunk granularity), the reviewers' comment, and the revised version of code (diff hunk granularity).
        
    %     \item \textbf{\tufanoData}: Tufano~\ea~\cite{tufano2022using} collected this dataset from Java projects in GitHub containing at least 50 pull requests, and 6,388 Java projects hosted in Gerrit.
    %     Each record in the dataset contains a triplet of code submitted for review (function granularity), a reviewer's comment, and code after being revised (function granularity).
    %     Tufano~\ea~\cite{tufano2022using} created two types of this dataset (i.e., Tufano\textsubscript{data} (with comment) and \tufanoData~(without comment)).
        
    %     \item  \textbf{\DACTData}: Pornprasit~\ea~\cite{pornprasit2023d} collected this dataset from the three Java projects hosted on Gerrit (i.e., Android, Google and Ovirt).
    %     Each record in the dataset contains a triplet of codebase (function granularity), code of the first version of a patch (function granularity), and code of the approved version of a patch (function granularity).
    % \end{itemize}

% we present the motivation and formulate the following research questions.




% \subsection{The Selection of Training Examples}
% \kla{grammar issues again?}
% \kla{is this training example for the whole experiment? why they have to be selected? I don't get it.}

% As suggested by OpenAI, a few training examples should be used to fine-tune GPT-3.5 to see if the performance improves. 
% Thus, we randomly select a set of examples from a whole training set by using the \texttt{random} function in python.
% We do so to reduce bias in the data selection.
% However, there is no rule or theory to determine the number of examples that should be selected from a training set.
% Thus, we use the trial-and-error approach to determine the suitable number of training examples.
% To do so, we start by using approximately 6\% training examples from a whole training set to fine-tune GPT-3.5.
% We find that GPT-3.5 that is fine-tuned with such training examples outperforms the existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d}.
% Therefore, based on the above finding, we use 6\% training examples for the whole experiment

% In this study, we randomly select approximately 6\% training examples from a whole training set since we found that LLMs that are fine-tuned with such training examples can outperform the existing code review automation approaches.
% To do so, we randomly \kla{why random?} select approximately 6\% of total input/output pairs \kla{what is the input/output pair? have you defined/} from the training dataset. \kla{why 6? you never justify it.}


% \kla{how can you ensure that your selection is not biased? would the results be impacted if other selection approaches were chosen?}

% \kla{one paragraph cannot be that short, Oat! this is not a sound research, lacking a proper justification, rationale, and systematic thinking.}


\subsection{Model Fine-Tuning}
% Model fine-tuning is further training pre-trained LLMs on domain-specific tasks so that LLMs can adapt to new tasks that it never learn during the pre-training phase.
% We explain the steps to fine-tune GPT-3.5 and Magicoder below.
% \kla{you never introduce which LLMs are you referring too?}

After an LLM is pre-trained, it can be fine-tuned to adapt to downstream tasks that it never learned in the pre-training phase.
To do so, as suggested by OpenAI, we first select a few training examples to fine-tune an LLM to see if the performance improves.
% As suggested by OpenAI, a few training examples should be used to fine-tune GPT-3.5 to see if the performance improves. 
Thus, we randomly select a set of examples from a whole training set by using the \texttt{random} function in Python to reduce bias in the data selection.
However, there is no rule or theory to determine the number of examples that should be selected from a training set.
Thus, we use the trial-and-error approach to determine the suitable number of training examples.
To do so, we start by using approximately 6\% training examples from a whole training set to fine-tune GPT-3.5.
We find that GPT-3.5 that is fine-tuned with such training examples outperforms the existing code review automation approaches~\cite{tufano2022using, li2022automating, pornprasit2023d}.
Therefore, based on the above finding, we use 6\% training examples for the whole experiment

% To fine-tune GPT-3.5, 
After that we use the selected training examples to fine-tune the studied LLMs.
In particular, we fine-tune GPT-3.5 by using the API provided by OpenAI\footnote{https://platform.openai.com/docs/guides/fine-tuning/create-a-fine-tuned-model}.
% After the training process is done, we use the fine-tuned GPT-3.5 to generate the improved code from a given submitted code and a reviewer comment (if available).
On the other hand, to fine-tune Magicoder~\cite{wei2023magicoder}, we leverage the state-of-the-art parameter-efficient fine-tuning technique called DoRA~\cite{liu2024dora}.
% recently proposed parameter-efficient fine-tuning technique called DoRA~\cite{liu2024dora}.
% We use this technique since it outperforms the LoRA technique.~\cite{hu2021lora}


% \subsection{The Selection of Demonstration Example}
% Demonstration examples are crucial components for few-shot prompting since they can affect the performance of LLMs~\cite{gao2023constructing}.
% % \kla{how crucial? why? what are they? This sentence just say "examples are crucial" but no further information or knowledge that other people can learn.}
% To select demonstration examples, we use BM25~\cite{robertson2009probabilistic} since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches for software engineering tasks.
% In this work, we use BM25~\cite{robertson2009probabilistic} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to obtain three demonstration examples from a training set, where each example consists of an input (i.e., submitted code) and output (i.e., improved code).
% \kla{why this?} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to obtain three example pairs of input and output from the training set. %, where 
% Each example pair \kla{the definition of input/output pair has never been formally introduced.} consists of submitted code and improved code.
% We use BM25~\cite{robertson2009probabilistic} since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches.\kla{in what context? for information retrieval? for software engineering? for search engine? }




\subsection{Prompting Techniques}
% \kla{I don't get why it is here as well. Have you mentioned some where earlier that you are going to focus on the three prompts? and WHY? } \kla{is this section the right order/position?}
% Prompting is the approach to leverage LLMs without fine-tuning.
% Prompting can be consider when resources (e.g., budgets) required for using LLMs are limited.

In this work, we conduct experiments with the following prompting techniques: zero-shot learning and few-shot learning.
We explain each prompting technique below.

% Zero-shot learning is the prompting technique that involves prompting LLMs to generate an output from a given instruction and an input.
% This prompting technique can be considered when only an instruction and an input (i.e., code submitted for review with a reviewer comment) are available.
% For this prompting technique, 
For \textit{zero-shot learning}, we first design the prompt templates as presented in Figure~\ref{fig:zero-shot prompt with comment} and Figure~\ref{fig:zero-shot prompt without comment} by following the guidelines from OpenAI\footnote{https://help.openai.com/en/articles/6654000-best-practices-for-prompt-engineering-with-openai-api}\footnote{https://platform.openai.com/docs/guides/prompt-engineering/strategy-write-clear-instructions} to ensure that the structure of the prompt is suitable for GPT-3.5.
The prompt templates consist of the following components: a perso\-na~\cite{white2023prompt}, instruction and input (i.e., submitted code).
The input also includes a reviewer comment if available.
We include a persona in the prompt templates to instruct GPT-3.5 to act as a software developer.
We do so to ensure that the improved code generated by GPT-3.5 looks like the source code written by a software developer.

Then, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt with comment} and the code submitted for review with a reviewer comment in the testing set.
However, in case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt without comment} and the code submitted for review instead.
Finally, we use LLMs to generate improved code from the constructed prompts.
We use the subscript \textit{Zero-shot} to denote LLMs with this prompting technique.


% construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt with comment} and the code submitted for review with a reviewer comment in the testing set.
% However, in case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt without comment} and the code submitted for review instead.
% Finally, we use LLMs to generate improved code from the constructed prompts.
% We use the subscript \textit{Zero-shot} to denote LLMs with this prompting technique.

% Few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} is the prompting technique that involves prompting LLMs to generate an output from a given instruction, demonstration examples and an actual input.
% The benefit of this prompting technique over zero-shot learning is that this prompting technique can help LLMs adapt to domain-specific tasks without model fine-tuning.
% For this prompting technique,  
For \textit{few-shot learning}~\cite{brown2020language, liu2021makes, wei2023larger}, we first design the prompt templates as presented in Figure~\ref{fig:few-shot prompt with comment} and Figure~\ref{fig:few-shot prompt without comment}.\footnote{Similar to zero-shot learning, we follow the guidelines from OpenAI.}
The prompt templates consist of components similar to the ones in the prompt template for zero-shot learning, and demonstration examples.

% \kla{how crucial? why? what are they? This sentence just say "examples are crucial" but no further information or knowledge that other people can learn.}
In few-shot learning, demonstration examples are crucial components for few-shot prompting since they can affect the performance of LLMs~\cite{gao2023constructing}.
Thus, we select demonstration examples by using BM25~\cite{robertson2009probabilistic} since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches for software engineering tasks.
In this work, we use BM25~\cite{robertson2009probabilistic} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to obtain three demonstration examples from a training set, where each example consists of an input (i.e., submitted code) and output (i.e., improved code).


Then, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt with comment}, the code submitted for review and reviewer comment in the testing set, and its corresponding selected examples.
In case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt without comment}, the code submitted for review in the testing set, and its corresponding selected examples instead.
Finally, we use LLMs to generate improved code from the constructed prompts.
We use the subscript \textit{Few-shot} to denote LLMs with this prompting technique.


% \smallsection{Zero-Shot Learning}
% Zero-shot learning is the prompting technique that involves prompting LLMs to generate an output from a given instruction and an input.
% Zero-shot learning can be considered when only an instruction and an input (i.e., code submitted for review with a reviewer comment) are available.
% For this prompting technique, we perform the following steps.

% First, we design the prompt templates as presented in Figure~\ref{fig:zero-shot prompt with comment} and Figure~\ref{fig:zero-shot prompt without comment} by following the guidelines from OpenAI\footnote{https://help.openai.com/en/articles/6654000-best-practices-for-prompt-engineering-with-openai-api}\footnote{https://platform.openai.com/docs/guides/prompt-engineering/strategy-write-clear-instructions} to ensure that the structure of the prompt is suitable for GPT-3.5.
% The prompt templates consist of the following components: a perso\-na~\cite{white2023prompt}, instruction and input (i.e., submitted code).
% The input also includes a reviewer comment if available.
% We include a persona in the prompt templates to instruct GPT-3.5 to act as a software developer.
% We do so to ensure that the improved code generated by GPT-3.5 looks like the source code written by a software developer.

% Then, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt with comment} and the code submitted for review with a reviewer comment in the testing set.
% However, in case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt without comment} and the code submitted for review instead.
% Finally, we use LLMs to generate improved code from the constructed prompts.


% \smallsection{Few-Shot Learning}
% Few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} is the prompting technique that involves prompting LLMs to generate an output from a given instruction, demonstration examples and an actual input.
% The benefit of this prompting technique over zero-shot learning is that this prompting technique can help LLMs adapt to domain-specific tasks without model fine-tuning.
% For this prompting technique, we perform the following steps.

% First, we use BM25~\cite{robertson2009probabilistic} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package to obtain three example pairs of input and output from the training set, where each example pair consists of submitted code and improved code.
% We do so since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches.

% Then, we design the prompt templates as presented in Figure~\ref{fig:few-shot prompt with comment} and Figure~\ref{fig:few-shot prompt without comment}.\footnote{Similar to zero-shot learning, we follow the guidelines from OpenAI.}
% The prompt templates consist of components similar to the ones in the prompt template for zero-shot learning, and example pairs.
% Then, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt with comment}, the code submitted for review and reviewer comment in the testing set, and its corresponding selected examples.
% In case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt without comment}, the code submitted for review in the testing set, and its corresponding selected examples instead.
% Finally, we use LLMs to generate improved code from the constructed prompts.

% \smallsection{Model Fine-Tuning}
% Model fine-tuning refers to further training pre-trained LLMs on domain-specific tasks so that LLMs can adapt to new tasks that it never learn during the pre-training phase.
% Since the approach to fine-tune GPT-3.5 and Magicoder is different, we explain the steps to fine-tune each of them below.

% To fine-tune GPT-3.5, we first randomly select approximately 6\% of total input/output pairs from the training dataset.
% % We do not use the whole training set to fine-tune GPT-3.5 since it is prohibitively expensive.
% Then, we use the selected training examples to fine-tune GPT-3.5 by using the API provided by OpenAI\footnote{https://platform.openai.com/docs/guides/fine-tuning/create-a-fine-tuned-model}.
% After that, we use the fine-tuned GPT-3.5 to generate the improved code from a given submitted code and a reviewer comment (if available).


% To fine-tune Magicoder, we leverage the recently proposed parameter-efficient fine-tuning technique called DoRA~\cite{liu2024dora}.
% We use this technique since it outperforms the LoRA technique.~\cite{hu2021lora}
% % The hyper-parameter settings of DoRA can be found in the supplementary material.


\subsection{Evaluation Measures}
% \kla{what is this evaluation? are you talking about "Evaluation Measures" or just "Evaluation" Evaluation of what?}
We use the following measures to evaluate the performance of the LLMs (i.e., GPT-3.5 and Magicoder~\cite{wei2023magicoder}) and code review automation approaches (i.e., CodeReviewer~\cite{li2022automating}, TufanoT5~\cite{tufano2022using}, and D-ACT~\cite{pornprasit2023d}) in our study.
% \kla{what LLMs? do you mean you evaluate GPT-4 or CodeLlama?}  \kla{what approaches?}.
% in our experiment:

    \begin{enumerate}
        % \item \textbf{Exact Match (EM)}~\cite{tufano2019learning, pornprasit2023d} is the number of generated code that is exactly the same as the actual code (i.e., the code in ground-truth).
        \item \textbf{Exact Match (EM)}~\cite{li2022automating, pornprasit2023d, tufano2019learning} is the number of the generated improved code that is the same as the actual improved code in the testing dataset.
        We use this measure since it is widely used for evaluating code review automation approaches~\cite{tufano2022using, pornprasit2023d,tufano2019learning}.
        To compare the generated improved code with the actual improved code, we first tokenize both improved code to sequences of tokens.
        Then, we compared the sequence of tokens of the generated improved code with the sequence of tokens of the actual improved code.
        % The higher EM, the better a model to generate code that is exactly the same as the actual code
        A high value of EM indicates that a model can generate improved code that is the same as the actual improved code in the testing dataset.
        
        \item \textbf{CodeBLEU}~\cite{ren2020codebleu} is the extended version of BLEU (i.e., an n-gram overlap between the translation generated by a deep learning model and the translation in ground tr\-uth)~\cite{bleu} for automatic evaluation of the generated code.
        We do not measure BLEU like in prior work~\cite{tufano2022using, li2022automating} since Ren~\ea~\cite{ren2020codebleu} found that this measure ignores syntactic and semantic correctness of the generated code.
        In addition to BLEU, CodeBLEU considers the weighted n-gram match, matched syntactic information (i.e., abstract syntax tree: AST) and matched semantic information (i.e., data flow: DF) when computing the similarity between the generated improved code and the actual improved code.
        % CodeBLEU can be calculated by the following equation:
        % % \begin{multline}
        %     % \nonumber
        % \footnotesize
        % $$\text{CodeBLEU} = \alpha \cdot \text{BLEU} + \beta \cdot \text{BLEU\textsubscript{weight}} + 
        % \gamma \cdot \text{Match\textsubscript{AST}} + \delta \cdot \text{Match\textsubscript{DF}}$$
        % % \end{multline}      
        % \normalsize
        % The higher CodeBLEU, the better a model to generate code that is syntactically and semantically similar to the actual code.
        A high value of CodeBLEU indicates that a model can generate improved code that is syntactically and semantically similar to the actual improved code in the testing dataset.

    \end{enumerate}


\subsection{Hyper-Parameter Setting}

    In this study, we use the following hyper-parameter settings when using GPT-3.5 to generate improved code: temperature of 0.0 (as suggested by Guo~\ea~\cite{guo2023exploring}), top\_p of 1.0 (default value), and max length of 512.
    To fine-tune GPT-3.5, we use hyper-parameters  (e.g., number of epochs and learning rate) that are automatically provided by OpenAI API.

    For Magicoder~\cite{wei2023magicoder}we use the same hyper-parameter as GPT-3.5 to generate improved code.
    To fine-tune Magicoder, we use the following hyper-parameters for DoRA~\cite{liu2024dora}: attention dimension $r$ of 16, alpha $\alpha$ of 8, and drop out of 0.1 .


% \subsection{Overview of Our Study Design}

% \kla{honestly, I don't understand the rest of this section. very hard to read.}

% \textit{(Oat): don't forget to fix based on comments}

% Figure~\ref{fig:study-design} presents an overview of our study design.
% We do zero-shot and few-shot prompting, and fine-tune GPT-3.5 to generate improved code (i.e., code after being revised) from a given submitted code (and a reviewer comment if available).
% % We perform zero-shot learning, perform few-shot learning, and fine-tune GPT-3.5 to generate improved code (i.e., code after being revised) from a given submitted code (and a reviewer comment if available).
% We choose GPT-3.5 in our study since GPT-3.5 is trained by using Reinforcement Learning from Human Feedback (RLHF)~\cite{ouyang2022training} to ensure that the generated output has high quality.
% To do zero-shot prompting with GPT-3.5, we ask GPT-3.5 to generate the improved code from the given input prompts.
% To do few-shot prompting with GPT-3.5, we first construct input prompts from the test samples and their selected demonstration examples.
% Then, we ask GPT-3.5 to generate the improved code from the given input prompts.
% Finally, for fine-tuning GPT-3.5, we use the selected training examples to fine-tune GPT-3.5.
% Then, we ask fine-tuned GPT-3.5 to generate the improved code from a given submitted code and a reviewer's comment (if available).
% In the below sections, we explain the details of prompt design, zero-shot prompting, few-shot prompting, and fine-tuning GPT-3.5.
% In the below sections, we explain how we design prompt templates for GPT-3.5, do zero-shot and few-shot prompting with GPT-3.5, and fine-tune GPT-3.5 in detail.

% To perform zero-shot learning with GPT-3.5 (as shown in Figure~\ref{fig:zero-shot-app}), we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt} and the code submitted for review (and reviewer's comment if available) in the testing set.
% Then, we ask GPT-3.5 to generate the improved code from a given input prompt.
% Then, we use GPT-3.5 to generate the improved code from the generated prompts.
% Then, we use the generated prompts as inputs to GPT-3.5 to generate the improved code.

% To perform few-shot learning with GPT-3.5 (as shown in Figure~\ref{fig:few-shot-app}), we first obtain three example pairs of input and output from the training set by using BM25~\cite{robertson2009probabilistic} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package.
% % select three pairs of input and output from the training set for each testing sample by using BM255~\cite{robertson2009probabilistic}.
% We do so since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches.
% % To select examples, we use the implementation of BM25~\cite{robertson2009probabilistic} from the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package. 
% % to select three pairs of input and output from the training set for each testing sample.
% Then, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt}, together with the input in the testing set and its corresponding selected examples
% % we use the input in the testing set and its corresponding selected examples to construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt}.
% After that, we ask GPT-3.5 to generate the improved code from a given input prompt.

% To fine-tune GPT-3.5 (as shown in Figure~\ref{fig:fine-tune-app}), we first randomly select approximately 6\% of total input/output pairs from the training dataset.
% We do not use the whole training set to fine-tune GPT-3.5 since it is prohibitively expensive.
% % select a subset of input/output pairs from the training dataset.
% % In particular, we randomly select approximately 6\% of the training dataset since using the whole training set to fine-tune GPT-3.5 is expensive.
% Then, we use the selected training examples to fine-tune GPT-3.5 by using the API provided by OpenAI\footnote{https://platform.openai.com/docs/guides/fine-tuning/create-a-fine-tuned-model}.
% % To do so, we fine-tune GPT-3.5 with and without using persona, similar to RQ2.
% After that, we ask fine-tuned GPT-3.5 to generate the improved code from a given submitted code and a reviewer's comment (if available).


% Outperform the existing deep learning-based approaches~\cite{}
% Due to very large model size, need just a few examples for fine-tuning (compared to fine-tuning pre-trained models that require thousands of data)
% Thus, good for early-stage software projects
% In later stage, developers may use models that they train by themselves.


% \revised{R1-3}{
% \subsection{Motivation of using GPT-3.5}

% We use GPT-3.5 in our study since prior work~\cite{deligiannis2023fixing, eliseeva2023commit, kang2023large, schafer2023adaptive} showed that GPT-3.5 can outperform the existing approaches in various software engineering tasks.
% Besides, GPT-3.5 requires a few examples to adapt to the tasks that it has never learnt during model pre-training phase.
% Thus, GPT-3.5 is suitable for early-stage software projects that do not have a large amount of dataset for fine-tuning pre-trained code models.
% }



% \subsection{Prompt Design}
% A prompt is a set of instructions provided to LLMs that programs LLMs to generate a desirable output~\cite{white2023prompt}.
% To ensure that LLMs generate a desirable output, a prompt needs to be carefully designed.
% Thus, in our study, we design the prompt templates for zero-shot prompting and few-shot prompting with GPT-3.5.
% % We do zero-shot prompting and few-shot prompting in our study over the others since the code review task is suitable for these prompting techniques.
% To design prompt templates, we follow the guidelines from OpenAI\footnote{https://help.openai.com/en/articles/6654000-best-practices-for-prompt-engineering-with-openai-api}\footnote{https://platform.openai.com/docs/guides/prompt-engineering/strategy-write-clear-instructions} to ensure that the structure of the prompt is suitable for GPT-3.5.
% % Figure~\ref{fig:zero-shot prompt with comment} and Figure~\ref{fig:zero-shot prompt without comment} show the prompt templates for zero-shot learning while Figure~\ref{fig:few-shot prompt with comment} and Figure~\ref{fig:few-shot prompt without comment} show the prompt templates for few-shot learning.
% Figure~\ref{fig:zero-shot prompt with comment} and Figure~\ref{fig:zero-shot prompt without comment} present the prompt template for zero-shot learning which consists of the following components: perso\-na~\cite{white2023prompt}, instruction and input (i.e., submitted code).
% The input also includes a reviewer comment if available.
% On the other hand, Figure~\ref{fig:few-shot prompt with comment} and Figure~\ref{fig:few-shot prompt without comment} present the prompt template for few-shot learning which consists of components similar to the ones in the prompt template for zero-shot learning, and a set of input (i.e., submitted code and a reviewer comment) and output (i.e., improved code) example pairs.
% % In particular, the prompt template for zero-shot learning (as depicted in Figure~\ref{fig:zero-shot prompt with comment} and Figure~\ref{fig:zero-shot prompt without comment}) consists of the following components: perso\-na~\cite{white2023prompt}, instruction and input (i.e., submitted code).
% % The input also includes a reviewer comment if available.
% % On the other hand, the prompt template for few-shot learning (as depicted in Figure~\ref{fig:few-shot prompt with comment} and Figure~\ref{fig:few-shot prompt without comment}) consists of components similar to the ones in the prompt template for zero-shot learning, and a set of input (i.e., submitted code and a reviewer comment) and output (i.e., improved code) example pairs.
% We include persona in both prompt templates to instruct GPT-3.5 to act as a software developer.
% We do so to ensure that the improved code generated by GPT-3.5 looks like the source code written by a software developer.
% % GPT-3.5 generate improved code as software developers would do.
% For the prompt template for few-shot prompting, we provide a set of example pairs to help GPT-3.5 adapt to the new task that it has never learned before.


% \subsection{Zero-Shot Learning}
% Zero-shot learning is the prompting technique that involves prompting LLMs to generate an output from a given instruction and an input.
% Zero-shot learning can be considered when only an instruction and an input (i.e., code submitted for review with a reviewer comment) are available.
% To do zero-shot prompting with GPT-3.5, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt with comment} and the code submitted for review with a reviewer comment in the testing set.
% However, in case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:zero-shot prompt without comment} and the code submitted for review instead.
% Then, we ask GPT-3.5 to generate the improved code from a given input prompt.


% %     \item In-context learning (ICL)~\cite{brown2020language, liu2021makes, wei2023larger} involves prompting LLMs to generate an output from example input/output pairs and an input.

% \subsection{Few-Shot Learning}
% Few-shot learning~\cite{brown2020language, liu2021makes, wei2023larger} is the prompting technique that involves prompting LLMs to generate an output from a given instruction, demonstration examples and an actual input.
% The benefit of this prompting technique over zero-shot learning is that this prompting technique can help LLMs adapt to domain-specific tasks without model fine-tuning.
% To do few-shot prompting with GPT-3.5, we first obtain three example pairs of input and output from the training set by using BM25~\cite{robertson2009probabilistic} provided by the \texttt{gensim}\footnote{https://github.com/piskvorky/gensim} package.
% We do so since prior work~\cite{gao2023constructing, yuan2023evaluating} shows that BM25~\cite{robertson2009probabilistic} can outperform other sample selection approaches.
% Then, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt with comment}, the code submitted for review and reviewer comment in the testing set, and its corresponding selected examples.
% In case a reviewer comment is not available, we construct input prompts from the prompt template in Figure~\ref{fig:few-shot prompt without comment}, the code submitted for review in the testing set, and its corresponding selected examples instead.
% After that, we ask GPT-3.5 to generate the improved code from a given input prompt.


% \subsection{Fine-Tuning GPT-3.5}
% Model fine-tuning refers to further training pre-trained LLMs on domain-specific tasks so that LLMs can adapt to new tasks that it never learn during the pre-training phase.
% To fine-tune GPT-3.5, we first randomly select approximately 6\% of total input/output pairs from the training dataset.
% % We do not use the whole training set to fine-tune GPT-3.5 since it is prohibitively expensive.
% Then, we use the selected training examples to fine-tune GPT-3.5 by using the API provided by OpenAI\footnote{https://platform.openai.com/docs/guides/fine-tuning/create-a-fine-tuned-model}.
% After that, we ask the fine-tuned GPT-3.5 to generate the improved code from a given submitted code and a reviewer comment (if available).

